Morse theory and higher torsion invariants II

Let p: M -> B be a family of compact manifolds equipped with a unitarily flat vector bundle F -> M. We generalize Igusa's higher Franz-Reidemeister torsion \tau(M/B;F) to the case that the fibre-wise cohomology H^*(M/B;F) -> B carries a parallel metric. If moreover M admits a fibre-wise Morse function, we compute the difference of \tau(M/B;F) and the higher analytic torsion \Cal T(M/B;F). We also generalise the examples given in math.DG/0111222 .

==> chtor.tex <==
%auto-ignore
\input morse2.def

\document

\Kapitel\ChernKapitel=7 Properties of the finite-dimensional higher torsion

In this chapter,
we collect some elementary properties
of the Chern torsion classes~$T(A',g^V,h^V)$
introduced in \TorsionKapitel.

We start by giving a description
of~$T(A',g^V,h^V)=T(\nabla^V,A',g^V)$
in Subsections~\NummerVon\ChernTorsionSubsection\
and~\NummerVon\ChernAltSubsection,
which does not make use of the function~$h^V$.
This is important for two reasons.
First,
it allows us to define a torsion class~$T(R,G)$
on the acyclic Whitehead space~$\Wh^h(R,G)$ in \TChRGDef,
and as well on the unitary Whitehead space~$\Wh^u(R,G)$ in \UniKapitel.
Second,
the new representation of~$T\(\nabla^V,A'g^V\)$
will allow us to compare Igusa's higher Franz-Reidemeister torsion
and~$T$ on a suitable Whitehead space in \IgusaKapitel.

We then analyse the behaviour of~$T(\nabla^V,A',g^V)$
on globally filtered complexes.
Applications include a gluing formula for the combinatorial torsion,
an extension of the examples in \BeispielKapitel,
and a reduction of the unitary higher torsion to an acyclic situation
in \UniKapitel.

%This result was already used in \BeispielKapitel\
%to calculate the higher torsions of a family of connected sums of manifolds.
%By a differential cone construction similar to Igusa's cone construction
%in \?where?,
%we can show that~$T(\nabla^V,A',g^V)$
%is determined by the higher torsion
%of an acyclic complex related to~$(V,\nabla^V,A')$.
%Then Igusa's two-index theorem implies
%that the universal torsion on the unitary Whitehead space
%is determined by its restriction
%to the acyclic two-index Whitehead space~$\Wh^{h,\{0,1\}}(R,G)$.

%Finally,
%we discuss an application of the above results to Lott's secondary $K$-theory
%of flat bundles.


\Abschnitt\ChernTorsionSubsection The Chern normalisation of the torsion forms

We give a formula for finite-dimensional the Chern torsion form
of \TorsionKapitel\ as an integral of the Chern form of a superconnection
over a two-dimensional domain.
This is the first step in finding a formula for~$T(A',g^V,h^V)$
that does not involve the endomorphism~$h^V$.

Let~$f(x)=x\,e^{x^2}$,
and recall that by \MVBTorsionDef\ and \ChernNormDef,
$$\split
	T\(A',g^V,h^V\)
	&=\int_0^1\(4s(1-s)\)\hochhalb{N^B}T_f\(A',g^V,h^V\)\,ds\\
	&=-\int_0^1\biggl({4s(1-s)\over2\pi i}\biggr)^{N^B\over 2}
		\int_1^\infty\Bigl(\strace_V\(N^Vf'(X_{t,1})\)-\chi'(H)f'(0)\\
	&\kern7em
		-\(\chi'(V)-\chi'(H)\)
			\,f'\(\sqrt{-t}/2\)\Bigr)
		\,{dt\over2t}\,ds\\
\noalign{\smallskip}
	&\qquad
	-\int_0^1\biggl({4s(1-s)\over2\pi i}\biggr)\hochhalb{N^B}
		\int_0^1\Bigl(\strace_V\(h^Vf'(X_{1,T})\)
			-\strace_V\(h^V\)\,f'(0)\\
	&\kern7em
		-\(\chi'(V)-\chi'(H)\)
			\,\(f'(\sqrt{-T}/2)-f'(0)\)\Bigr)
		\,{dT\over2T}\,ds\;.
\endsplit\Formel\TChFormel$$

Let~$\overline A'
=A'+{\del\over\del s}\,ds+{\del\over\del t}\,dt+{\del\over\del T}\,dT$
be the extension of the flat superconnection~$A'=\nabla^V+a_0+\dots$
to the pullback~$\^1\overline B=B\times(0,1)\times\R_>^2$.
We define a metric
	$$\^1g^{\overline V}
	=g^V\biggl(\Bigl({t\over4s(1-s)}\Bigr)^{N^V}
		\,T^{h^V}\punkt,\punkt\biggr)\;,$$
which coincides with the metric of~\GtTDef\ at~$s={1\over2}$.
Let~$\^1\overline A''$ denote the adjoint of~$\overline A'$
with respect to~$\^1g^{\overline V}$,
then
$$\split
	\^1\overline A''
	&=\nabla^{V,*}
		+\sum_j\biggl({t\over4s(1-s)}\biggr)^{1-j}
			\,T^{-h^V}\,a''_j\,T^{h^V}\\
	&\qquad
		+\log T\,dh^V
		+\biggl({\del\over\del s}
			+{N^V\over 1-s}-{N^V\over s}\biggr)\,ds
		+\biggl({\del\over\del t}+{N^V\over t}\biggr)\,dt
		+\biggr({\del\over\del T}+{h^V\over T}\biggr)\,dT\;.
\endsplit$$
Conjugating everything by~$\bigl({t\over4(1-s)^2}\bigr)\hochhalb{N^V}
\,T\hochhalb{h^V}$
gives two flat superconnections
$$\align
\split
	\^1\Asl'
	&=\nabla^V
		+\sum_j\biggl({t\over4(1-s)^2}\biggr)\hochhalb{1-j}
			\,T\hochhalb{h^V}\,a'_j\,T\hochmhalb{h^V}
		-{\log T\over2}\,dh^V\\
	&\qquad
		+\biggl({\del\over\del s}-{N^V\over 1-s}\biggr)\,ds
		+\biggl({\del\over\del t}-{N^V\over 2t}\biggr)\,dt
		+\biggr({\del\over\del T}-{h^V\over 2T}\biggr)\,dT\;,
\endsplit\Formel\EinsAslxFormel\\
\noalign{\smallskip}\allowdisplaybreak
\split
	\^1\Asl''
	&=\nabla^{V,*}
		+\sum_j\biggl({t\over4s^2}\biggr)\hochhalb{1-j}
			\,T\hochmhalb{h^V}\,a''_j\,T\hochhalb{h^V}
		+{\log T\over2}\,dh^V\\
	&\qquad
		+\biggl({\del\over\del s}-{N^V\over s}\biggr)\,ds
		+\biggl({\del\over\del t}+{N^V\over 2t}\biggr)\,dt
		+\biggr({\del\over\del T}+{h^V\over 2T}\biggr)\,dT\;.
\endsplit\Formel\EinsAslxxFormel\endalign$$

As in~\BGzwei,
we consider the superconnection
$$\split
	\^1\Asl
	&=(1-s)\,\^1\Asl'+s\,\^1\Asl''\\
	&=\nabla^{\overline V,u}
		+\sum_j\biggl({t\over4}\biggr)\hochhalb{1-j}\,
			\biggl((1-s)^j\,T\hochhalb{h^V}\,a'_j\,T\hochmhalb{h^V}
				+s^j\,T\hochmhalb{h^V}\,a''_j\,T\hochhalb{h^V}
			\biggr)\\
	&\qquad
		+(2s-1)\,\biggl({\omega^V\over2}
			+{\log T\over 2}\,dh^V+{N^V\over 2t}\,dt
			+{h^V\over 2T}\,dT\biggr)-2N^V\,ds\;.
\endsplit\Formel\EinsAslFormel$$
Note that~$\^1\Asl$ contains no negative powers of~$1-s$ or~$s$,
so we can extend it to~$B\times[0,1]\times\R_>^2$.
Because both~$\^1\Asl'$ and~$\^1\Asl''$ are flat,
we find that
	$$\^1\Asl^2
	=-s(1-s)\,\Bigl(\^1\Asl''-\^1\Asl'\Bigr)^2
		-\Bigl(\^1\Asl''-\^1\Asl'\Bigr)\,ds\;.
	\Formel\BGZweiInterpolationFormel$$

\Remark\AslSquareRem
Formula\BGZweiInterpolationFormel\
is well suited for describing~$\^1\Asl^2$
in~$B\times(0,1)\times[1,\infty)\times\R$.
For the restriction to~$s=0$,
we obtain instead
$$\split
	\^1\Asl\bigr|_{s=0}
	&=\^1\Asl'\bigr|_{s=0}
		+{\sqrt t\over 2}\,T\hochmhalb{h^V}\,a''_0\,T\hochhalb{h^V}\\
	\Land
	\^1\Asl^2\bigr|_{s=0}
	&=\biggl[\^1\Asl'\bigr|_{s=0}
		\,,\;{\sqrt t\over 2}\,T\hochmhalb{h^V}\,a''_0\,T\hochhalb{h^V}
		\biggr]\;.
\endsplit\Formel\AslSquareRemFormel$$
Note that~$\^1\Asl^2|_{s=0}$ is in triangular shape with respect
to the $\Z$-grading of~$V$,
with the diagonal term given
by~${t\over4}\,\bigl[T\hochhalb{h^V}\,a'_j\,T\hochmhalb{h^V},
T\hochmhalb{h^V}\,a''_0\,T\hochhalb{h^V}\bigr]$.
This has two consequences.
\roster
\item
The kernel of~$\(\^1\Asl^2\)\dg0$ does not jump at~$s=0$, and
\item
The restriction of~$\strace\(\^1\Asl^2\)\dg0$ to~$s=0$
is of degree~$0$.
\endroster
Similar observations are of course true at~$s=1$.
\endremark	


\Proposition\TChProp.
Up to exact forms on~$B$,
the Chern analytic torsion form is given by
	$$\align
	T\(A',g^V,h^V\)
	&=-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,t)\in[0,1]\times[1,\infty)}\biggl(
			{1\over2}\,\strace_V\Bigl(e^{-\^1\Asl^2}\Bigr)
				-\chi'(H)\,{ds\,dt\over 2t}\\
	&\kern10em
		-\(\chi'(V)-\chi'(H)\)\,f'\(\sqrt{-t}/2\)
			\,{ds\,dt\over2t}\biggr)\\
\noalign{\smallskip}\allowdisplaybreak
	&\qquad
		-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,T)\in[0,1]^2}\biggl(
		{1\over2}\,\strace_V\Bigl(e^{-\^1\Asl^2}\Bigr)
			-\strace_V\(h^V\)
		\,{ds\,dT\over 2T}\\
	&\kern10em
		-\(\chi'(V)-\chi'(H)\)
			\,(\Bigl(f'\(\sqrt{-T}/2\)-1\Bigr)
		\,{ds\,dT\over2T}\biggr)\;.
\endalign$$

\Proof
Comparing \MVBTorsionDef\ and \ChernNormDef\
with the formula above,
we easily see that the proposition holds in degree~$0$.
In particular,
we do not need to investigate any correction terms.

Let~$\^1\Asl'$ and~$\^1\Asl''$
be defined by~\EinsAslxFormel, \EinsAslxxFormel,
and set
	$$\^1\Xsl
	={1\over2}\,\Bigl(\^1\Asl''-\^1\Asl'\Bigr)
	=\^1\Xsl_{s,t,T}
		+\biggl({N^V\over 2(1-s)}-{N^V\over 2s}\biggr)\,ds
		+{N^V\over 2t}\,dt+{h^V\over 2T}\,dT\;,$$
then
	$$\^1\Xsl^2
	=\^1\Xsl_{s,t,T}^2
	+\biggl[\biggl({N^V\over 2(1-s)}-{N^V\over 2s}\biggr)\,ds
		+{N^V\over 2t}\,dt+{h^V\over 2T}\,dT\;,
			\;\^1\Xsl_{s,t,T}\biggr]\;.
	\Formel\IgusaXslQuadratFormel$$

We calculate the following contribution
to the integrand in formula~\TChFormel\ for~$T\(A',g^V,h^V\)$:
$$\multline
	\int_0^1\(4s(1-s)\)\hochhalb{N^B}\strace\Biggl(
		\biggl({N^V\over2t}\,dt+{h^V\over2T}\,dT\biggr)
		\,f'\Bigr(\Xsl_t\Bigr)\Biggr)\,ds\\
\split
	&=\int_0^1\strace\Biggl(
		\biggl({N^V\over2t}\,dt+{h^V\over2T}\,dT\biggr)
		\,f'\biggl(\sqrt{s(1-s)}
		\,\Bigl(\Asl''_{\topsmash{\textstyle{t\over4s(1-s)}},T}
		-\Asl'_{\topsmash{\textstyle{t\over4s(1-s)}},T}\Bigr)
		\biggr)\Biggr)\,ds\\
	&=\int_0^1\strace\Biggl(
		\biggl({N^V\over2t}\,dt+{h^V\over2T}\,dT\biggr)
		\,f'\biggl(\sqrt{s(1-s)}
		\,\Bigl(\Asl''_{\topsmash{\textstyle{\;t\over4s^2}},T}
		-\Asl'_{\topsmash{\textstyle{t\over4(1-s)^2}},T}\Bigr)
		\biggr)\Biggr)\,ds\\
	&=\int_0^1\strace\Biggl(
		\biggl({N^V\over2t}\,dt+{h^V\over2T}\,dT\biggr)
		\,f'\Bigl(\sqrt{4s(1-s)}
		\;\^1\Xsl_{s,t,T}\Bigr)\Biggr)\,ds\;.
\endsplit\endmultline\tag\FormelNummer\IgusaTChIntegrand$$
For the second equation,
we have conjugated by~$\bigl({s\over1-s}\bigr){}^{\botsmash{N^V\over 2}}$
within the trace.

On the other hand,
by~\BGZweiInterpolationFormel\ and~\IgusaXslQuadratFormel,
and because the supertrace of an even positive power
of an odd operators vanishes,
we have
$$\split
	{1\over2}\,\strace\Bigl(e^{-\^1\Asl^2}\Bigr)
	&={1\over2}
		\,\strace\Bigl(e^{4s(1-s)\,\^1\Xsl^2+2\,\^1\Xsl\,ds}
			\Bigr)\\
	&=\chi(V)+{1\over\sqrt{4s(1-s)}}
		\,\strace\Bigl(f\(\sqrt{4s(1-s)}\,\^1\Xsl\)\Bigr)\,ds\\
	&=\chi(V)+{1\over\sqrt{4s(1-s)}}
		\,\strace\Bigl(f\(\sqrt{4s(1-s)}
			\,\^1\Xsl_{s,t,T}\)\Bigr)\,ds\\
	&\qquad
		+\strace\biggl(\biggl({N^V\over2t}\,dt+{h^V\over 2T}\,dT\biggr)
			\,f'\Bigl(\sqrt{4s(1-s)}\,\^1\Xsl_{s,t,T}\Bigr)
		\biggr)\,ds
		+\dots\;,
\endsplit\Formel\IgusaTChIntegrandZwei$$
where the remaining term involves~$ds$, $dt$ and~$dT$.
The previous equation and~\IgusaTChIntegrand\ together
with \MVBTorsionDef\ and \ChernNormDef\
prove the proposition.
\qed\enddemo


\Abschnitt\ChernAltSubsection A new formula for the Chern torsion classes

We now want to get rid of the endomorphism~$h^V$
in our formula for~$T\(A',g^V,h^V\)$.
This implies that we have to replace the last integral in \TChProp\
by something different.
This is done in two steps,
\ZweiAslProp\ and \ChTorsionThm.

First,
let
	$$\^2\overline V
		\to \^2\overline B
		=B\times(0,1)\times\R_>\times[0,1]$$
be the pullback of~$V\to B$,
and let~$(s,T,u)$ be the coordinates on~$(0,1)\times\R_>\times[0,1]$.
We extend the superconnections~$\Asl'|_{t=1/4}$ and~$\Asl''|_{t=1/4}$
of~\MVBAslFormel\
and~$\^1\Asl|_{t=1}$ to~$\^2\overline B$,
and set
	$$\Asl=(1-s)\,\Asl'+s\,\Asl''\;.\Formel\AslFormel$$
We then consider the superconnection
$$\split
	\^2\Asl
	&=u\,\^1\Asl|_{t=1}+(1-u)\,\Asl|_{t=1/4}\\
	&=\nabla^{\overline V,u}+\sum_j2^{j-1}
		\,\biggl(\((1-s)^ju+(1-s)(1-u)\)
				\,T\hochhalb{h^V}\,a'_j\,T\hochmhalb{h^V}\\
	&\kern8em
			+\(s^ju+s(1-u)\)
				\,T\hochmhalb{h^V}\,a''_j\,T\hochhalb{h^V}
		\biggr)\\
	&\qquad
		+(2s-1)\,\biggl({\omega^V\over2}
			+{\log T\over 2}\,dh^V
			+{h^V\over 2T}\,dT\biggr)
		-2u\,N^V\,ds\;.
\endsplit\Formel\ZweiAslFormel$$

As~$T\to 0$,
this superconnection becomes singular.
Note that by \MVBDef,
there exists~$\eps>0$ with
	$$T\hochhalb{h^V}\,a'_j\,T\hochmhalb{h^V}
	=O\Bigl(T\hochhalb\eps\Bigr)
		\Mand
	T\hochmhalb{h^V}\,a''_j\,T\hochhalb{h^V}
	=O\Bigl(T\hochhalb\eps\Bigr)\;.
	\Formel\AslGoodTerms$$
The remaining terms in~$\^2\Asl$ define a new superconnection
$$%\split
	\^2\Asl_0 %&
	=\nabla^{\overline V,u}
		+(2s-1)\,\^2\Xsl_0-2u\,N^V\,ds\;,%\\
%	&=(1-s)\,\biggl(\nabla^{\overline V}
%			-{\log T\over 2}\,dh^V-{h^V\over 2T}\,dT\biggr)\\
%	&\qquad
%		+s\,\biggl(\nabla^{\overline V,*}
%			+{\log T\over 2}\,dh^V+{h^V\over 2T}\,dT\biggr)
%		-2u\,N^V\,ds\;.
%\endsplit
$$
where
	$$\^2\Xsl_0
	={\omega^V\over2}+{\log T\over 2}\,dh^V+{h^V\over 2T}\,dT\;.$$
Note that~$\^2\Xsl_0^2=\omega^V/4$.
Because~$N^V$ commutes with~$\^2\Asl_0$,
the curvature of~$\^2\Asl_0$ is %as in~\BGZweiInterpolationFormel\
given by
$$%\split
	\^2\Asl_0^2 %&
	=-s(1-s)\,\(\omega^V\)^2-2\,\^2\Xsl_0\,ds-2\,N^V\,du\,ds %\\
%	&=-s(1-s)\,\(\omega^V\)^2
%		-\biggl(\omega^V+\log T\,dh^V+{h^V\over T}\,dT\biggr)\,ds
%		-2\,N^V\,du\,ds\;.
%\endsplit
$$

Let us now compute the (unnormalised) Chern character form of~$\^2\Asl_0$.
We find that
$$\split
	\strace\Bigl(e^{-\^2\Asl_0^2}\Bigr)
	&=\strace\Bigl(e^{s(1-s)\,\(\omega^V\)^2}\Bigr)
		-2\strace\Bigl(N^V\,e^{s(1-s)\,\(\omega^V\)^2}\Bigr)\,du\,ds\\
	&\qquad
		+{1\over\sqrt{s(1-s)}}
			\,\strace\biggl(f\Bigl(\sqrt{4s(1-s)}\,\^2\Xsl_0\Bigr)
				\biggr)\,ds\\
\noalign{\smallskip}\allowdisplaybreak
%	&=\chi(V)-2\chi'(V)\,du\,ds
%		+{1\over\sqrt{s(1-s)}}
%			\,\strace\biggl(f\Bigl(\sqrt{s(1-s)}\,\omega^V\Bigr)
%				\biggr)\,ds\\
%	&\qquad
%		+d\strace\biggl(h^V\,\log T
%				\,f'\Bigl(\sqrt{s(1-s)}\,\omega^V\Bigr)
%				\biggr)\,ds\\
%\noalign{\smallskip}\allowdisplaybreak
	&=\chi(V)-2\chi'(V)\,du\,ds+d\strace\(h^V\,\log T\)\,ds\\
	&\qquad
%		+{1\over\sqrt{s(1-s)}}
%			\,\strace\biggl(f\Bigl(\sqrt{s(1-s)}\,\omega^V\Bigr)
%				\biggr)\,ds
		+\strace\Bigl(\omega^V\,e^{s(1-s)\,\(\omega^V\)^2}\Bigr)
			\,ds\;.
\endsplit\Formel\ZweiAslChFormel$$
Here we have used that positive even powers of odd operators vanish,
that~$\bigl[\nabla^{V,u},\omega^V\bigr]=0$,
and that~$\omega^V$, $h^V$ and~$N^V$ supercommute pairwise.

As in~\AlphaTZeroLimit,
it follows that there exists an~$\eps'>0$ with
$$\multline
	\strace\Bigl(e^{-\^2\Asl^2}\Bigr)
		-d\strace\(h^V\,\log T\)\,ds
%\strace\(h^V\)\,{dT\,ds\over T}-\log T\,d\strace\(h^V\)\,ds
	\\
	=\chi(V)-2\chi'(V)\,du\,ds
		+\strace\Bigl(\omega^V\,e^{s(1-s)\,\(\omega^V\)^2}\Bigr)\,ds
	+O\(T^{\eps'}\)+O\(T^{\eps'}\)\,{dT\over T}\;,
\endmultline\tag\FormelNummer\ZweiAslTZeroLimit$$
where the terms~$O\(T^{\eps'}\)$ do not contain the exterior variable~$dT$.

For~$T_0>0$, consider the polyhedron~$\^2D=[0,1]\times[T_0,1]\times[0,1]$.
\psset{unit=0.07\hsize}
$$\pspicture(-1.5,-1)(2.5,2.4)
\ifdraft\psline(-1.5,-1)(2.5,-1)(2.5,2.4)(-1.5,2.4)(-1.5,-1)\fi
	\psline{->}(0,-0.1)(0,2)
%	\uput[270](0,-0.1){$\scriptstyle 0$}
	\uput[90](0,2){$\scriptstyle T$}
	\psline{->}(-0.1,0)(2,0)
%	\uput[180](-0.1,0){$\scriptstyle 0$}
	\uput[0](2,0){$\scriptstyle u$}
	\psline{->}(0.1,0.05)(-1.2,-0.6)
	\uput[210](-1.2,-0.6){$\scriptstyle s$}
	\psline(1.6,-0.1)(1.6,0.1)
	\uput[270](1.6,-0.1){$\scriptstyle 1$}
	\psline(-1,-0.4)(-1,-0.6)
	\uput[270](-1,-0.6){$\scriptstyle 1$}
	\psline(-0.1,1.6)(0.1,1.6)
	\uput[180](-0.1,1.6){$\scriptstyle 1$}
	\psline(-0.1,0.2)(0.1,0.2)
	\uput[150](-0.1,0.2){$\scriptstyle T_0$}
	{\psset{linewidth=1.2pt}
	\psline(-1,1.3)(0.8,1.3)
	\psline(0.8,1.3)(1.6,1.6)
	\psline(-1,1.3)(0,1.6)
	\psline(0,1.6)(1.6,1.6)
	\psline(-1,-0.27)(-1,1.3)
	\psline(-1,-0.27)(0.8,-0.27)
	\psline(0.8,-0.27)(0.8,1.3)
	\psline(0.8,-0.27)(1.6,0.2)
	\psline(1.6,0.2)(1.6,1.6)
	\psset{linestyle=dashed}
	\psline(-1,-0.27)(0,0.2)
	\psline(0,0.2)(1.6,0.2)
	\psline(0,0.2)(0,1.6)
	\psset{linewidth=0.2pt}
	\psline(-1,-0.5)(0.8,-0.5)
	\psline(0.8,-0.5)(1.6,0)
	\psline(-1,-0.5)(-1,-0.28)
	\psline(0.8,-0.5)(0.8,-0.28)
	\psline(1.6,0)(1.6,0.2)}
\endpspicture$$

By Stokes' theorem, the form
	$$-(2\pi i)\hochmhalb{N^B}\int_{(B\times\del \^2D)/B}
		{1\over2}\,\biggl(\strace\Bigl(e^{-\^2\Asl^2}\Bigr)
			-\strace\(h^V\)\,{dT\,ds\over T}
			+2\chi'(V)\,du\,ds\biggr)
		$$
is exact.
We study the behaviour of the integrals over the six faces as~$T_0\to 0$.
This will allow us to replace one contribution to the Chern torsion class
by two contributions which are easier to handle.


\subsubhead$\alpha$) The faces~$s=0$ and~$s=1$\endsubsubhead
Let us consider the restriction to~$s=0$,
where by \AslSquareRemFormel, \ZweiAslFormel\ and~\AslFormel,
$$\align
	\^2\Asl|_{s=0}
	&=\Asl'|_{t=1/4}+{u\over2}\,T\hochmhalb{h^V}\,a''_0\,T\hochhalb{h^V}\\
		\Land
	\^2\Asl^2|_{s=0}
	&={u\over2}\,\biggl[\Asl'|_{t=1/4}\,
			,\;T\hochmhalb{h^V}\,a''_0\,T\hochhalb{h^V}\biggr]
		-{1\over2}\,T\hochmhalb{h^V}\,a''_0\,T\hochhalb{h^V}\,du
\endalign$$
because~$\bigl(\Asl'\bigr)^2=(a''_0)^2=0$.
Note that~$\^2\Asl^2|_{s=0}$ is in triangular shape with respect to~$N^V$,
with diagonal term
	$${u\over 4}\,\biggl[T\hochhalb{h^V}\,a'_0\,T\hochmhalb{h^V}\,
			,\;T\hochmhalb{h^V}\,a''_0\,T\hochhalb{h^V}\biggr]\;.$$
This implies that the supertrace of~$e^{-\^2\Asl^2}$ contains neither~$dT$
nor~$du$.
A similar statement holds at~$s=1$.
In particular
	$$0
	=\int_{(s,T)\in[T_0,1]\times[0,1]}
		{1\over2}\,\strace\Bigl(e^{-\^2\Asl^2|_{s=0}}\Bigr)
	=\int_{(s,T)\in[T_0,1]\times[0,1]}
		{1\over2}\,\strace\Bigl(e^{-\^2\Asl^2|_{s=1}}\Bigr)\;.
	\Formel\ZweiSNullFormel$$

\subsubhead$\beta$) The face~$u=0$\endsubsubhead
With~\MVBAslFormel, \MVBXslFormel\ and~\BGZweiInterpolationFormel,
we have
$$\align
	\^2\Asl|_{u=0}
	&=(1-s)\,\Asl'|_{t=1/4}+s\,\Asl''|_{t=1/4}\\
		\Land
	\^2\Asl^2|_{u=0}
	&=-4s(1-s)\,\Xsl|_{t=1/4}^2-2\,\Xsl|_{t=1/4}\,ds\;.
\endalign$$

Again by~\ZweiAslTZeroLimit,
we know that the following integral exists:
	$$\int_{(s,T)\in[0,1]^2}
		\biggl({1\over2}\,\strace\Bigl(e^{-\^2\Asl^2|_{u=0}}\Bigr)
			-\strace\(h^V\)\,{dT\,ds\over 2T}\biggr)\;.$$

\subsubhead$\gamma$) The face~$u=1$\endsubsubhead
By~\EinsAslFormel\ and~\ZweiAslFormel,
	$$\^2\Asl|_{u=1}
	=\^1\Asl|_{t=1}\;.$$
In particular, \IgusaTChIntegrand\ and~\IgusaTChIntegrandZwei\ imply that
	$$\int_{(s,T)\in[0,1]\times[T_0,1]}
		{1\over2}\,\strace\Bigl(e^{-\^2\Asl^2|_{u=1}}\Bigr)
	=-\int_{T_0}^T\int_0^1\(4s(1-s)\)\hochhalb{N^B}
		\strace\biggl(h^V\,f'\Bigl(\Xsl_t\Bigr)\biggr)
		\,{dT\over2T}\;.$$

By~\ZweiAslTZeroLimit,,
we know that the following integral exists:
	$$\int_{(s,T)\in[0,1]\times[T_0,1]}
		\biggl({1\over2}\,\strace\Bigl(e^{-\^2\Asl^2|_{u=1}}\Bigr)
			-\strace\(h^V\)\,{dT\over 2T}\,ds\biggr)\;.$$

\subsubhead$\delta$) The face~$T=1$\endsubsubhead
The integral
	$$\int_{(s,u)\in[0,1]^2}
		\biggl({1\over2}\,\strace\Bigl(e^{-\^2\Asl^2|_{T=1}}\Bigr)
			+\chi'(V)\,du\,ds\biggr)$$
exists and can be nonzero.
It will become a contribution to~$T\(A',g^V,h^V\)$
in the next intermediate step.

\subsubhead$\eps$) The face~$T=T_0$\endsubsubhead
From~\ZweiAslTZeroLimit,
we conclude that
	$$\lim_{T_0\to 0}
	\int_{(s,u)\in[0,1]^2}
		\biggl({1\over2}\,\strace\Bigl(e^{-\^2\Asl^2|_{T=T_0}}\Bigr)
			+\chi'(V)\,du\,ds\biggr)
	=0\;.$$

Stokes' theorem and~$\alpha$--$\eps)$
imply the following intermediate result.

\Proposition\ZweiAslProp.
Up to exact forms on~$B$,
the Chern analytic torsion~$T\(A',g^V,h^V\)$
can be expressed as
	$$\align
	T\(A',g^V,h^V\)
	&=-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,t)\in[0,1]\times[1,\infty)}\biggl(
			{1\over2}\,\strace_V\Bigl(e^{-\^1\Asl^2}\Bigr)
				-\chi'(H)\,{dt\over 2t}\,ds\\
	&\kern10em
		-\(\chi'(V)-\chi'(H)\)
			\,f'\(\sqrt{-t}/2\)\,{dt\over2t}\,ds\biggr)\\
\noalign{\smallskip}\allowdisplaybreak
	&\qquad
		-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,u)\in[0,1]^2}\biggl(
		{1\over2}\,\strace_V\Bigl(e^{-\^2\Asl^2|_{T=1}}\Bigr)
			+\chi'(V)\,du\,ds\biggr)\\
\noalign{\smallskip}\allowdisplaybreak
	&\qquad
		-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,T)\in[0,1]^2}\biggl(
		{1\over2}\,\strace_V\Bigl(e^{-\^2\Asl^2|_{u=0}}\Bigr)
			-\strace_V\(h^V\)
		\,{dT\,ds\over 2T}\\
	&\kern10em
		-\(\chi'(V)-\chi'(H)\)
			\,\Bigl(f'\(\sqrt{-t}/2\)-1\Bigr)
		\,{dT\,ds\over2T}\biggr)\;.
\endalign$$

We are now in a position to finally eliminate~$h^V$
from our representation of~$T(A',g^V,h^V)$.
For the final step,
we let
	$$\^3\overline V
		\to\^3\overline B
		=B\times[0,1]\times\R_>\times[0,1]$$
be the pullback of~$V\to B$,
and let~$(s,T,v)$ be the coordinates on~$[0,1]\times\R_>\times[0,1]$.
We define a superconnection
$$\split
	\^3\Asl
	&=v\,\Bigl((1-s)\,\Asl'|_{t={1/4}}
			+s\,\Asl''|_{t={1/4}}\Bigr)
		+(1-v)\,\Bigl((1-s)\,\nabla^{\overline V}
			+s\,\nabla^{\overline V,*}\Bigr)\\
	&=\nabla^{\overline V,u}+v\,\sum_j2^{j-1}
		\,\biggl((1-s)\,T\hochhalb{h^V}\,a'_j\,T\hochmhalb{h^V}%\\
%	&\kern8em
			+s\,T\hochmhalb{h^V}\,a''_j\,T\hochhalb{h^V}\biggr)\\
	&\qquad
		+(2s-1)\,\biggl({\omega^V\over2}
			+v\,{\log T\over 2}\,dh^V
			+v\,{h^V\over 2T}\,dT\biggr)\;.
\endsplit\Formel\DreiAslFormel$$

As above, we use those terms that do not vanish as~$T\to 0$
to define a new superconnection
	$$\^3\Asl_0
	=\nabla^{\overline V,u}
		+(2s-1)\,\biggl({\omega^V\over2}
			+v\,{\log T\over 2}\,dh^V
			+v\,{h^V\over 2T}\,dT\biggr)\;.$$
Similar as above, we calculate
	$$\^3\Asl_0^2
	=-s(1-s)\(\omega^V\)^2-\omega^V\,ds
		-{1\over2}\,d\(h^V\,\log T\)\,d\((2s-1)v\)\;.$$
As above, this implies
that there exists an~$\eps'>0$ such that
$$\multline
	\strace\Bigl(e^{-\^3\Asl^2}\Bigr)
		-{1\over2}\,d\strace\(h^V\,\log T\)\,d\((2s-1)v\)\\
	=\chi(V)+\strace\Bigl(\omega^V\,e^{s(1-s)\,(\omega^V)^2}\Bigr)\,ds
	+O\(T^{\eps'}\)+O\(T^{\eps'}\)\,{dT\over T}\;,
\endmultline\tag\FormelNummer\DreiAslTZeroLimit$$

Let~$\^3D=[0,1]^3$, with coordinates~$s$, $T$ and~$v$.
By Stokes' theorem, the form
	$$-(2\pi i)\hochmhalb{N^B}\int_{(B\times\del \^3D)/B}
		{1\over2}\,\biggl(\strace\Bigl(e^{-\^3\Asl^2}\Bigr)
			-\strace\(h^V\)\,{dT\over 2T}
				\,d\((2s-1)v\)\biggr)$$
is exact.
We study the behaviour of the integrals over the six faces of~$\^3D$
as~$T_0\to 0$.
This will allow us to replace one contribution to the Chern torsion class
by another one that is easier to handle.


\subsubhead$\alpha$) The faces~$s=0$ and~$s=1$\endsubsubhead
Let us consider the restriction to~$s=0$,
where by~\DreiAslFormel,
$$\align
	\^3\Asl|_{s=0}
	&=v\,\Asl'|_{t={1/4}}+(1-v)\,\nabla^{\overline V}\\
		\Land
	\^3\Asl^2|_{s=0}
	&=-4v(1-v)\,\Bigl(\Asl'|_{t={1/4}}-\nabla^{\overline V}\Bigr)^2
		-2\,\Bigl(\Asl'|_{t={1/4}}-\nabla^{\overline V}\Bigr)\,dv\;.
\endalign$$
Note that~$\bigl(\Asl'|_{t={1/4}}-\nabla^{\overline V}\bigr)$
is in triangular shape with respect to the local partial ordering
induced by~$h^V$,
and the diagonal term is just~${1\over 2}\,d\(h^V\,\log T\)$.
A similar statement holds at~$s=1$.
In particular
$$\split
	0
	&=\int_{(T,v)\in[T_0,1]\times[0,1]}
		{1\over2}\,\biggl(\strace\Bigl(e^{-\^3\Asl^2|_{s=0}}\Bigr)
			+\strace\(h^V\)\,{dT\over 2T}\,dv\)\biggr)\\
	&=\int_{(T,v)\in[T_0,1]\times[0,1]}
		{1\over2}\,\biggl(\strace\Bigl(e^{-\^3\Asl^2|_{s=1}}\Bigr)
			-\strace\(h^V\)\,{dT\over 2T}\,dv\)\biggr)\;.
\endsplit$$


\subsubhead$\beta$) The face~$v=0$\endsubsubhead
With~\MVBAslFormel, \MVBXslFormel\ and~\BGZweiInterpolationFormel,
we have
	$$\^3\Asl|_{v=0}=(1-s)\,\nabla^{\overline V}+s\,\nabla^{\overline V,*}
		\Mand
	\^3\Asl^2|_{v=0}
	=-4s(1-s)\,\(\omega^V\)^2-2\,\omega^V\,ds\;.
	\Formel\AslDreiVnullFormel$$

Clearly, $\^3\Asl^2|_{v=0}$ does not contain the exterior variable~$dT$,
so
	$$\int_{(s,T)\in[0,1]^2}
		{1\over2}\,\strace\Bigl(e^{-\^3\Asl^2|_{v=0}}\Bigr)
	=0\;.$$

\subsubhead$\gamma$) The face~$v=1$\endsubsubhead
By~\ZweiAslFormel\ and \DreiAslFormel,
	$$\^3\Asl|_{v=1}
	=\^2\Asl|_{u=1}\;.$$
By~\ZweiAslTZeroLimit,
we know that the following integrals exist and are equal:
$$\multline
	\int_{(s,T)\in[0,1]^2}
		{1\over2}\,\biggl(\strace\Bigl(e^{-\^2\Asl^2|_{u=0}}\Bigr)
			-2\strace\(h^V\)\,{dT\over 2T}\,ds\biggr)\\
	=\int_{(s,T)\in[0,1]^2}
		{1\over2}\,\biggl(\strace\Bigl(e^{-\^3\Asl^2|_{v=1}}\Bigr)
			-2\strace\(h^V\)\,{dT\over 2T}\,ds\biggr)\;.
\endmultline$$

\subsubhead$\delta$) The face~$T=1$\endsubsubhead
The integral
	$$\int_{(s,v)\in[0,1]^2}
		{1\over2}\,\strace\Bigl(e^{-\^3\Asl^2|_{T=1}}\Bigr)$$
exists and can be nonzero.
It will become a contribution to~$T\(A',g^V,h^V\)$.

\subsubhead$\eps$) The face~$T=T_0$\endsubsubhead
From~\DreiAslTZeroLimit,
we conclude that
	$$\lim_{T_0\to 0}
	\int_{(s,v)\in[0,1]^2}
		{1\over2}\,\strace\Bigl(e^{-\^3\Asl^2|_{T=T_0}}\Bigr)
	=0\;.$$

We may thus define a Chern torsion form without using~$h^V$.

\Definition\ChtorDef
The finite dimensional {\em Chern torsion class\/} is
modulo exact forms defined as
	$$\align
	T\(\nabla^V,A',g^V\)
	&=-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,t)\in[0,1]\times[1,\infty)}\biggl(
			{1\over2}\,\strace_V\Bigl(e^{-\^1\Asl^2}\Bigr)
				-\chi'(H)\,{dt\,ds\over 2t}\\
	&\kern10em
		-\(\chi'(V)-\chi'(H)\)
			\,f'\(\sqrt{-t}/2\)\,{dt\,ds\over2t}\biggr)\\
\noalign{\smallskip}\allowdisplaybreak
	&\qquad
		-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,u)\in[0,1]^2}\biggl(
		{1\over2}\,\strace_V\Bigl(e^{-\^2\Asl^2|_{T=1}}\Bigr)
			-\chi'(V)\,du\,ds\biggr)\\
\noalign{\smallskip}\allowdisplaybreak
	&\qquad
		-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,v)\in[0,1]^2}\biggl(
		{1\over2}\,\strace_V\Bigl(e^{-\^3\Asl^2|_{T=1}}\Bigr)\\
	&\kern10em
		-\(\chi'(V)-\chi'(H)\)\,\Bigl(f'\(\sqrt{-t}/2\)-1\Bigr)
			\,{dv\,ds\over2v}\biggr)\;.
\endalign$$
\enddefinition

Then the considerations above immediately prove the following result.

\Theorem\ChTorsionThm.
The two definitions of a finite-dimensional Chern torsion form agree,
so up to exact forms on~$B$,
	$$T\(A',g^V,h^V\)=T\(\nabla^V,A',g^V\)\;.$$

If~$A'=\nabla^V+a'_0$ with~$a'_0\in\Gamma(\End^1V)$,
we let~$T^{\roman{BL}}(A',g^V)$ denote the Bismut-Lott torsion form
of~\BL\ in the Chern normalisation of~\BGzwei, cf.~\ChernSubsection.
Together with \MVBTorsionRem,
\ChTorsionThm\ has the following consequence.

\Corollary\ChBLTorCor.
Let~$A'=\nabla^V+a'_0$ with~$a'_0\in\Gamma(\End^1V)$,
then
	$$T\(\nabla^V,A',g^V\)=T^{\roman{BL}}(A',g^V)\;.$$

\Theorem\ChernBLThm.
Let~$(V,\nabla^V)\to B$ be a flat $\Z$-graded vector bundle
with a flat superconnection~$A'$ such that~$A'-\nabla^V\in\Omega^*(B;\End V)$
takes values in a nilpotent subalgebra of~$\End V$,
which may vary over~$B$.
Then for any metric~$g^V$ on~$V$,
we have
	$$dT\(\nabla^V,A',g^V\)=\cho\(\nabla^V,g^V\)-\cho\(\nabla^H,g^H\)\;.$$

\Proof
By \ChtorDef\ and the preceeding arguments,
we find that
$$\multline
	dT\(\nabla^V,A',g^V\)
	={1\over2}\,(2\pi i)\hochhalb{1-N^B}\Biggl(-\lim_{t\to\infty}\int_{s\in[0,1]}
			\strace_V\Bigl(e^{-\^1\Asl^2|_{T=1}}\Bigr)\\
\split
		&+\int_{s\in[0,1]}
			\strace_V\Bigl(e^{-\^3\Asl^2|_{v=0\atop T=1}}\Bigr)
		+\int_{t\in[1,\infty)}
			\strace_V\Bigl(e^{-\^1\Asl^2|_{T=1}}\Bigr)
			\biggr|_{s=0}^1\\
		&+\int_{u\in[0,1]}
			\strace_V\Bigl(e^{-\^2\Asl^2|_{T=1}}\Bigr)
			\biggr|_{s=0}^1
		+\int_{v\in[0,1]}
			\strace_V\Bigl(e^{-\^3\Asl^2|_{T=1}}\Bigr)
			\biggr|_{s=0}^1\Biggr)\;.
\endsplit\endmultline\tag\FormelNummer\ChBLdTFormel$$

Arguing as in~\IgusaTChIntegrand\ and~\IgusaTChIntegrandZwei,
we compute
$$\align
	\kern4em&\kern-4em
	(2\pi i)\hochhalb{1-N^B}\,
		\lim_{t\to\infty}\int_{s\in[0,1]}
			{1\over2}\,\strace_V\Bigl(e^{-\^1\Asl^2|_{T=1}}\Bigr)\\
	&=(2\pi i)\hochhalb{1-N^B}\,\lim_{t\to\infty}
		\int_{s\in[0,1]}{1\over\sqrt{4s(1-s)}}\,
			\strace\Bigl(f\(\sqrt{4s(1-s)}\,\^1\Xsl_{s,t,1}\)\Bigr)
			\,ds\\
	&=(2\pi i)\hochhalb{1-N^B}\,\lim_{t\to\infty}
		\int_{s\in[0,1]}{1\over\sqrt{4s(1-s)}}\,
			\,\strace\biggl(f\Bigl(\sqrt{4s(1-s)}
				\,\Xsl_{t\over4s(1-s)}\Bigr)\biggr)\,ds\\
	&=\lim_{t\to\infty}\int_{s\in[0,1]}
		\biggl({4s(1-s)\over2\pi i}\biggr)\hochhalb{N^B-1}
			\,\strace\Bigl(f\(\Xsl_t\)\Bigr)\,ds
	=\cho\(\nabla^H,g^H_V\)
\endalign$$
as in the proof of \MVBTorsionThm.
On the other hand,
we have
$$\multline
	(2\pi i)\hochhalb{1-N^B}\int_{s\in[0,1]}{1\over2}\,
			\strace_V\Bigl(e^{-\^3\Asl^2|_{v=0\atop T=1}}\Bigr)\\
	=(2\pi i)\hochhalb{1-N^B}
		\lim_{v\to 0}\int_{s\in[0,1]}{1\over\sqrt{4s(1-s)}}\,
			\strace_V\Bigl(f\(\sqrt{s(1-s)}\,\omega^V\)\Bigr)\,ds
	=\cho\(\nabla^V,g^V\)\;.
\endmultline$$

We still have to show that the remaining terms on the right hand side
of~\ChBLdTFormel\ vanish.
By \AslSquareRem,
the restriction of~$\strace_V\bigl(e^{-\^1\Asl^2}\bigr)$ to~$s=0$
and~$s=1$ is of degree~$0$ and hence does not contain~$dt$,
so
	$$\int_{t\in[1,\infty)}
			{1\over2}\,\strace_V\Bigl(e^{-\^1\Asl^2|_{T=1}}\Bigr)
			\biggr|_{s=0}^1
	=0\;.$$
By~\ZweiAslChFormel,
the integrand~$\strace_V\bigl(e^{-\^2\Asl^2}\bigr)$
involves no term that contains~$du$ but not~$ds$,
so
	$$\int_{u\in[0,1]}
			{1\over2}\,\strace_V\Bigl(e^{-\^2\Asl^2|_{T=1}}\Bigr)
			\biggr|_{s=0}^1
	=0\;.$$
Finally,
we have
$$\multline
	\int_{v\in[0,1]}{1\over2}
		\,\strace_V\Bigl(e^{-\^3\Asl^2|_{s=0\atop T=1}}\Bigr)\\
	=\int_{v\in[0,1]}{1\over\sqrt{4v(1-v)}}
		\,\strace_V\biggl(f\Bigl(\sqrt{4v(1-v)}
			\,\(\Asl'|_{t={1/4}}-\nabla^V\)\Bigr)\biggr)\,dv
	=0\;,
\endmultline$$
because~$\Asl'-\nabla^V$ takes values
in a nilpotent subalgebra of~$\End V$.
Our theorem follows from the equations above.
\qed\enddemo

\ChernBLThm\ shows that~$T(\nabla^V,A',g^V)$ behaves as expected
even without the existence of a Morse endomorphism~$h^V$.
Proceeding as in the proof of \MorseTorsionCor,
we can therefore draw the following conclusion.

\Corollary\ChernBLCor.
Let~$(V,\nabla^V)\to B$ be a flat $\Z$-graded vector bundle
with a flat superconnection~$A'$ such that~$A'-\nabla^V\in\Omega^*(B;\End V)$
takes values in a nilpotent subalgebra of~$\End V$,
which may vary over~$B$.
Assume that both~$V$ and~$H=H^*(V,a'_0)$ carry parallel metrics,
then the form
	$$T\(\nabla^V,A',g^V\)+\chslo\(\nabla^H,g^H,g^H_V\)$$
is even, closed and real,
and its cohomology class is independent of the choice of parallel metrics
in degree~$\ge2$.


\Remark\TChRem
Let us state some properties of \ChtorDef\ above.
\roster
\item
The formula for~$T\(\nabla^V,A',g^V\)$
makes essential use of the Chern normalisation.
Integrating over two-dimensional domains
instead of one-dimensional contours as in \MVBTorsionDef\
allows a much larger choice of superconnections to use in the definition.
In fact, the integrals in \ChtorDef\
do not arise from applying the Chern normalisation
operator~$\int_0^1\(s(1-s)\)^{N^B}\,ds$ to a one-dimensional
contour integral.
\item
We have to include the flat reference connection~$\nabla^V$
in the notation~$T\(\nabla^V,A',g^V\)$
because~$\nabla^V$ is used
for the construction of the superconnection~$\^3\Asl$
in~\DreiAslFormel\ above.
\item
We had to assume that~$A'-\nabla^V$ is an inhomogeneous differential form
with values in a nilpotent subalgebra of~$\End V$,
which may vary over~$B$.
In fact, we could define~$T\(\nabla^V,A',g^V\)$ without this assumption.
However,
we would then be unable to prove that
	$$dT\(\nabla^V,A',g^V\)
	=\cho\(\nabla^V,g^V\)-\cho\(\nabla^H,g^H_V\)\;.$$
By the way,
we do not have to demand that the nilpotent subalgebra  mentioned above
can locally be chosen parallel.
This is because by flatness of~$A'$,
	$$\bigl[\nabla^V,a'_k\bigr]=-a'_0a'_{k+1}-\dots-a'_{k+1}a'_0$$
is again an element of the subalgebra.
%\item
%The definition of~$T(\nabla^V,A',g^V)$ looks complicated
%because it is pieced together from three contributions.
%Note however that the restriction of~$\Asl$ to the hyperplanes~$s=0$
%and~$s=1$ is flat.
%This allows us to deform the domain of integration
%\?weiter?
%Thus, our formula for~$T(\nabla^V,A',g^V)$
%is much more flexible than the original formula for~$T_f(A',g^V,h^V)$.
\endroster
\endremark


Let from now on~$T\(\nabla^V,\Cal A',g^{\Cal V}\)$ denote the form
constructed in \ChTorsionThm,
%then we can use~$T\(\nabla^V,\Cal A',g^{\Cal V}\)$
which can be used
to define a universal torsion class on the acyclic Whitehead space.
We assume that~$G$ is a subgroup of a unitary group,
so that the bundle~$\Cal V\to\Wh^h(R,G)$
carries a canonical parallel metric~$g^{\Cal V}$.

\Definition\TChRGDef
Define~$T(R,G)\in H^{\even}\bigl(\Wh^h(R,G),\R\bigr)$
to be the class represented by the cocycle
which assigns to every simplex~$\Delta$ in~$\cWh^{\diff}(R,G)$
the integral
	$$\int_\Delta T\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)\;.$$
\enddefinition

Then~$T(R,G)\dg0$ equals the fibre-wise Franz-Reidemeister torsion
of the acyclic complex~$(\Cal V,a_0)$.
Another possibility would have been to find an adapted
endomorphism~$h^{\Cal V}$ over~$\bigl|\cWh^{\diff}(R,G)\bigr|$.
Here the difficulty is that one has to make sure that \MVBDef~(3)
is satisfied.
This is possible if~$h^{\Cal V}$ is chosen suitably
and the tautological superconnection~$\Cal A'$
on~$\Cal V\to\bigl|\cWh^{\diff}(R,G)\bigr|$
is pulled back to the interior of each simplex
using cut-off functions as in \PatchSuperconnectionDefinition.
Of course, by \ChTorsionThm,
the class obtained this way would be cohomologous
to the class~$T(R,G)$ defined in \TChRGDef\ above.

Let~$(V,A',h^V)$ be a family Thom-Smale complex over~$B$
such that~$\nabla^V$ is unitarily flat and fibre-wise acyclic.
By \WhFunctorProp\ and \WhSimpUniversalRem,
there exists a ``classifying functor''
$\Xi=\Xi^\diff_{p,h,F}\colon S\to\cWh^{\diff,h}(R,G)$,
inducing a classifying map~$\xi\colon B\to\Wh^h(R,G)$ up to homotopy,
such that
	$$(V,\nabla^V,A',g^V)
	\cong\xi^*\(\Cal V,\nabla^{\Cal V},\Cal A',g^{\Cal V}\)\;.$$
%		\Mand
%	(H,\nabla^H,g^H)\cong\xi^*\(\Cal H,\nabla^{\Cal H},g^H\)

\Corollary\ChTorsionCor.
Let~$S$ be a simplicial complex on~$B$
and let~$\Xi\colon S\to\cWh^{\diff,h}(R,G)$ be a simplicial map.
Let~$(V,\nabla^V,A',g^V)=\Xi^*\(\Cal V,\nabla^{\Cal V},\Cal A',g^{\Cal V}\)$,
then
	$$T\(\nabla^V,A',g^V\)%+\chslo\(\nabla^H,g^H,g^H_V\)
	=\abs\Xi^*T(R,G)
	\quad\in H^{\even}(\abs S,\R)\;.\tag1$$
\parr
In particular,
if~$p\colon M\to B$ is a proper submersion
with a fibrewise Morse-function~$h\colon M\to\R$,
if~$(F,\nabla^F,g^F)\to M$ is a unitarily flat
and fibrewise acyclic vector bundle,
and if~$\xi\colon B\to\Wh(R,G)$ is constructed as Chapter~4 of~\IBuch,
cf.\ \WhSimpUniversalRem,
then
	$$T(M/B,F,h)=\xi^*T(R,G)\dg{\ge2}\;.\tag2$$


\Proof
Claim~(1) is an immediate consequence of \ChTorsionThm\ and \TChRGDef.
By \IgusaFunctorThm,
Igusa's functor~$\Xi$ is homotopic
to the functor constructed in \ComplexKapitel.
Thus, (2) follows from \MorseTorsionDef\ and~(1).
\qed\enddemo


\Abschnitt\SpecSeqSubsection Higher torsion and filtrations

If there is a filtration of the vector bundle~$V$
that is compatible with~$\nabla^V$ and~$A'$,
and preserves the local splitting of~$V$ of \MVBDef,
then we show that the higher torsion~$T\(\nabla^V,A',g^V\)$
can be computed using higher torsions associated
to a spectral sequence.
Such filtered complexes arise in the following situations.
\roster
\item
In the case that the fibre~$X$ of~$p\colon N\to B$ is itself fibred
by~$p=p_2\circ p_1$, with~$p_1\colon N\to M$ and~$p_2\colon M\to B$,
the filtration of~$\Omega^*(M/B;F)$ by relative horizontal degree
gives a family of Leray spectral sequences over~$B$.
The analytic torsion of such a multifibration was treated by Ma in~\Ma.
Here,
we recover Ma's result in the case that both fibrations admit
fibre-wise Morse functions,
if the fibre-wise Morse function on~$M$ with respect to~$h_2$
admits a Smale gradient field.
\item
If the bundle~$p\colon M\to B$ admits a fibre-wise function such
that~$0$ is a regular value on each fibre of~$p$,
one has a decomposition~$M=M^+\cup M^-$ with~$M^-=h^{-1}(-\infty,0]$
and~$M^+=h^{-1}[0,\infty)$.
Under certain assumptions on~$H$,
Igusa proves in~\IBuch, Chapter~5 that the higher Franz-Reidemeister torsion
of~$M\to B$ equals the sum of the torsions of~$M^+\to B$ and~$M^-\to B$
already on the level of maps from~$B$ to~$\Wh(R,G)$.
If~$h$ can be chosen to be Morse on every fibre of~$p$,
we obtain a gluing formula for~$T_{\ch}(M/B;F,h)$.
A gluing formula for the infinitesimal equivariant analytic torsion
in a similar situation was proved by Bunke in~\BuZwei.
\item
Suppose that~$F\to M$ and~$H=H^*(M/B;F)$ admit parallel metrics,
then we get a filtered complex on~$\widehat V=V\oplus H\to B$
which is fibre-wise acyclic.
Here, the spectral sequence degenerates,
and~$T_{\ch}(M/B;F,h)
=T_{\ch}\bigl(\nabla^{\hat V},\widehat A',g^{\hat V}\bigr)$.
In other words,
the torsion class on the acyclic Whitehead space determines
the torsion class on the unitary Whitehead spaces
that will be defined in \UniKapitel.
\endroster
We will prove a finite dimensional analogue of Ma's results in~\Ma,
Section~3.2,
where the fibre-wise Leray spectral sequence of a family of submersions is
considered.

Suppose that the vector bundle~$(V,\nabla^V,A')$ admits a metric~$g^V$
and a decreasing graded filtration
	$$F^0V^j=V\supset\cdots\supset F^{k_0}V^j=0
	\Formel\GlobFiltDef$$
that is compatible with~$\nabla^V$ and~$A'=\nabla^V+a'$,
and put~$F^pV=V$ for~$k\le 0$ and~$F^pV=0$ for~$p\ge k_0$.
Then let~$(E_k,d'_k)\to B$ be the spectral sequence
associated to the filtered complex~$(V,a'_0)$.
There is an associated filtration
	$$F^0H=H\supset\cdots\supset F^{k_0}H=0
		\Mtext{with}
	F^pH=\(\ker(a'_0)\cap F^pV\)\bigm/\(\im(a'_0)\cap F^pV\)\;.
	\Formel\SpecSeqHFiltration$$
The following result has been proved by Ma in~\Ma\
in an infinite-dimensional setting.

\Proposition\SpecSecBundleProp.
For~$k=0$,
let the operator~$d'_0$ on~$E_0^p=F^pV/F^{p+1}V$ be induced by~$a'_0$.
There are a flat connection~$\nabla^{E_0}$ and a flat superconnection~$D'_0$
of total degree~$1$ on~$E_0$,
induced by~$\nabla^V$ and~$A'$,
such that~$D'_0$ starts with~$d'_0$ in degree~$0$,
and~$D'_0-\nabla^{E_0}$ is a differential form with values
in some nilpotent subalgebra of~$\End E_0$ which may vary over~$B$.
\parr
For~$k\ge 0$,
we have a vector bundle~$E_{k+1}=\(H^*(E_k,d'_k)\)\to B$.
If~$\nabla^{E_{k+1}}$ denotes the Gau\ss-Manin connection
induced by~$D'_k$
then~$\nabla^{E_{k+1}}$ is flat,
and the fibre-wise differential~$d'_k$ is parallel
with respect to~$\nabla^{E_{k+1}}$.
In particular,
the superconnection~$D'_{k+1}$
defined by~$D'_{k+1}=\nabla^{E_{k+1}}+d'_{k+1}$
is flat and of total degree~$1$.
\parr
The spectral sequence~$E_k$ converges
to~$E_\infty=E_{k_0}$ with~$E_\infty^{p,q}=F^pH^q/F^{p+1}H^q$
and~$\nabla^{E_\infty}$ is the connection induced by~$\nabla^H$.
\qed

Let~$g^V$ be a metric on~$V$
and identify~$E_0^p$ with~$(F^{p+1}V)^\perp\cap F_pV$.
This allows us to identify
	$$V\cong E_0=\bigoplus_pE_0^p\;,\Formel\SpecSeqSplitting$$
and~$g^V$ induces a metric~$g^{E_0}$ on~$E_0$.
We inductively define metrics on~$E_k$ as follows.
Assume that~$g^{E_k}$ is already defined,
and let~$d_k^{\prime*}$ denote the adjoint of~$d'_k$ with respect to~$g^{E_k}$.
Then we can identify~$E_{k+1}=H(E_k,d'_k)$
with the $(d'_k+d_k^{\prime*})$-harmonic elements of~$E_k$.
This induces a metric~$g^{E_{k+1}}$ on~$E_{k+1}$.

By assumption,
the spectral sequence converges to~$E_{k_0+1}=E_\infty\to B$,
and we obtain a metric~$g^{E_\infty}=g^{\botsmash{E_{\scriptstyle k_0+1}}}$.
A metric~$g^H$ on~$H$ allows us to identify~$E_\infty^{p+q}$
with~$F^pH^{p+q}\cap\(F^{p+1}H^{p+q}\)^\perp$ similar as above.

\Definition\FiltSplitDef
Let~$(V,\nabla^V)$ be a flat vector bundle
with a $\nabla^V$-parallel filtration~$F^*V$.
A metric~$g^V$ is called {\em adapted to\/}~$F^*V$
if the subbundles~$(F^{p+1}V)^\perp\cap F_pV$ are also $\nabla^V$-parallel.
\enddefinition

\Remark\FiltSplitRem
We collect some examples and properties of adapted metrics.
\roster
\item
Any $\nabla^V$-parallel metric is adapted to~$F^*V$.
\item
Suppose that~$(V,A',h^V)$ is a family Thom-Smale complex.
If each subbundle~$F^p$ can locally be written as the direct sum
of some of the bundles~$V^j_\alpha$ of \MVBDef,
then any metric~$g^V$ adapted to~$(V,A',h^V)$ in the sense of \MorseMetricDef\
is in particular adapted to~$F^*V$.
This will be the case in all the applications we have in mind.
\item
Suppose~$g^V$ is adapted to~$F^*V$.
Then the adjoint~$\nabla^{V,*}$ of~$\nabla^V$ with respect to~$g^V$
also respects the filtration~$F^*V$ and the decomposition~\SpecSeqSplitting,
and we have
	$$\cho\(\nabla^V,g^V\)
	=\sum_{p,q}(-1)^{p+q}\,\cho\Bigl(\nabla^{E_0^p},g^{E_0^p}\Bigr)
	=\cho\(\nabla^{E_0},g^{E_0}\)\;.$$
Similarly, if~$g^V_0$ and~$g^V_1$ are two adapted metrics
that induce the same splitting~\SpecSeqSplitting,
then~$g^V_t=(1-t)\,g^V_0+t\,g^V_1$ is adapted for all~$t$,
so modulo exact forms,
	$$\chslo\(\nabla^V,g^V_0,g^V_1\)
	=\chslo\(\nabla^{E_0},g^{E_0}_0,g^{E_0}_1\)\;.$$
\item
The bundle~$H\to B$ is filtered by~\SpecSeqHFiltration,
but even if~$g^V$ is adapted to~$F^*V$,
it is not clear that there is a metric~$g^H$ adapted to~$F^*H$.
However,
if we assume that~$g^H$ is adapted,
we can use~$g^H$ to identify
	$$H^{p,q}:=F^pH^{p+q}\cap\(F^{p+1}H^{p+q}\)^\perp
	\cong F^pH^{p+q}\bigm/F^{p+1}H^{p+q}
	=E_\infty^{p,q}$$
as flat vector bundles with respect to~$\nabla^H$ and~$\nabla^{E_\infty}$,
and to define
	$$\chslo\(\nabla^H,g^H,g^{E_\infty}\)
	=\sum_{p,q}(-1)^{p+q}\,\chslo\(\nabla^{E_\infty^{p,q}}
		,g^{H^{p,q}},g^{E^{p,q}_\infty}\)\;.$$
\endroster
\endremark

We can now state the main result of this subsection,
which we prove below.

\Theorem\SpecSeqThm.
Suppose that~$g^V$ is adapted to the filtration~$F^*V$,
and that~$g^H$ is adapted to the induced filtration on~$H$.
Then the torsion of~$V$ can be computed as
$$\multline
	T\(\nabla^V,A',g^V\)+\chslo\(\nabla^H,g^H,g^H_V\)\\
	=T\(\nabla^{E_0},D'_0,g^{E_0}\)
		+\sum_{k=1}^{k_0}T^{\roman{BL}}\(D'_k,g^{E_k}\)
		+\chslo\(\nabla^{E_\infty},g^H,g^{E_\infty}\)\;.
\endmultline$$

\Remark\SSMaRemark
Let~$N@>p_1>>M@>p_2>>B$ be a family of proper submersions as initem~(1)
at the beginning of this subsection.
Assume that~$N$ carries a fibre-wise Morse function~$h_1$
with respect to~$\pi_1$,
and that~$M$ carries a fibre-wise Morse function~$h_2$.
Over each compact subset of~$B$,
$h=\eps,h_1+h_2\circ\pi_1$ becomes a fibre-wise Morse function
with respect to~$\pi=\pi_2\circ\pi_1$ for~$\eps$ small enough.
The family-Thom-Smale complex of~$h$ carries a natural filtration
by horizontal degree with respect to~$\pi_1$
if~$h_2$ admits a fibre-wise Morse-Smale gradient field.
In this case,
the filtration gives rise to the Leray spectral sequence of~$N_b\to M_b$
for each~$b\in B$.

In this situation,
\SpecSeqThm\ implies that \MainTheorem\ is compatible
with Ma's formula for the analytic torsion of iterated fibre bundles in~\Ma.
We leave the details to the interested reader.
The necessity for the existence of a Morse-Smale gradient field for~$h_2$
is reflected by the fact that already the $E_1$-term in the Leray spectral
of the filtered complex~$V$ associated with~$h$
carries a superconnection of the form~$\nabla^{E_1}+d'_1$.

Note that if~$h_2$ does not admit a fibre-wise Morse-Smale gradient field,
we still get local filtrations over subsets of~$B$ by the values of~$h_2$.
However,
the type of the sectral sequence changes as~$b\in B$ varies,
and we are situation similar to the one describe in \ComplexKapitel.
\endremark



\Abschnitt\SSProofAbs A proof of Theorem 7.37

If~$g^V$ is adapted,
we may define a $\nabla^V$-parallel number operator~$N^F$ on~$V$,
which acts on~$F^p\cap(F^{p+1})^\perp$ by~$p$.
We define a new metric~$g^V_r$ on~$V$ by
	$$g^V_r=g^V\,r^{N^F}=\bigoplus_pr^p\,g^V|_{E_0^p}\;.
	\Formel\SpecSeqGvrFormel$$
Let~$g^{E_k}_r$ denote the metrics on the bundles~$E_k\to B$
induced by~$g^V_r$ as above.
Because we have identified~$E_{k+1}^{p,q}$ with a subbundle of~$E_k^{p,q}$
in order to define~$g^{E_{k+1}}$,
it follows by induction that
	$$g^{E_k^{p,q}}_r=g^{E_k^{p,q}}\,r^{N^F}=r^p\,g^{E_k^{p,q}}$$
for all~$k\ge 0$, including~$k=\infty$.

Clearly,
the statement of our theorem is compatible with variation of~$g^V$
by metrics that preserve the splitting~\SpecSeqSplitting\ of~$V$.
We may therefore prove the theorem by replacing~$g^V$ with~$g^V_r$
for some small~$r>0$,
and considering the limit~$r\to 0$.
Note that modulo exact forms,
	$$\chslo\(\nabla^V,g^V,g^V_r\)
	={1\over2}\,\int_1^r\,\strace_V\(N^F\)\,{dr\over r}
	={\log r\over 2}\,\strace_V\(N^F\)$$
because~$N^F$ is parallel with respect to~$\nabla^V$ and~$\nabla^{V,*}$.
We still denote the induced number operators on~$E_k$ by~$N^F$.
A careful count shows that
$$\align
	\strace_{E_k}\(N^F\)
%	&=\sum_{p,q}p\,(-1)^{p+q}\,\Bigl(E_k^{p,q}-\dim\(\im d_k^{\prime p,q}\)
%		-\dim\(\im d_k^{\prime p-k,q+k-1}\)\Bigr)\\
%	&=\strace_{E_k}\(N^F\)-k\,\sum_{p,q}(-1)^{p+q}\,\dim\(\im d_k^{\prime p,q}\)\\
	&=\strace_{E_{k+1}}\(N^F\)+k\,\(\chi'(E_{k+1})-\chi'(E_k)\)\;,
\endalign$$
so

	$$\chslo\(\nabla^V,g^V,g^V_r\)
	={\log r\over 2}
		\,\biggl(\strace_{E_\infty}(N^F)
			+\sum_{k=1}^\infty\(\chi'(E_k)-\chi'(E_\infty)\)
		\biggr)\;.
	\Formel\SpecSeqChsloVFormel$$

%Using~$g^H$,
%we identify~$H$ and~$E_\infty=F^*H/F^{*+1}H$.
%Setting~$g^H_r=g^Hr^{N^F}$,
%we obtain
%	$$\chslo\(\nabla^H,g^H,g^H_r\)={\log r\over2}\,\strace_H\(N^F\)
%	=\chslo\(\nabla^{E_\infty},g^{E_\infty},g^{E_\infty}_r\)$$
%and
%	$$\chslo\(\nabla^V,g^V,g^V_r\)-\chslo\(\nabla^H,g^H,g^H_r\)
%	={\log r\over 2}\,\sum_{k=1}^\infty\(\chi'(E_k)-\chi'(E_\infty)\)\;.$$
%By the variation formula for~$T\(\nabla^V,A',g_r\)$ and the equation above,
%we find that
%$$\multline
%	T\(\nabla^V,A',g^V\)+\chslo\(\nabla^H,g^H,g^H_V\)\\
%	=\lim_{r\to0}\biggl(T\(\nabla^V,A',g^V_r\)
%		+\chslo\(\nabla^H,g^H_r,g^H_{V,r}\)
%		-{\log r\over 2}\,\sum_{k=1}^\infty
%			\(\chi'(E_k)-\chi'(E_\infty)\)\biggr)\;.
%\endmultline\tag\FormelNummer\SpecSeqLimesFormelEins$$


If~$A''$ denotes the adjoint of~$A'$ with respect to~$g^V$,
then the adjoint of~$A'$ with respect to~$g^V_r$ is given by
	$$A''_r=r^{-N^F}\,A''\,r^{N^F}\;.$$
Conjugating both~$A'$ and~$A''_r$ with~$r\hochhalb{N^F}$ gives
new superconnections
	$$\Asl'_r=r\hochhalb{N^F}\,A'\,r\hochmhalb{N^F}
		\Mand
	\Asl''_r=r\hochmhalb{N^F}\,A''\,r\hochhalb{N^F}\;.$$
Let
	$$\Asl_r={1\over2}\,\(\Asl'_r+\Asl''_r\)
		\Mand
	\Xsl_r={1\over2}\,\(\Asl''_r-\Asl'_r\)\;.$$
We note that under the identification of~\SpecSeqSplitting,
	$$\lim_{r\to 0}\Asl'_r=D'_0
		\Mand
	\lim_{r\to 0}\Asl''_r=D''_0\;,
	\Formel\SpecSeqZeroLimit$$
where~$D''_0$
is the adjoint of~$D'_0$ with respect to~$g^{E_0}$,
and thus also with respect to all~$g^{E_0}_r$ for all~$r>0$.
If we define superconnections~$\^1\Asl_r$, $\^2\Asl_r$ and~$\^3\Asl_r$
on~$V$
and~$\^1\Dsl_0$, $\^2\Dsl_0$ and~$\^3\Dsl_0$ on~$E_0$
as in~\EinsAslFormel, \ZweiAslFormel, \DreiAslFormel\ at~$T=1$,
then similarly,
	$$\lim_{r\to 0}\^j\Asl_r=\^j\Dsl_0
	\Formel\SpecSeqZeroLimitZwei$$
for~$j=1$, $2$, $3$.


Equation~\SpecSeqZeroLimitZwei\ immediately clarifies the following behaviour
of two of the three integrals in \ChtorDef.
We have
	$$\lim_{r\to0}\int_{(s,u)\in[0,1]^2}
		{1\over2}\,\strace_V\Bigl(e^{-\^2\Asl^2_r}\Bigr)
	=\int_{(s,u)\in[0,1]^2}
		{1\over2}\,\strace_V\Bigl(e^{-\^2\Dsl^2_0}\Bigr)\;,
	\Formel\SpecSeqIntZweiLimes$$
and
$$\split
	\kern4em&\kern-4em
	\lim_{r\to0}\int_{(s,v)\in[0,1]^2}\biggl(
		{1\over2}\,\strace_V\Bigl(e^{-\^3\Asl^2}\Bigr)
			-\(\chi'(V)-\chi'(H)\)
			\,\Bigl(f'\({\sqrt{-v}/2}\)-1\Bigr)
			\,{dv\,ds\over2v}\biggr)\\
	&=\int_{(s,v)\in[0,1]^2}\biggl(
		{1\over2}\,\strace_V\Bigl(e^{-\^3\Dsl^2_0}\Bigr)
			-\(\chi'(E_0)-\chi'(E_1)\)
			\,\Bigl(f'\({\sqrt{-v}/2}\)-1\Bigr)
			\,{dv\,ds\over2v}\biggr)\\
	&\qquad
		-\(\chi'(E_1)-\chi'(E_\infty)\)\int_0^1
			\Bigl(f'\({\sqrt{-v}/2}\)-1\Bigr)
			\,{dv\over2v}\;.
\endsplit\Formel\SpecSeqIntDreiLimes$$
In particular,
in the limit we recover two of the three terms in the definition
of~$T\(\nabla^{E_0},D'_0,g^{E_0}\)$
up to a simple correction term.

If we write
	$$\alpha_{r,t}=\biggl(
		\strace_V\Bigl(N^V\,f'\(\Xsl_{r,t}\)\Bigr)
		-\chi'(H)\biggr)\,{dt\over2t}\;,$$
then by its construction in \ChernTorsionSubsection,
the remaining integral takes the form
$$\multline
	\int_{(s,t)\in[0,1]\times[1,\infty)}\biggl(
		{1\over2}\,\strace_V\Bigl(e^{-\^1\Asl_r^2}\Bigr)
		-\chi'(H)\,{ds\,dt\over2t}
		-\(\chi'(V)-\chi'(H)\)\,f'\(\sqrt{-t}/2\)
			\,{ds\,dt\over2t}\biggr)\\
	=\int_0^1\(4s(1-s)\)\hochhalb{N^B}\,ds
		\int_1^\infty\alpha_{r,t}
	-\(\chi'(E_0)-\chi'(E_\infty)\)\int_1^\infty f'\(\sqrt{-t}/2\)
			\,{dt\over2t}\;.
\endmultline\tag\FormelNummer\SpecSeqIntEinsFormel$$
We will split the integral over~$\alpha_{r,t}$
into finitely many subintervals,
which we will rescale differently.

Similar as in~\MM, \Dai\ or~\Ma,
we have to control the ``small eigenvalues''
of~$\tilde a_{0,r}={1\over2}\,\(\tilde a'_{0,r}+\tilde a''_{0,r}\)$
as~$r\to 0$.
Let us write
$$\alignat3
	a'_j&=\sum_ka^{\prime(k)}_j&
		&\Mtext{with}&
	a^{\prime(k)}_j|_{E_0^{p,q}}
		&\colon E_0^{p,q}\to E_0^{p+k,q+1-k}\;,\\
	a''_j&=\sum_ka^{\prime\prime(k)}_j&
		&\Mtext{with}&
	a^{\prime\prime(k)}_j|_{E_0^{p,q}}
		&\colon E_0^{p,q}\to E_0^{p-k,q+k-1}\;,\\
			\Land
	x_j&=\sum_kx\nr k_j&
		&\Mtext{with}&
	x\nr k_j&=\(a^{\prime\prime(k)}_j-a^{\prime(k)}_j\)\bigm/2
\endalignat$$
for all~$p$, $q$.
Then the components~$\tilde a_{j,r}$
and~$\tilde x_{j,r}$ of~$\Asl_r-\nabla^{E_k,u}$ and~$\Xsl_r$
in~$\Omega^j(B;\End V)$ are given by
	$$\tilde a_{j,r}=\sum_kr\hochhalb k\,a\nr k_j
		\Mand
	\tilde x_{j,r}=\sum_kr\hochhalb k\,x\nr k_j\;.
		\Formel\SpecSeqAslrNullFormel$$

We define a superconnection~$D_k={1\over2}\,(D'_k+D''_k)$ on~$E_k$,
and let~$d_k={1\over2}\,(d'_k+d''_k)$ denote its component of degree~$0$.
Similarly,
we construct fibrewise operators
	$$Y_k={1\over2}\,(D''_k-D'_k)=y_k+{\omega_k\over2}
		\quad\in\quad\End E_k$$
for~$k\ge 1$ with~$y_k={1\over2}\,(d''_k-d'_k)$ 
and~$\omega_k=\nabla^{E_k,*}-\nabla^{E_k}$.
We put
	$$Y_{k,t}=\sqrt t\,y_k+{\omega^{E_k}\over2}\;.$$

\Definition\SpecSeqUepsDef
Set
	$$U_{\eps,k}
	=\bigl\{\,z\in\C\bigm|d\(z,\Spec(y_k)\)>\eps\,\bigr\}\;.$$
\enddefinition

Let~$\Pi_k\in\End E_0$ denote the orthogonal projection onto~$E_k$,
regarded as a subset of~$V\cong E_0$.
The evaluation of~\SpecSeqIntEinsFormel\
is based on a quantitative version of a result of Bismut-Berthomieu
and Ma in our finite-dimensional setting.
We will prove the following theorem in \BBAbs.

\Theorem\SpSSmEvThm{(\BB, Theorem~6.5; \Ma, Theorem~2.2)}.
There exist~$r_0>0$, $c>0$ and~$C>0$
such that for all~$r\in(0,r_0)$, $k\ge 1$
and all~$\lambda\in U_{\eps,k}$
with~$\max(\abs\lambda,\eps^{-1})<c\,r\hochmhalb1$,
one has
	$$\Bigl\|\Bigl(\lambda-r\hochmhalb k\,\tilde x_{0,r}\Bigr)^{-1}
		-\Pi_k\,(\lambda-y_k)^{-1}\,\Pi_k\Bigr\|
	\le C\,\sqrt{r}\,\eps^{-1}
		\,\(1+\max(\abs\lambda,\eps^{-1})\)\;,$$
and for~$r\in(0,r_0)$, $k=0$ and~$\lambda\in U_{\eps,0}$
with~$\eps^{-1}<c\,r\hochmhalb1$,
	$$\bigl\|\bigl(\lambda-\tilde x_{0,r}\bigr)^{-1}
		-\(\lambda-\tilde x_{0,0}\)^{-1}\bigr\|
	\le C\,\sqrt{r}\,\eps^{-1}
		\,\(1+\eps^{-1}\)\;.$$

Let us fix constants~$0<c_1<c_2<\infty$ such that for all~$k$,
	$$\Spec(Y_k)\setminus\{0\}\subset i[c_1,c_2]\cup -i[c_1,c_2]\;.$$
Let~$\Gamma_{r,t}=\Gamma_{r,t}^1\cup\Gamma_{r,t}^2\cup\Gamma_{r,t}^3\subset\C$
be the contour depicted in \SpecSeqContour.

\Figur(-2,-4)(2,4)\psset{unit=0.07\hsize}
	\psline{->}(-2.05,0)(2.1,0)
	\psline{->}(0,-4.05)(0,4.1)
	{\psset{linewidth=0.2pt,linestyle=dashed}
	 \psline(0.5,-4)(0.5,4)
	 \psline(-0.5,-4)(-0.5,4)}
	{\psset{linewidth=0.2pt}
	 \psline(-0.2,1.5)(-0.7,1.5)
	 \psline(-0.2,2)(-0.7,2)
	 \psline(-0.2,3.5)(-0.7,3.5)
	 \psline(-0.2,-1.5)(-0.7,-1.5)
	 \psline(-0.2,-2)(-0.7,-2)
	 \psline(-0.2,-3.5)(-0.7,-3.5)}
	{\psset{linewidth=1.5pt}
	 \psarc(0,0){0.5}{0}{360}
	 \psarc(0,1.5){0.5}{180}{360}
	 \psline(0.5,1.5)(0.5,2)
	 \psline(-0.5,1.5)(-0.5,2)
	 \psarc(0,2){0.5}{0}{180}
	 \psarc(0,3.5){0.5}{180}{360}
	 \psline(0.5,3.5)(0.5,4)
	 \psline(-0.5,3.5)(-0.5,4)
	 \psarc(0,-2){0.5}{180}{360}
	 \psline(0.5,-1.5)(0.5,-2)
	 \psline(-0.5,-1.5)(-0.5,-2)
	 \psarc(0,-1.5){0.5}{0}{180}
	 \psarc(0,-3.5){0.5}{0}{180}
	 \psline(0.5,-3.5)(0.5,-4)
	 \psline(-0.5,-3.5)(-0.5,-4)}
	\psline(-0.1,1.5)(0.1,1.5)
	\psline(-0.1,2)(0.1,2)
	\psline(-0.1,3.5)(0.1,3.5)
	\psline(-0.1,-1.5)(0.1,-1.5)
	\psline(-0.1,-2)(0.1,-2)
	\psline(-0.1,-3.5)(0.1,-3.5)
	\uput[225](-0.5,0){$\scriptstyle-{\eps\over\sqrt t}$}
	\uput[315]( 0,0){$\scriptstyle 0$}
	\uput[315]( 0.5,0){$\scriptstyle {\eps\over\sqrt t}$}
	\uput[180](-0.7,1.5){$\scriptstyle ic_1$}
	\uput[180](-0.7,2){$\scriptstyle ic_2$}
	\uput[180](-0.7,3.5){$\scriptstyle {ic_1\over 2\sqrt r}$}
	\uput[180](-0.7,-1.5){$\scriptstyle-ic_1$}
	\uput[180](-0.7,-2){$\scriptstyle-ic_2$}
	\uput[180](-0.7,-3.5){$\scriptstyle-{ic_1\over 2\sqrt r}$}
	\uput[0](0.5,3.5){$\scriptstyle\Gamma_{r,t}^3$}
	\uput[0](0.5,1.75){$\scriptstyle\Gamma_{r,t}^2$}
	\uput[45](0.5,0){$\scriptstyle\Gamma_{r,t}^1$}
	\uput[0](0.5,-1.75){$\scriptstyle\Gamma_{r,t}^2$}
	\uput[0](0.5,-3.5){$\scriptstyle\Gamma_{r,t}^3$}
\EndFigur\SpecSeqContour
{The contour~$\Gamma_{r,t}=\Gamma_{r,t}^1
\cup\Gamma_{r,t}^2\cup\Gamma_{r,t}^3\subset\C$}

We split the integral~\SpecSeqIntEinsFormel\ as
$$\align
	\int_1^\infty\alpha_{r,t}
	&=\int_1^{r\hochmhalb1}\alpha_{r,t}
		+\sum_{k=1}^{k_0-1}\int_{r^{-k+{1\over2}}}^{r^{-k-{1\over2}}}
			\alpha_{r,t}
		+\int_{r^{-k_0+{1\over2}}}^\infty
			\alpha_{r,t}\\
	&=\int_1^{r\hochmhalb1}\alpha_{r,t}
		+\sum_{k=1}^{k_0-1}\int_{r^{1\over2}}^{r^{-{1\over2}}}
			\alpha_{r,r^{-k}t}
		+\int_{r^{1\over2}}^\infty
			\alpha_{r,r^{-k_0}t}\;.
\endalign$$
For~$k\ge0$, $r\in(0,r_0)$ with~$r_0$ sufficiently small
and for~$t\in\bigl(t^{r\over2},t^{-{r\over2}}\bigr)$,
we consider
$$\align
	\alpha'_{k,r,t}
	&:=\biggl(\strace_V\Bigl(N^V\,f'\(\widetilde X_{r,r^{-k}t}\)\Bigr)
		-\chi'(E_{k+1})\biggr)\,{dt\over 2t}\\
	&=\Biggl(\strace_V\biggl(N^V\,f'\Bigl(
		t\hochhalb1\,r\hochmhalb k\,\tilde x_{0,r}
		+\tilde x_{1,r}+t\hochmhalb1\,r\hochhalb k\,\tilde x_{2,r}
			+\dots\Bigr)\biggr)
		-\chi'(E_{k+1})\Biggr)\,{dt\over 2t}\;,
\endalign$$
such that
	$$\int_{r^{1\over2}}^{r^{-{1\over2}}}\alpha_{r,r^{-k}t}
	=\int_{r^{1\over2}}^{r^{-{1\over2}}}\alpha'_{k,r,t}
		-\(\chi'(E_{k+1})-\chi'(E_\infty)\)\,{\log r\over2}\;.
	\Formel\SSAlphaXIntFormel$$

We will treat the integrals over~$t\in\bigl[r\hochhalb1,1\bigr]$
and~$t\in\bigr[1,r\hochmhalb1\bigr]$ separately.
For~$t\in\bigr[1,r\hochmhalb1\bigr]$ and~$k\ge 0$,
we write
$$\multline
%	\kern2em&\kern-2em
	f'\(\widetilde X_{r,r^{-k}t}\)
%	&={1\over2\pi i}\int_{\Gamma^1_{r,t}\cup\Gamma^2_{r,t}
%				\cup\Gamma^3_{r,t}}
%		{f'(\sqrt t\,\lambda)\,d\lambda
%		\over\lambda-r\hochmhalb k\,\tilde x_{0,r}
%			-t\hochmhalb1\,\tilde x_{1,r}
%			-t\hochmhalb1\,O\(r\hochhalb kt\hochmhalb1\)}\\
	={1\over2\pi i}\int_{\Gamma^1_{r,t}\cup\Gamma^2_{r,t}
				\cup\Gamma^3_{r,t}}
		\,{f'(\sqrt t\,\lambda)
			\over\lambda-r\hochmhalb k\,\tilde x_{0,r}}\\
		\,\sum_{j=0}^\infty
			\Biggl(t\hochmhalb1\,\biggl(\tilde x_{1,r}
				+O\Bigl(r\hochhalb kt\hochmhalb1\Bigr)\biggr)
			\,{1\over\lambda-r\hochmhalb k\,\tilde x_{0,r}}
			\Biggr)^j\,d\lambda\;.
\endmultline$$
Let us note that because~$\Gamma_{r,t}$ depends explicitly on~$t$,
the real part of~$\sqrt t\,\lambda$ remains bounded by~$\eps$,
so that~$f\bigl(\sqrt t\,\lambda\bigr)$ remains uniformly bounded, too.

For~$\lambda\in\Gamma^1_{r,t}$ and~$k\ge1$,
\SpSSmEvThm\ implies that
	$$\Biggl\|{f'(\sqrt t\,\lambda)
			\over\lambda-r\hochmhalb k\,\tilde x_{0,r}}
		\,\sum_{j=0}^\infty
			\Biggl(t\hochmhalb1\,\biggl(\tilde x_{1,r}
				+O\Bigl(r\hochhalb kt\hochmhalb1\Bigr)\biggr)
			\,{1\over\lambda-r\hochmhalb k\,\tilde x_{0,r}}
			\Biggr)^j
		-{f'(\sqrt t\,\lambda)\over\lambda-t\hochmhalb1Y_{k,t}}\Biggr\|
	\le C\,\sqrt r\,t\;.$$
Integrating over the contour~$\Gamma^1_{r,t}$
of length~$O\bigl(t\hochmhalb1\bigr)$
gives
	$$\Biggl\|\int_{\Gamma^1_{r,t}}\Biggl(
		{f'(\sqrt t\,\lambda)\,d\lambda
			\over\lambda-t\hochmhalb1\,\widetilde X_{r,r^{-k}t}}
		-{f'(\sqrt t\,\lambda)\,d\lambda
			\over\lambda-t\hochmhalb1Y_{k,t}}\Biggr)\Biggr\|
	\le C\,\sqrt{rt}\;.$$
For~$t<r\hochmhalb1$, we have~$\sqrt r<t^{-1}$,
so the integral
over~$t\in\bigl[1,r\hochmhalb1\bigr]$ of the difference above converges.
By~\BL,
we already know that
	$$\int_1^\infty\Biggl(\int_{\Gamma^1_{r,t}}
			\strace_V\biggl(N^V\,{f'(\sqrt t\,\lambda)\,d\lambda
				\over\lambda-t\hochmhalb1Y_{k,t}}\biggr)
		-\chi'(E_{k+1})\Biggr)\,{dt\over 2t}$$
converges,
so we have uniform convergence for the contribution from~$\Gamma^1_{r,t}$
to~\SSAlphaXIntFormel\ for~$t\in\bigl[1,r\hochmhalb1\bigr]$.

The reasoning for the integral over~$\Gamma^2_{r,t}$ is similar,
but we use that~$\abs{\Im\lambda}>c>0$,
so~$f\bigl(\sqrt t\,\lambda\bigr)$ decays rapidly as~$t\to\infty$
uniformly on~$\Gamma^2_{r,t}$.
Finally the integral over~$\Gamma^3_{r,t}$ vanishes as~$r\to 0$
because~$\abs{\Im\lambda}>r\hochmhalb 1 c$.
This shows that
	$$\lim_{r\to 0}\int_1^{r\hochmhalb1}\alpha'_{k,r,t}
	=\int_1^\infty
		\Bigl(\strace\(N^V\,f'(Y_{k,t})\)
			-\chi'\(E_{k+1}\)\Bigr)\,{dt\over 2t}\;.$$

For~$k=0$,
we similarly recover the remaining contribution
to~$T(\nabla^{E_0},D'_0,g^{E_0})$
up to divergencies and correction terms,
because
$$\split
	\kern4em&\kern-4em
	\lim_{r\to 0}\biggl(\int_1^{r\hochmhalb1}\alpha_{r,t}
		+{\log r\over4}\,\(\chi'(E_1)-\chi'(E_\infty)\)\biggr)\\
	&=\int_1^\infty\biggl(
		\strace_V\Bigl(N^{E_0}\,
			f'\(\Xsl_{0,t}\)\Bigr)
		-\chi'(E_1)%\\
%	&\kern6em
		-\(\chi'(E_0)-\chi'(E_1)\)\,f'\({\sqrt{-t}/2}\)
			\biggr)\,{dt\over2t}\\
	&\qquad
		+\(\chi'(E_0)-\chi'(E_1)\)
			\,\int_1^\infty f'\({\sqrt{-t}/2}\)
			\,{dt\over2t}\;.
\endsplit\Formel\SpecSeqIntEinsNullLimes$$


We use the contour~$\Gamma_{r,1}$
for all~$t\in\bigl[r\hochhalb1,1\bigr]$ and~$k\ge1$.
Using \SpSSmEvThm\ and the results of~\BL,
we can again prove uniform convergence,
and we find that
$$\multline
	\lim_{r\to 0}\int_{r\hochhalb1}^1
		\biggl(\strace\Bigl(N^V\,f'\(\widetilde X_{r,r^{-k}t}\)\Bigr)
			-\chi'\(E_k\)\,f'\(\sqrt{-t}/2\)\biggr)\,{dt\over 2t}\\
	=\int_0^1
		\biggl(\strace\Bigl(N^V\,f'\(Y_{k,t}\)\Bigr)
			-\chi'\(E_k\)\,f'\(\sqrt{-t}/2\)\biggr)
		\,{dt\over 2t}\;.
\endmultline$$

Thus for~$k\ge 1$,
$$\split
	\kern4em&\kern-4em
	\lim_{r\to 0}\biggl(\int_{r\hochhalb1}^{r\hochmhalb1}\alpha_{r,r^{-k}t}
		+{\log r\over4}\,\(\chi'(E_k)-\chi'(E_{k+1})\)
		+{\log r\over2}\,\(\chi'(E_{k+1})-\chi'(E_\infty)\)\biggr)\\
	&=\int_0^\infty\Bigl(
		\strace_V\bigl(N^{E_k}
			\,f'(Y_{k,t})\bigr)
		-\chi'(E_{k+1})%\\
%	&\kern6em
		-\(\chi'(E_k)-\chi'(E_{k+1})\)\,f'\({\sqrt{-t}/2}\bigr)
			\Bigr)\,{dt\over2t}\\
	&\qquad
		+\(\chi'(E_k)-\chi'(E_{k+1})\)
			\,\biggl(\int_1^\infty
				\,f'\({\sqrt{-t}/2}\)\,{dt\over2t}%\\
%	&\qquad
		+\int_0^1\Bigl(f'\({\sqrt{-t}/2}\)-1\Bigr)
			\,{dt\over2t}\biggr)\;.
\endsplit\Formel\SpecSeqIntEinsEinsLimes$$
Modulo divergencies and correction terms in degree~$0$,
we find~$T^{\roman{BL}}\(D'_k,g^{E_k}\)$ in the limit.

Finally,
we regard the last contribution
	$$\int_{\sqrt r}^\infty\alpha_{r,r^{-k_0}t}\;.$$
Because~$E_{k_0}=E_\infty$,
we know that
	$$\Spec\Bigl(r\hochmhalb{k_0}\tilde x_{0,r}\Bigr)
	\subset\{0\}\cup i\biggl(-\infty,-r\hochmhalb1{c_1\over2}\biggr)
		\cup i\biggl(r\hochmhalb1{c_1\over2},\infty\biggr)\;.$$
For~$\lambda\in\Gamma^1_{r,t}$,
we therefore have
	$$\Bigl\|\Bigl(\lambda-r\hochmhalb{k_0}\tilde x_{0,r}\Bigr)^{-1}
		-\Pi_{\ker\tilde x_{0,r}}\,\lambda^{-1}
			\,\Pi_{\ker\tilde x_{0,r}}\Bigr\|
	\le C\,\sqrt r$$
and
	$$\Bigl\|\Bigl(\lambda-r\hochmhalb{k_0}\Xsl_{r,t}\Bigr)^{-1}
		-\Pi_{\ker\tilde x_{0,r}}\,\lambda^{-1}
			\,\Pi_{\ker\tilde x_{0,r}}\Bigr\|
	\le C\,\sqrt{r/t}\;.$$
Since only integrals of~$f'\bigl(\sqrt t\,\lambda\bigr)
\,\bigl(\lambda-r\hochmhalb{k_0}\Xsl_{r,t}\bigr)^{-1}$
over~$\Gamma^1_{r,t}$ and~$\Gamma^3_{r,t}$ contribute
to~$f'\bigl(\Xsl_{r,r\hochmhalb{k_0}t}\bigr)$,
we conclude that
	$$\lim_{r\to 0}\int_{r\hochhalb1}^\infty
			\alpha_{r,r^{-k_0}t}
	=0\;.\Formel\SpecSeqIntEinsZweiLimes$$

Combining~\SpecSeqIntZweiLimes, \SpecSeqIntDreiLimes,
\SpecSeqIntEinsNullLimes, \SpecSeqIntEinsEinsLimes\
and~\SpecSeqIntEinsZweiLimes,
we can compute the asymptotic behaviour of~$T\(\nabla^V,A',g^V_r\)$ by
$$\multline
%	\kern4em&\kern-4em
	\lim_{r\to 0}\Biggl(T\(\nabla^V,A',g^V_r\)
		-{\log r\over2}\,\sum_{k=1}^{k_0-1}
			\(\chi(E_k)-\chi(E_\infty)\)\Biggr)\\
	=T\(\nabla^{E_0},D'_0,g^{E_0}\)
		+\sum_{k=1}^{k_0-1}T^{\roman{BL}}\(D'_k,g^{E_k}\)\;.
\endmultline\tag\FormelNummer\SpecSecIntLimes$$
Moreover,
we can extend both summations over~$k$ to infinity.

It remains to study the variation of~$\chslo\(\nabla^H,g^H,g^H_{V,r}\)$
as~$r\to 0$.
Identifying~$H$ and~$E_\infty$ using~$g^H$,
we find
	$$\chslo\(\nabla^H,g^H,g^H_{V,r}\)
	=\chslo\(\nabla^H,g^H,g^{E_\infty}\)
		+\chslo\(\nabla^{E_\infty},g^{E_\infty},g^{E_\infty}_r\)
		+\chslo\(\nabla^H,g^{E_\infty}_r,g^H_{V,r}\)\;.
	\Formel\SSChsloHDecomp$$
Clearly
	$$\chslo\(\nabla^{E_\infty},g^{E_\infty},g^{E_\infty}_r\)
	={\log r\over2}\,\strace_{E_\infty}(N^F)\;.
	\Formel\SpecSeqChsloExFormel$$

If we put~$H_r=\ker a_{0,r}$ and~$\widetilde H=\ker\tilde a_{0,r}$
and let~$\nabla^{H_r}$ and~$\nabla^{\tilde H_r}$ denote the connections
induced by~$A'$ and~$\Asl'_r$,
then
$$\split
	\chslo\(\nabla^H,g^{E_\infty}_r,g^H_{V,r}\)
	&=\chslo\Bigl(\nabla^{H_r}
		,\(r^{N^F\over2}\,\Pi_{k_0}\,r^{-{N^F\over2}}|_{H_r}\)^*g^V_r
		,g^V_r|_{H_r}\Bigr)\\
	&=\chslo\(\nabla^{\tilde H_r},\(\Pi_{k_0}|_{\tilde H_r}\)^*g^V
		,g^V|_{\tilde H_r}\)
\endsplit$$
because~$E_{k_0}=E_\infty$.
On the other hand,
let~$\Pi_{\tilde H_r}$ denote the $g^V$-orthogonal projection
onto~$\widetilde H_r$.
Then
	$$\lim_{r\to 0}\Pi_{\tilde H_r}
	={1\over2\pi i}\,\lim_{r\to0}\int_{\Gamma^1_{r,t}}
		{d\lambda\over\lambda-r\hochmhalb{k_0}\tilde a_{0,r}}
	=\Pi_{k_0}$$
in all~$C^k$-norms,
so
	$$\lim_{r\to 0}\chslo\(\nabla^H,g^{E_\infty}_r,g^H_{V,r}\)
	=\lim_{r\to 0}\chslo\(\nabla^{\tilde H_r}
			,\(\Pi_{k_0}|_{\tilde H_r}\)^*g^V,g^V|_{\tilde H_r}\)
	=0\;.$$
By~\SpecSeqChsloExFormel\ and~\SSChsloHDecomp,
	$$\lim_{r\to 0}\biggl(\chslo\(\nabla^H,g^H,g^H_{V,r}\)
		-{\log r\over 2}\,\strace_{E_\infty}(N^F)\biggr)
	=\chslo\(\nabla^H,g^H,g^{E_\infty}\)\;.
	\Formel\SpecSeqChsloHFormel$$

Now it follows from~\SpecSeqChsloVFormel,
\SpecSecIntLimes\ and~ \SpecSeqChsloHFormel\ that
$$\multline
	T\(\nabla^V,A',g^V\)
		+\chslo\(\nabla^H,g^H,g^H_V\)\\
\split
	&=\lim_{r\to 0}\Bigl(T\(\nabla^V,A',g^V_r\)
		+\chslo\(\nabla^V,g^V_r,g^V\)
		+\chslo\(\nabla^H,g^H,g^H_{V,r}\)\Bigr)\\
	&=T\(\nabla^{E_0},D'_0,g^{E_0}\)
		+\sum_{k=1}^\infty T^{\roman{BL}}\(D'_k,g^{E_k}\)
		+\chslo\(\nabla^H,g^H,g^{E_\infty}\)\;.
\endsplit\endmultline$$
This completes the proof of \SpecSeqThm.
\qed


\Abschnitt\BBAbs A proof of the Berthomieu-Bismut convergence results

This chapter should be considered an appendix containing the proofs
of some results that are analogous to results proved in \BB.
In particular,
we prove \SpSSmEvThm\ for~$k\ge 1$,
however regarding the family of self-adjoint operators~$\tilde a_{0,r}$
instead of~$\tilde x_{0,r}$.
The case~$k=0$ is an easy exercise that we leave to the reader.

\Proposition\BBSechsEins{(\BB, Theorem~6.1)}.
For each~$r\ge1$ and each~$k\ge 1$,
there are inclusions~$E_{k,r}^{p,q}\subset E_0^{p,q}$
such that~$E_{k,r}^{p,q}
=\ker\(d'_{k-1,r}+d''_{k-1,r}\)\subset E^{p,q}_{k-1,r}$,
and~$E_{k,r}^{p,q}$ is given by
$$\multline
	E_{k,r}^{p,q}
	=\biggl\{\,v_0\in E_0^{p,q}\biggm|
			\text{there exist~$v_1$, \dots, $v_{k-1}$ such that}\\
		\sum_{i=0}^j\tilde a_{0,r}\nr i v_{j-i}=0
			\text{ for~$j=0$, \dots, }k-1\,\biggr\}\;.
\endmultline\tag 1$$
Let~$\Pi_{k,r}\colon E_0\to E_{k,r}$ denote the orthogonal projection
with respect to~$g$.
The operator~$d_{k,r}={1\over2}\,\(d'_{k,r}+d''_{k,r}\)$ acts on~$E_{k,r}$ by
	$$d_{k,r}v_0
	=\Pi_{k,r}\sum_{i=1}^k\tilde a_{0,r}\nr iv_{j-i}\;.\tag 2$$
There exists a linear map~$\phy_k\colon E_{k,T}\to V^{k-1}$
such that for~$v_0\in E_{k,r}$ and~$(v_{1},\dots,v_{k-1})=\phy_{k}(v_0)$,
one has
	$$\sum_{i=0}^j\tilde a_{0,r}^{\prime(i)}\,r\hochhalb{j-i}\,v_{j-i}=0
		\Rtext{ for~$j=0$, \dots, }k-1\;.\tag 3$$

\Proof The proof is a simple adaptation of the proof given in~\BB.
\qed\enddemo

It follows from this theorem that for all~$k$
both the subspace~$E_{k,r}\subset E_0$
and the operator
	$$r\hochmhalb k\,d_{k,r}\in\End\(E_{k,r}\)$$
are independent of~$r$.
Later on,
we put
	$$E_k=E_{k,r}\;,\qquad
	\Pi_k=\Pi_{k,r}\Mand
	d_k=r\hochmhalb k\,d_{k,r}\in\End\(E_k\)\;.$$

If~$\phy_k(v_0)=(v_1,\dots,v_{k-1})$,
we define~$\phy_{k,r}$ by putting
	$$\phy_{k,r}(v_0)
	=\Bigl(r\hochhalb1v_1,\dots,r\hochhalb{k-1}v_{k-1}\Bigr)\;.$$

Next,
we study the resolvent of~$\tilde a_{0,r}$.
We begin with an approximation.
Because~$(d'_{0,r})^2=(d''_{0,r})^2=0$,
the operators~$\rho\,d'_{0,r}+\bar\rho\,d''_{0,r}$
have the same square for all~$\rho\in S^1\subset\C$
and thus the same spectrum.
For this reason,
	$$iU_{\eps,k}
	=\bigl\{\,z\in\C\bigm|d\(z,\Spec(d_k)\)>\eps\,\bigr\}\;.$$

\Proposition\BBSechsZwei{(\BB, Theorem~6.2)}.
For each~$k\ge 0$ and each~$\lambda\in iU_{\eps,k}$,
there exists a linear map
	$$\psi_{k,r,\lambda}\colon V\to V^{k+1}
		\Mtext{with}
	v\mapsto(v_{0,r},\dots,v_{k,r})$$
such that
	$$v_{0,r}=(\lambda-d_k)^{-1}\Pi_kv\in E_k\tag1$$
and
$$\alignat2
	\sum_{i=0}^j\tilde a_{0,r}\nr{j-i}v_{i,r}&=0
		&&\Rtext{for~$j=0$, \dots, $k-1$, and}\tag2\\
	r\hochmhalb k\sum_{i=0}^k\tilde a_{0,r}\nr{k-i}v_{i,r}
		&=\lambda v_{0,r}-v\;.\tag3
\endalignat$$
Moreover there exists a constant~$C>0$ such that
	$$\abs{v_{i,r}}\le C\,r\hochhalb{i}\,\eps^{-1}\abs v
		\Rtext{for~$i=1$, \dots, }k\;.\tag4$$

\Proof
As in the proof of \BBSechsEins,
we first solve the equations~(2) and
	$$\Pi_{k-l,r}\biggl(\lambda v_{0,r}
		-\sum_{i=0}^k\tilde a_{0,r}\nr{k-i}v_{i,r}\biggr)
	=\Pi_{k-l,r}v\tag2'$$
with~$v_{k,r}=0$ by induction over~$l=0$, \dots, $k-1$,
and finally give a solution for~$l=k$,
where~(3') is equivalent to~(3).

For~$l=0$,
we have to find~$v_{0,r}\in E_k$ with
	$$\Bigl(\lambda-r\hochmhalb k\,d_{k,r}\Bigr)\,v_{0,r}
	=\(\lambda-d_k\)\,v_{0,r}
	=\Pi_{k,r}v\;,$$
which gives~(1).
We put~$(v_{1,r},\dots,v_{k-1,r})=\phy_{k,r}(v_0)$.
Then by \BBSechsEins,
equations~(2) and~(3') hold for~$l=0$,
and there exists a constant~$C$ such that
	$$\abs{v_{0,r}}\le C\,\(\eps\,(1+\abs\lambda)\)^{-1}\,\abs v
		\Mand
	\abs{v_{i,r}}
	\le C\,r\hochhalb{i}\,\eps^{-1}\,\abs v
		\Rtext{for~$i=1$, \dots, $k-1$}\;.$$

In the following steps,
we have to choose~$w_0\in E_{k-l}$ such that
	$$d_{k-l}w_0
	=r\hochhalb l\Pi_{k-l,r}\biggl(\lambda v_{0,r}-v
		-r\hochmhalb k\,\sum_{i=0}^{k-1}\tilde a_{0,r}\nr{k-i}v_{i,r}\biggr)
	\quad\in\quad E^{\prime\perp}_{k-l+1}\subset E_{k-l}\;.$$
The right hand side is still of order~$C\,r\hochhalb l\,\eps^{-1}\abs v$.
We have~$\bigl|d_{k-l}^{-1}|_{E_{k-l+1}^{\prime\perp}}\bigr|\le C'$,
so that~$w_0$ is of order~$C\,C'\,r\hochhalb l\,\,\eps^{-1}\abs v$.
For definiteness,
we may demand that~$s_l+w_0\in E_{k-l+1}^{\prime\perp}$
without changing the estimate above.
We take~$(w_1,\dots,w_{l-1})=\phy_{k-l,r}(w_0)$
and replace~$(v_{0,r},\dots,v_{k-1,r})$ by
	$$\(v_{0,r},\dots,v_{l-1,r},v_{l,r}+w_0,\dots,v_{k-1,r}+w_{l-1}\)\;.$$
For this new tupel,
(2) and~(3') hold for~$l$ and~(4) holds with a new constant~$C$.

Finally for~$k=l$,
it remains to determine~$v_{k,r}\in E_{1}^{\prime\perp}$ with
	$$\tilde a_0\nr0\,v_{k,r}
	=r\hochhalb k\,\(\lambda v_{0,r}-v\)
		-\sum_{i=0}^{k-1}\tilde a_{0,r}\nr{k-i}v_{i,r}
	\quad\in\quad E_{1}^{\prime\perp}\;.$$
This implies that~(2) and~(3) hold,
and~(4) holds with a new constant~$C$,
so we are done.
\qed\enddemo

If we put
	$$\bar\psi_{k,r,\lambda}=v_{0,r}+\dots+v_{k,r}\;,$$
then \BBSechsZwei\ immediately implies
	$$\Bigl(\lambda-r\hochmhalb k\,\tilde a_{0,r}\Bigr)\,\bar\psi_{k,r,\lambda}(v)
	=v+\lambda\,\sum_{i=1}^kv_{i,k}
		-r\hochmhalb k\,\sum_{j=k+1}^\infty\sum_{i=0}^k
			\tilde a_{0,r}\nr{j-i}\,v_{i,r}\;.
	\Formel\BBSechsVier$$
Note that the first sum is finite because our filtration~$F^pV$
has finite length.
As in~\BB,
this gives the main result on the asymptotics of the operator~$\tilde a_{0,r}$.


\Theorem\BBSechsFuenf{(\BB, Theorem~6.5)}.
There exist~$r_0>0$, $c>0$ and~$C>0$
such that for all~$k\ge 1$, all~$r\in(0,r_0)$
and all~$\lambda\in iU_{\eps,k}$
with~$\max(\abs\lambda,\eps^{-1})<c\,r\hochmhalb1$,
one has
	$$\Bigl\|\Bigl(\lambda-r\hochmhalb k\,\tilde a_{0,r}\Bigr)^{-1}
		-\Pi_k\,(\lambda-d_k)^{-1}\,\Pi_k\Bigr\|
	\le C\,\sqrt{r}\,\eps^{-1}
		\,\(1+\max(\abs\lambda,\eps^{-1})\)\;.\quad\qed$$

For~$k=0$, we may replace~$\max(\abs\lambda,\eps^{-1})$
simply by~$\eps^{-1}$ in the theorem.
\SpSSmEvThm\ follows from \BBSechsFuenf\ by replacing~$\tilde a_{0,r}$
by~$\tilde x_{0,r}$ etc.

\Proof
Write~\BBSechsVier\ as
	$$\Bigl(\lambda-r\hochmhalb k\,\tilde a_{0,r}\Bigr)\,\bar\psi_{k,r,\lambda}(v)
	=v+R_{k,r,\lambda}(v)\;,$$
then \BBSechsZwei\ implies that the operator norms of~$\psi_{k,r,\lambda}$
and~$R_{k,r,\lambda}(v)$ satisfy the estimates
	$$\norm{\psi_{k,r,\lambda}-\Pi_k\,(\lambda-d_k)^{-1}\,\Pi_k}
		=O\(\sqrt r/\eps\)
		\Mand
	\norm{R_{k,r,\lambda}}=O\(\sqrt r\,\max(\abs\lambda,\eps^{-1})\)\;.$$
The ``max'' comes from the fact that the~$\eps^{-1}$ in \BBSechsZwei\ becomes
relevant only if~$\abs\lambda$ is small
(for large~$\abs\lambda$, we may may choose a large value of~$\eps$).
Let us fix~$c>0$ and~$r_0>0$ suitably small and let us assume that~$r<r_0$
and~$\max(\abs\lambda,\eps^{-1})\le c\,r\hochmhalb1$.
Then~\BBSechsVier\ gives us a series converging to
the resolvent of~$r\hochhalb k\,\tilde a_{0,r}$,
and we estimate
$$\split
	\Bigl(\lambda-r\hochmhalb k\,\tilde a_{0,r}\Bigr)^{-1}
	&=\sum_{k=0}^\infty\psi_{k,r,\lambda}\,\(-R_{k,r,\lambda}\)^k\\
	&=\Bigl(\Pi_k\,(\lambda-d_k)^{-1}\,\Pi_k
			+O\(\sqrt r/\eps\)\Bigr)
		\,\Bigl(1+O\(\sqrt r\,\max(\abs\lambda,\eps^{-1})\)\Bigr)\;.
	\quad\qed
\endsplit$$
\enddemo

As in~\BB,
this implies that for~$r$ sufficiently small,
the operator~$\tilde a_0$ has eigenvalues of order~$r\hochhalb k$
that correspond precisely to the eigenvalues of~$d_k$.
The condition on~$\abs\lambda$ guarantees
that~$\lambda$ stays away from the eigenvalues
of~$r\hochmhalb k \tilde a_{0,r}$ corresponding
to those of~$r\hochhalb{k'-k}\,d_{k'}$ with~$k'<k$
when taking the resolvent.
Similarly,
the restriction to~$\eps^{-1}$ guarantees
that~$\lambda$ avoids the eigenvalues of~$r\hochmhalb k \tilde a_{0,r}$
corresponding to those of~$r\hochhalb{k'-k}\,d_{k'}$ with~$k'>k$.

\enddocument


==> framing.tex <==
%auto-ignore
\input morse2.def

\document

\Kapitel\FramingKapitel={10}
The Framing Principle and a higher Cheeger-M\"uller Theorem

We use Igusa's framing principle to establish \TeilZweiTheorem\
for fibre bundles with fibrewise Morse functions
and fibrewise acyclic flat vector bundles.
We establish a cohomological analogue of Igusa's splitting lemma.
Using this result and \TeilZweiTheorem,
we prove the generalised second statement of~\ApplThm.
Throughout this chapter,
we will use the complex matrix ring~$R=\Cal M(\C)=\lim_{\to}\Cal M_r(\C)$
and the unitary group~$G=U=\lim_{\to}U(r)$.
We let~$\tau=\tau\(\Cal M(\C),U\)$ denote the universal unitary torsion
class on~$\Wh^u\(\Cal M(\C),U\)$.

\Abschnitt\FramedSubsection Igusa's framed function theorem

We recall the definition of generalised fibre-wise Morse functions
and framed functions
in the sense of~\Iframed.
Framed functions always exist by Igusa's framed function theorem.
By~\IBuch, Chapter~4,
each generalised Morse function gives rise
to a classifying map~$\xi_{p,h,F}\colon B\to\Wh\(\Cal M(\C),U\)$.
Suppose that this map lifts to~$\Wh^u\(\Cal M(\C),U\)$,
then we can define a torsion class~$\tau(M/B;F,h)$
by pulling back the universal torsion class~$\tau\(\Cal M(\C),U\)\in\Wh^u\(\Cal M(\C),U\)$.

Let~$p\colon M\to B$ be a fibre-bundle with $n$-dimensional fibres,
and let~$h\colon M\to\R$ be a smooth function.
We denote by~$C\subset M$ the set of fibre-wise singularities,
i.e., the zero set of~$dh|_{TX}$.
The subset of fibre-wise Morse singularities will be denoted~$C\Morse$.

\Definition\SingTypeDef
%A point~$p\in C_b\subset X_b$
%is called a {\em fibre-wise Morse singularity of index\/}~$k$,
%if there are coordinates~$x_0$, \dots, $x_n$ of~$X_b$ around~$p$
%such that
%	$$f(q)
%	=f(p)-{x_1^2\over2}-\dots-{x_k^2\over2}
%		+{x_{k+1}^2\over2}+\dots+{x_n^2\over2}\tag1$$
%for all~$q\in X_b$ near~$p$.
%
A point~$p\in C_b\subset X_b$
is called a {\em birth-death singularity of index\/}~$k$
if there is a neighbourhood~$V\subset B$ of~$b$,
a function~$f_0\colon V\to\R$,
a local trivialisation of~$p^{-1}V\cong B\times X$
with coordinates~$b_1$, \dots, $b_m$ of~$V$
and~$x_0$, \dots, $x_n$ on~$X_b$ of~$X$ around~$p$,
such that
	$$f(q)
	=f_0(b_1,\dots,b_m)-{x_1^2\over2}-\dots-{x_k^2\over2}
		+{x_{k+1}^2\over2}+\dots+{x_{n-1}^2\over2}
		+{x_n^3\over3}-b_1\,x_n$$
for all~$q\in p^{-1}V$ near~$p$.
Let~$C\cubical\subset C$ denote the set
of all birth-death singularities
of~$h$.
\enddefinition

\Definition\GenMorseFnDef
Let~$M\to B$ be a fibre bundle with fibre-wise boundary~$\del M=M_0\cup M_1$.
A {\em generalised fibre-wise Morse function\/}
is a function~$h\colon M\to[0,1]$ such that~$0$ and~$1$ are regular values
with~$h^{-1}(i)=M_i$ for~$i\in\{0,1\}$,
and such that~$h$ has only fibre-wise Morse singularities
and birth-death singularities,
i.e., a function with the property that~$C=C\Morse\cup C\cubical$.
\enddefinition

Then as in \IBuch, Chapter~4,
each proper generalised fibre-wise Morse function~$h\colon M\to\R$
with finitely many singularities on each fibre
gives rise to a classifying map~$\xi_{p,h,F}\colon B\to\Wh\(\Cal M(\C),U\)$
up to homotopy.
Assume that~$g^F$ and~$g^H$ are parallel metrics on~$F\to M$ and~$H\to B$,
then we also have a lift~$\xi_{p,h,F}^u\colon B\to\Wh^u\(\Cal M(\C),U\)$.
We can now combine Igusa's definition of the higher Franz-Reidemeister torsion
with our definition of Morse torsion forms.


\Definition\GenMorseTorsionDef
Assume that~$F\to M$ and~$H\to B$ admit parallel metrics.
%~$g^F$ and~$g^H$.
Let~$h\colon M\to\R$ be a proper generalised fibre-wise Morse function
with finitely many fibre-wise singularities on each fibre,
and let~$\xi_{p,h,F}^u\colon B\to\Wh^u\(\Cal M(\C),U\)$
be the corresponding classifying map.
Then we define the {\em higher Franz-Reidemeister torsion\/}
	$$\tau(M/B;F,h)=\(\xi_{p,h,F}^u\)^*\tau\(\Cal M(\C),U\)\dg{\ge2}
		\quad\in H^{\even,\ge2}(B;\R)\;.$$
\enddefinition

We could also define~$\tau(M/B;F,h)\dg0=\tau(M/B;F,h,g^V,g^H)\dg0$
in degree~$0$,
however,
it seems better to work with Franz-Reidemeister metrics instead.

Note that~$\tau(M/B;F,h)$ still depends on the choice of~$h$.
To define an independent invariant of~$p\colon M\to B$
and~$F\to M$ only,
Igusa further restricts the space of admissible functions~$h$.
Up to homotopy,
there is a unique splitting of the vertical tangent bundle
	$$TX|_{C\Morse}=T^s\Morse X\oplus T^u\Morse X\to C\Morse$$
such that~$d^2h$ is positive (negative) definit on~$T^s\Morse X$
($T^u\Morse X$).
There is a similar splitting
	$$TX|_{C\cubical}
	=T^s\cubical X\oplus T^u\cubical X\oplus T^c\cubical X
	\to C\cubical\;,$$
where~$T^c\cubical=\ker(d^2h)\cong\R\times C\cubical$
is the unique cubic direction
corresponding to the coordinate~$x_n$ in \SingTypeDef,
which is oriented by the third derivative of~$h$.
%If we fix a vertical Riemannian metric~$g\TX$,
%we may choose the coordinates in~\SingTypeDef~(1) and~(2)
%such that the space~$T^uX$ spanned by~$x_0$, \dots, $x_k$ is
%orthogonal to the space spanned by~$x_{k+1}$, \dots, $x_n$.
%This way,
%we obtain unique unstable tangent bundles~$T^u\Morse X\to C\Morse$
%and~$T^u\cubical X\to C\cubical$.
%Note that the isomorphism type of~$T^u\Morse X\to C\Morse$
%and~$T^u\cubical X\to C\cubical$ does not depend on the choice of~$g\TX$.

In order to obtain a somewhat unique generalised fibre-wise Morse function,
Igusa considers functions~$h$
such that the bundles~$T^u\Morse X$ and~$T^u\cubical X$
admit compatible trivialisations.
In the coordinates of \SingTypeDef,
let
	$$C^\pm
	=\bigl\{\,q\bigm|x_1(q)=\dots=x_{n-1}(q)=0\text{, $b_1>0$, and }
			x_n=\pm\sqrt{b_1}\,\bigr\}\subset C\Morse\;,$$
then~$C^+$ has fibre-wise Morse index~$k+1$ and~$C^-$ has index~$k$.

\Definition\FramedFnDef
Trivialisations~$T^u\Morse X\cong C\Morse\times\R^{\ind_h}$
and~$T^u\cubical X\cong C\cubical\times\R^{\ind_h}$
are called {\em compatible\/}
if near each point~$p\in C\cubical$,
the trivialisation of~$T^u\cubical X$ near~$p$ extends continously
to the trivialisation of~$T^u\Morse X|_{C^-}$,
and the trivialisation of~$T^u\cubical X\oplus T^c\cubical X$
extends continously
to the trivialisation of~$T^u\Morse X|_{C^+}$.
A {\em framed function\/} is a generalised fibre-wise Morse function on~$M$
with fixed compatible trivialisations of~$T^u\Morse X$ and~$T^u\cubical X$.
\enddefinition

With this definition,
we can now state a version of Igusa's framed function theorem (\Iframed).

\Fact\IframedThm(Framed Function Theorem).
Let~$p\colon M\to B$ be a fibre bundle
with fibre-wise boundary~$\del M=M_0\cup M_1$.
If~$\dim M\ge 2\,\dim B$,
then~$M$ carries a framed function~$h\colon M\to[0,1]$ with~$h^{-1}(i)=M_i$
for~$i=0$, $1$.
Let~$p\colon M\to B$ be a fibre bundle with~$\dim M> 2\,\dim B$,
and let~$h_0$, $h_1\colon M\to\R$ be framed functions as above,
then there exists a framed function~$h$ on~$M\times[0,1]\to B\times[0,1]$
with the same properties
that restricts to the given functions and framings on~$M\times\{0,1\}$.

This implies that for~$\dim M> 2\,\dim B$,
the homotopy class of~$\xi_{p,h,F}\colon B\to\Wh\(\Cal M(\C),U\)$
is independent of the choice of the framed function~$h$.
Of course,
the same holds for any lift~$\xi^u_{p,h,F}\colon B\to\Wh^u\(\Cal M(\C),U\)$
with respect to a fixed parallel metric on~$H$.
Igusa defines a unique higher Franz-Reidemeister torsion
for unitarily flat bundles~$F\to M$ such that~$H^*(M/B;F)\to B$ is trivial,
cf.~\IBuch, Theorem~5.7.5.
We extend Igusa's definition as follows.

\Definition\IgusaTorsionDef
Assume that~$M\to B$ is a smooth fibre bundle with~$\dim M> 2\,\dim B$,
with compact fibres,
and with fibre-wise boundary~$\del M=M_0\cup M_1\to B$.
Assume that~$0$ and~$1$
are regular values of the framed function~$h\colon M\to[0,1]$
with~$h^{-1}(0)=M_0$ and~$h^{-1}(1)=M_1$.
Let~$F\to M$ be a unitarily flat vector bundle
such that the fibre-wise cohomology~$H^*(M/B;F)\to B$ admits a parallel
metric.
Let~$\xi^u_{p,h,F}\colon B\to\Wh^u\(\Cal M(\C),U\)$ be the classifying map
defined by these data.
Then the {\em unitary higher Franz-Reidemeister torsion\/} of~$(M,M_0)\to B$
and~$F$
is defined as
	$$\tau(M/B,M_0/B;F)
	=\tau(M/B,M_0/B;F,h)
	=\(\xi^u_{p,h,F}\)^*\tau;.$$

If~$M\to B$ is as above but with~$\dim M\le 2\,\dim B$,
then for~$N$ sufficiently large,
define
	$$\tau(M/B,M_0/B;F)
	=\tau\(M\times\R P^{2N}/B\,,\;M_0\times\R P^{2N}/B\,;\;F\)\;.$$
\enddefinition

It is an easy consequence of \IframedThm\ that~$\tau$ is well-defined.
For suppose that~$h_0\colon M\times\R P^{2N_0}\to[0,1]$
and~$h_1\colon M\times\R P^{2N_1}\to[0,1]$
are framed functions with fibre-wise compact sublevels
and finitely many critical points on each fibre.
Then both functions can be extended to framed functions
on~$\bar h_{0,1}\colon M\times\R P^{2N_0}\times\R P^{2N_1}\to[0,1]$
by adding a fixed Morse function~$\R P^{2N_i}\to(-\eps,\eps)$
on the additional factor~$\R^{N_1}$ or~$\R^{N_0}$
and correcting near the boundary components.
The functions~$\bar h_0$ and~$\bar h_1$
can then be joined by a framed function on the bundle
	$$\(M\times\R P^{2N_0}\times\R P^{2N_1}\)
	\times[0,1]\to B\times[0,1]\;.$$
Thus, we clearly have
$$\multline
	\tau\((M\times\R P^{N_0},M_0\times\R P^{N_0})/B;F,h_0\)\\
\split
	&=\tau\((M\times\R P^{2N_0}\times\R P^{2N_1},
		M_0\times\R P^{2N_0}\times\R P^{2N_1})/B;F,\bar h_0\)\\
	&=\tau\((M\times\R P^{2N_0}\times\R P^{2N_1},
		M_0\times\R P^{2N_0}\times\R P^{2N_1})/B;F,\bar h_1\)\\
	&=\tau\((M\times\R P^2{N_1},M_0\times\R P^{N_1})/B;F,h_1\)\;.
\endsplit\endmultline$$

\Remark\IgusaTorsionRem
Assume that~$M\to B$ is a fibre-bundle with closed fibres
and that~$h\colon M\to(0,1)$ is a fibre-wise Morse function.
Then by \IgusaFunctorThm\ and \IgleichMVBThm,
we clearly have	
	$$\tau_{\ch}(M/B;F,h)=\(\xi^u_{p,h,F}\)^*\tau\(\Cal M(\C),U\)\;.$$
If~$h$ is framed,
% i.e., the bundle~$T^uX\to C$ is trivial,
then
	$$\tau(M/B;F)=T(M/B;F,h)\;.$$
Nevertheless, Igusa's Definition is much more general than~\MorseTorsionDef.
One need not assume that~$h$ is fibre-wise Morse,
so~$\tau(M/B;F)$ is defined for all bundles with compact fibres
by \IframedThm,
and one can work with fibers that have a boundary.
\endremark


\Abschnitt\FramingSubsection Igusa's framing principle

We recall Igusa's framing principle,
and we use it to compare the higher analytic torsion of Bismut-Lott 
with Igusa's higher Franz-Reidemeister torsion
if there exists a fibre-wise Morse function
and a fibre-wise acyclic flat vector bundle.
At this point,
the identity of Igusa's and our higher torsion on~$\Wh^h\(\Cal M_r(\C),U(r)\)$
proved in \IgusaKapitel\ is crucial,
since we need both torsions within a single equation.

%Let~$h\colon M\to\R$ be a generalised fibre-wise Morse function
%such that~$h^{-1}(-\infty,a]$ intersects each fibre in a compact set
%for all~$a\in\R$,
%and with a finite number of singularities on each fibre of~$p\colon M\to B$.
%By the special coordinates of \SingTypeDef\ around~$C\cubical$,
%we may identify the extensions of the bundles~$T^uX|_{C^-}\oplus\R$
%and~$T^uX|_{C^+}$ in a neighbourhood of~$C\cubical$,
%where we have dropped the subscripts ``Morse'' and ``cubical'' to~$T^uX$
%for brevity.
%Then we have a well-defined characteristic class
%	$$(-1)^{\ind h}\,\^0J(T^uX)
%	={1\over2}\,\sum_{k=1}^\infty(-1)^{\ind h}
%		\,\zeta'(-2k)\,\ch(T^uX)\dg{4k}
%	\in H^{4*}(C;\R)\;.
%		\Formel\JTuXDef$$
%There are various ways to check this.
%If we regard~$C=C\Morse\cup C\cubical$ as a submanifold of~$M$,
%we find that~$C\cubical$ is a two-sided smooth submanifold of codimension~$1$.
%Passing~$C\cubical$ has the effect of adding or subtracting
%a trivialised one-dimensional subbundle to/from~$T^uX\to C\Morse$.
%Thus over a generic compact subset of~$M$,
%we can turn~$T^uX$ into a vector bundle~$\overline{T^uX}\to C$
%by adding trivial bundles whose rank depends on the connected component
%of~$C\Morse$.
%Note that by construction,
%we have~$\^0J(E)=\^0J(E\oplus\R)$ for all vector bundles~$E$.
%Thus,
%the form defined in~\JTuXDef\ is simply an additive characteristic
%class of~$\overline{T^uX}\to C$.
%


Recall that the additive characteristic class~$\^0J(E)$
was defined in~\BGzwei\ by
	$$\^0J(T^uX)
	={1\over2}\,\sum_{k=1}^\infty\,\zeta'(-2k)\,\ch(E)\dg{4k}
	\in H^{4*}(M;\R)
		\Formel\JTuXDef$$
for an arbitrary vector bundle~$E$ over a manifold~$M$.
Let now~$h$ be a fibre-wise Morse function.
The pushdown or ``transfer'' map~$\hat p_*\colon H^*(C;\R)\to H^*(B;\R)$
produces a class
	$$\hat p_*\((-1)^{\ind h}\,\^0J(T^uX)\)\in H^{4*}(B;\R)\;.$$
This class can in fact be extended to the situation
where~$h$ is a generalised fibre-wise Morse function,
cf.~\IKomplex.

The following theorem has been proved in \IBuch, Chapter~6 and~\IKomplex\
in the case that~$H\to B$ is a trivial bundle,
but for generalised fibre-wise Morse functions.
We will recall Igusa's proof
and show that it extends to the unitary case.
For simplicity,
we restrict our attention to true fibre-wise Morse functions
and closed fibres.

\Theorem\FramingThm.
Assume that~$F\to M$ and~$H\to B$ carry parallel metrics.
Let~$h$ be a fibre-wise Morse function.
Then
	$$\tau(M/B;F,h)
	=\tau(M/B;F)
		+2\hat p_*\((-1)^{\ind h}\^0J(T^u\Morse X)\)\,\rk F\;.$$

We note that generalised fibre-wise Morse functions enter through
Igusa's framed function theorem.
We remark that a general version of the framing principle
could also be concluded from a generalisation of \MainTheoremZwei\
to generalised Morse functions.

\Proof
We copy the proof of~\IBuch.
Replacing~$M$ by~$M\times\R$ and~$h$ by~$\bar h=(p,z)\mapsto h(p)+{z^2\over2}$,
we may assume that~$T^sX\to C$ contains a trivial subbundle
corresponding to the coordinate~$z$.
We note that both~$h$ and~$\bar h$ give rise to the same homotopy
class of maps~$\xi\colon B\to\Wh^u\(\Cal M(\C),U\)$,
and thus by \IgusaTorsionDef\ to the same higher torsion.
We continue to write~$M$ and~$h$ for the new bundle
and fibre-wise Morse function.
%and use~$z$ as a coordinate of the trivial subbundle of~$T^sX$ near~$C$
%with~$z|_C=0$.

%By the parametrised Morse Lemma,
%we can choose fibre-wise coordinates~$x$, $y$, $z$
%in a neighbourhood~$U$ of~$C$ with~$(x,y,z)|_C=0$
%such that
%	$$h(b;x,y,z)=h(b;0)+{1\over2}\,\Bigl(\abs x^2-\abs y^2+z^2\Bigr)\;.$$
%We replace~$h$ by a new function~$h_1$
%that coindices with~$h$ outside~$U$
%and inside~$U$ has two additional critical points~$C^+=(0,0,\eps)$
%and~$C^-=(0,0,2\eps)$ of indices~$\ind_C h+1$ and~$\ind_C h$
%for some small~$\eps>0$.
%\?Bildchen?
%As explained in~\IBuch,
%this can be done in such a way that no flow line
%of the negative gradient flow of~$h_1$ originating in~$C$
%converges to~$C^+\cup C^-$,
%and also no flow line originating in~$C^+\cup C^-$ and leaving~$U$
%comes back to~$C^+\cup C^-$.
%Then the new complex~$V_1\to B$
%takes the form~$\(V_1,\nabla^{V_1},A'_1\)$
%with
%	$$\(V_1,\nabla^{V_1}\)
%	=\(V\dg1,\nabla^V\)\oplus\(V,\nabla^V\)\oplus\(V,\nabla^V\)\;,$$
%where the summand correspond to~$C^+$, $C$ and~$C^-$ in that order,
%and
%	$$A'_1=\pmatrix\nabla^V&B&\id\\&A'&\\&&\nabla^V\endpmatrix\;.$$
%In other words,
%the functor~$\Xi_1^u\colon B\to\cWh^u\(\Cal M(\C),U\)$
%associated to~$h_1$
%arises from the old~$\Xi^u$ by stabilisation in~$\cWh^u\(\Cal M(\C),U\)$.
%Clearly,
%	$$\tau(M/B;F,h_1)=\tau(M/B;F,h)\;.\Formel\FrameTauHeinsFormel$$
%
%By the framed function theorem,
%we can replace~$h_1$ by a new function~$h_2$ that coincides with~$h_1$
%outside a small neighbourhood~$V$ of~$C^-$ and is framed inside~$V$.

Igusa then constructs a generalised fibre-wise Morse
function~$h_1\colon M\to\R$ with the following properties.
\roster
\item $h_1=h$ outside a neighbourhood~$U$ of~$C$.
\item $h_1$ is related by cancelation of Morse-type singularities
to a framed function~$h_2$
that coincides with~$h_2$ outside~$M\setminus U$.
\item The critical set~$C_1$ of~$h_1$ takes the form~$C_1=C\cup C'$,
and no negative gradient flow line of~$h_1$
originating in~$C_1$ and leaving~$U$ or originating in~$C$ converges to~$C'$.
\endroster

By~(2),
the map~$\xi_1\colon B\to\Wh^u\(\Cal M(\C),U\)$ constructed from~$h_1$
is homotopic to the map~$\xi_2\colon B\to\Wh^u\(\Cal M(\C),U\)$ from~$h_2$
because the corresponding functors are homotopic up to an elementary extension.
This shows that
	$$\tau(M/B;F)=\tau(M/B;F,h_2)=\tau(M/B;F,h_1)
	\Formel\FrameTauHdreiFormel$$
because~$h_2$ is framed.
%It remains to understand the difference~$\tau(M/B;F,h_1)-\tau(M/B;F,h)$

Note that~$h_1$ is no longer a Morse function.
By~(3),
we can construct the complex~$\(V_1,\nabla^{V_1},A'_1\)$
outside~$p(C'\cubical)$
such that
	$$\(V_1,\nabla^{V_1}\)
	=\(V,\nabla^V\)\oplus\(W,\nabla^W\)\;,$$
where the two summands correspond to~$C$ and~$C'$,
and
	$$A'_1
	=\pmatrix B'&*\\0&A'\endpmatrix\;.$$
We also note that~$V_1$ carries a natural parallel metric
because obviously~$F|_U$ carries a parallel metric by the assumption
that~$g^V$ is adapted and parallel.
Again by~\IBuch,
we may assume that each birth-death singularity of~$h_1$
locally gives rise to an elementary expansion of~$W$ in the sense of
\DiffElExDef.
This allows us to define a filtration of~$\(V_1,\nabla^{V_1},A'_1\)$
outside~$p(C'\cubical)$ by
	$$\(V_1,\nabla^{V_1},A'_1\)
		\supset\(W,\nabla^W,B'\)
		\supset0\;,
	\Formel\FrameFiltration$$\
and this filtration is compatible with stabilisation at the birth-death
singularities of~$h_1$.

The subcomplex~$\(W,\nabla^W,B'\)$ is fibre-wise acyclic.
%By property~(3) above,
%we may regard it as the pushdown of a complex living over~$C$.
By Igusa's calculations in~\IBuch, Chapters~6 and~7,
we obtain
	$$T\(\nabla^W,B',g^W\)
	=-2\,\hat p_*\((-1)^{\ind h}\,\^0J(T^uX)\)\,\rk F\;.$$
Note that Igusa's calculations apply here
because by \IgleichMVBThm,
Igusa's higher Franz-Reide\-mei\-ster torsion
is equal to the torsion of \IgusaTorsionDef\ in the acyclic case.

It follows from the fibre-wise acyclicity of~$\(W,\nabla^W,B'\)$
that the spectral sequence associated to~\FrameFiltration\
degenerates at~$E_1=H$.
\SpecSeqThm\ and~\FrameTauHdreiFormel\ now imply that
$$\align
	\tau(M/B;F)
	&=\tau(M/B;F,h_1)\\
	&=\tau\(\nabla^V,A',g^V\)
		+T\(\nabla^W,B',g^W\)\\
	&=\tau(M/B;F,h)-2\,\hat p_*\((-1)^{\ind h}\,\^0J(T^uX)\)\,\rk F\;.
		\quad\qed
\endalign$$
\enddemo


\Abschnitt\ProofZweiSubsection A Proof of Theorem~0.3

We give a short proof of \MainTheoremZwei\ and show
that it is compatible with some of Igusa's results.

\demo{Proof\/ \rm of \MainTheoremZwei}
Let~$M\to B$ be a family of compact manifolds,
and let~$F\to M$ be a flat vector bundle.
We assume that there exists a fibre-wise Morse function~$h\colon M\to\R$
and that the vector bundles~$F\to M$ and~$H^*(M/B;F)\to B$
carry parallel metrics.
We construct a family Thom--smale complex~$(V,\nabla^V,A')$ as usual.
\TeilEinsTheorem\ then reduces to
$$\multline
	\Cal T\(T^HM,g\TX,\nabla^F,g^F\)
	-T\(\nabla^V,A',g^V\)-\chslo\(\nabla^H,g^H_{L_2},g^H_V\)\\
	=\hat p_*\((-1)^{\ind h}\,\^0J(T^sX-T^uX)\)\,\rk F\;.
\endmultline\tag\FormelNummer\ProofZweiFormelEins$$
By definition of~$\Cal T(M/B;F)$ and~$\tau(M/B;F,h)=T(M/B;F,h)$,
we have
$$\multline
	\Bigl(\Cal T\(T^HM,g\TX,\nabla^F,g^F\)
		-\tau\(A',g^V,g^V\)
		-\chslo\(\nabla^H,g^H_{L_2},g^H_V\)\Bigr)\dg{\ge2}\\
	=\Cal T(M/B;F)-\tau(M/B;F,h)\;.
\endmultline\tag\FormelNummer\ProofZweiFormelZwei$$

The framing principle above allows us to compute
$$\multline
	\tau(M/B;F,h)\\
\split
	&=\tau(M/B;F)+\hat p_*\((-1)^{\ind h}\,\^0J(TX)\)\,\rk F
		-\hat p_*\((-1)^{\ind h}\,\^0J(T^sX-T^uX)\)\,\rk F\\
	&=\tau(M/B;F)+\int_{M/B}e(TX)\,\^0J(TX)\,\rk F
		-\hat p_*\((-1)^{\ind h}\,\^0J(T^sX-T^uX)\)\,\rk F\;,
\endsplit\endmultline\tag\FormelNummer\ProofZweiFormelDrei$$
where the last identity holds
because the singular current~$(-1)^{\ind h}\,\delta_C$
is homologous to~$e(TX)$ by the family Poincar\'e-Hopf theorem.

Combining~\ProofZweiFormelEins--\ProofZweiFormelDrei,
we obtain
	$$\Cal T(M/B;F)
	=\tau(M/B;F)+\int_{M/B}e(TX)\,\^0J(TX)\,\rk F\;,$$
which was the assertion of~\MainTheoremZwei.
\qed\enddemo



\Abschnitt\GlueAbs A glueing formula for the unitary torsion

We prove a glueing formula for the unitary torsion of a family
of manifolds that are glued together from two submanifolds with a common
hypersurface.
The main ingredient is \SpecSeqThm.

Suppose that~$M^+\to B$ and~$M^-\to B$ are two proper submersions
with fibre-wise boundary~$\del M^\pm=M^\pm_0\cup M^\pm_1$.
Let~$F^\pm\to M^\pm$ be two flat vector bundles
with parallel metric~$g^{F^\pm}$.
We assume that there exists a diffeomorphism~$\phy\colon M^-_1\to M^+_0$
that lifts to a parallel linear isometry~$\Phi\colon F^-|_{M^-_1}\to F^+|_{M^+_0}$,
so
$$\CD
	F^-|_{M^-_1}@>\Phi>>F^+|_{M^+_0}\\
	@VVV@VVV\\
	M^-_1@>\phy>>M^+_0&\;.
\endCD$$
By glueing,
we obtain
	$$F :=F^-\cup_\Phi F^+\quad\to\quad M:=M^-\cup_\phy M^+\;.
	\Formel\GlueConstruction$$
Moreover, we put~$\del M=M_0\cup M_1$ with
	$$M_0=M^-_0\Mand M_1=M^+_1\;.$$

The following result is a cohomological version
of Igusa's Splitting Lemma in~\IBuch, 5.7.8,
where a similar result was obtained 
for maps to the Whitehead space,
but with more restrictive conditions on~$H\(M^\pm/B,M^\pm_0;F\)$.

\Theorem\GlueingThm.
Assume that the fibre-wise cohomology bundles~$H\(M^\pm/B,M^\pm_0;F\)\to B$
carry parallel metrics.
Then the fibre-wise cohomology~$H\(M/B,M_0/B;F)\to B$
also carries a parallel metric,
and
	$$\tau(M/B,M_0/B;F)
	=\tau(M^-/B,M^-_0/B;F^-)+\tau(M^+/B,M^+_0/B;F^+)
		\quad\in\quad H^{\even,\ge2}(B;\R)\;.$$

\Proof
We may assume that there exist framed function~$h^\pm\colon M^\pm\to[0,1]$
such that~$i=0$, $1$ are regular values
with~$(h^\pm)^{-1}(i)=M^\pm_i$.
Then the function~$h\colon M\to[0,1]$ with
	$$h(p)
	=\cases
		{h^-(p)\over2}		&\text{for~$p\in M^-$, and}\\
		{1+h^+(p)\over2}	&\text{for~$p\in M^+$.}
	\endcases$$
is framed and satisfies~$h^{-1}(i)=M_i$ for the regular values~$i=0$, $1$.

We construct a family Thom-Smale complex~$(V,\nabla^V,A')\to B$ as before
and let~$\xi=\xi_{p,h,F}\colon M\to\Wh^u\(\Cal(\C),U\)$
denote the corresponding map to the universal unitary Whitehead space.
Then~$V$ admits a natural filtration
	$$\(V,\nabla^V,A'\)
		\supset\(V^+,\nabla^{V^+},A^{+\prime}\)
		\supset 0\;.$$
The two steps of the associated spectral sequence take the form
$$\align
	E_0
	&=\(V^-,\nabla^{V^-},A^{-\prime}\)
		\oplus\(V^+,\nabla^{V^+},A^{+\prime}\)\\
		\Land
	E_1
	&=\(H^*(V^-,a_0^{-\prime})\oplus H^*(V^+,a_0^{+\prime})\,,\;
		\nabla^{E_1}+d'_1\)\;.
\endalign$$

By our assumptions,
the bundles~$H^*(V^\pm,a_0^{\pm\prime})\cong H^*(M^\pm/B,M^\pm_0;F)\to B$
carry parallel metrics~$g^{H^\pm}$.
Let~$g^{H^+\oplus H^-}$ denote the direct sum of these metrics
on~$E_1=H^*(V^-,a_0^{-\prime})\oplus H^*(V^+,a_0^{+\prime})$.
Moreover,
the coboundary
	$$d'_1\colon H^*(V^-,a_0^{-\prime})\to H^*(V^+,a_0^{+\prime})$$
is parallel with respect to~$\nabla^{E_1}$ by \SpecSecBundleProp.
This implies that the total fibre-wise cohomology
	$$H:=H^*(V,a'_0)\cong H^*(M/B,M_0/B;F)\to B$$
carries a parallel metric induced by~$g^{H^+\oplus H^-}$
via finite-dimensional Hodge theory,
which we denote by~$g^H$.
The appendix of~\BL\ implies that
	$$T^{\roman{BL}}\(D'_1,g^{H^+\oplus H^-}\)
	=T^{\roman{BL}}\(\nabla^{E_1}+d'_1,g^{H^+\oplus H^-}\)
	=0\;.
		\Formel\GlueEeinsFormel$$

We can now apply \SpecSeqThm\ to find that
$$\align
	\kern4em&\kern-4em
	T\(\nabla^V,A',g^V\)+\chslo\(\nabla^H,g^H,g^H_V\)\\
	&=T\(\nabla^{E_0},D'_0,g^{E_0}\)
		+T^{\roman{BL}}\(D'_1,g^{E_1}\)
		+\chslo\(\nabla^H,g^H,g^{E_\infty}\)\\
	&=T\(\nabla^{E_0},D'_0,g^{E_0}\)
		+\chslo\(\nabla^{E_1},g^{H^+\oplus H^-},g^{E_1}\)
		+T^{\roman{BL}}\(D'_1,g^{H^+\oplus H^-}\)\\
	&=T\(\nabla^{V^+},A^{+\prime},g^{V^+}\)
		+\chslo\(\nabla^{H^+},g^{H^+},g^{H^+}_{V^+}\)\\
	&\qquad
		+T\(\nabla^{V^-},A^{-\prime},g^{V^-}\)
		+\chslo\(\nabla^{H^-},g^{H^-},g^{H^-}_{V^-}\)
\endalign$$
modulo exact forms on~$B$.
The theorem follows.
\qed\enddemo

For proper submersions with closed fibres,
\GlueingThm\ implies a cut-and-paste formula.
Here,
we assume that~$M_0\to B$ and~$M_1\to B$ are two proper submersion such
that
	$$M_i=M_i^+\cup_{M_i^0}M_i^-$$
for~$i=0$, $1$,
where~$M_i^\pm$, $M_1^\pm$ are families of closed submanifolds
intersecting in the common boundary~$M_i^0=M_i^+\cap M_i^-$.
Assume that~$F_i\colon M_i$ is a flat vector bundle
with a parallel metric~$g^{F_i}$ for~$i=0$, $1$
and that there exists a diffeomorphism~$\phy\colon M_0^0\to M_1^0$
which lifts to a linear isometry~$\Phi\colon F_0|_{M_0^0}\to F_1|_{M_1^0}$,
$$\CD
	F_0|_{M_0^0}@>\Phi>>F_1|_{M_1^0}\\
	@VVV@VVV\\
	M_0^0@>\phy>>M_1^0&\;.
\endCD$$
Then we can construct two new families of closed submanifolds
	$$M'_0=M_0^-\cup_\phy M_1^+
		\Mand
	M'_1=M_1^-\cup_\phy M_0^+$$
that carry flat vector bundles~$F'_i\to M'_i$ for~$i=0$, $1$.

\Corollary\GlueingCor.
Assume that the bundles~$H^*(M_i^-/B;F_i)\to B$
and~$H^*(M_i^+/B,M_i^0/B;F)\to B$ carry parallel metrics for~$i=0$, $1$.
Then~$H^*(M_i/B;F_i)\to B$ and~$H^*(M'_i/B;F_i)\to B$ also carry
parallel metrics,
and we have
	$$\tau(M_0/B;F)+\tau(M_1/B;F)
	=\tau(M'_0/B;F)+\tau(M'_1/B;F)
	\quad\in\quad H^{\even,\ge2}(B;\R)\;.$$

\Proof
This is an immediate consequence of \GlueingThm.
\qed\enddemo


\Abschnitt\HatcherZweiSubsection A proof of Theorem~0.2

We want to use \GlueingCor\ to construct some more examples
of ``exotic'' smooth structures on fibre bundles from Hatcher's
example as described in \HatcherSubsection.
Assume that we are in the situation of \GenFibreSubsection.
That is,
we fix~$k>0$ and~$l>0$ sufficiently large with respect to~$k$,
and we let~$X$ be an arbitrary compact connected $(2l-1)$-dimensional manifold.
We decompose~$X$ along a hypersurface~$X^0$ into
	$$X=X^+\cup_{X^0}X^-\;,$$
such that~$X^-$ is diffeomorphic to the $(2l-1)$-dimensional disc~$D^{2l-1}$.

We also let~$M_\gamma\to S^{4k}$ denote Hatcher's example
constructed starting with a generator~$\gamma\in\pi_{4k-1}(O)$ of~$\ker J$.
In particular,
$M_\gamma$ admits a fibre-wise Morse function with six critical points
(in fact, four would already be enough),
such that the unique maximum has a trivial disc bundle neighbourhood,
so we can decompose
	$$M_\gamma=M_\gamma^+\cup_{M_\gamma^0}M_\gamma^-\;,$$
where now~$M_\gamma^+\to S^{4k}$ is diffeomorphic to~$D^{2l-1}\times S^{4k}$.

Assume that~$X$ carries a flat vector bundle~$F\to X$ of rank~$r$
with parallel metric~$g^F$,
then~$F|_{X^-}$ is trivial.
We fix a diffeomorphism~$\phy\colon X^0\times S^{4k}\to M_\gamma^0$
and a lift~$\Phi\colon F|_{X^0}\times S^{4k}\to M_\gamma^0\times\C^r$
as a parallel linear isometry.
We construct
	$$F'_\gamma
	:=\(F|_{X^+}\times S^{4k}\)\cup_\Phi\(M_\gamma^-\times\C^r\)
		\quad\to\quad
	M'_\gamma
	=\(X^+\times S^{4k}\)\cup_\phy M_\gamma^-$$
Glueing the other two parts gives the trivial bundle
	$$\C^r\times S^{2l-1}\times S^{4k}
		\quad\to\quad
	S^{2l-1}\times S^{4k}=X^-\cup_\phy M_\gamma^+\;.$$
By construction,
the fibre-wise cohomology bundles of~$X^-\times S^{4k}\to S^{4k}$,
$(X^+,X^0)\times S^{4k}\to S^{4k}$, $M_\gamma^+\to S^{4k}$
and~$M_\gamma^-\to S^{4k}$ with coefficients in~$F$ respectively in~$\C^r$
are all trivial.
We may apply \MainTheoremZwei\ and \GlueingCor\ and get
$$\split
	\Cal T\(M'_\gamma/S^{4k};F'_\gamma\)
	&=\tau\(M'_\gamma/S^{4k};F'_\gamma\)
	=\tau\(M_\gamma/S^{4k},\C^r\)\\
	&=2^{2-k}\,b_k\,\zeta'(-2k)\,u
		\quad\in\quad H^{4k}\(S^{4k};\R\)\;.
\endsplit\Formel\HatcherGlueingFormelEins$$

The above construction of~$M'_\gamma$ generalises 
the example of \GenFibreSubsection\ to the case of non-trivial~$F$.
As in \HatcherMoreSubsection,
we may glue~$j$ copies of the bundle~$M'_\gamma\to S^{4k}$
to an arbitrary fibre bundle~$M\to B$ with fibre~$X$
and $4k$-dimensional compact oriented base~$B$,
to obtain a new bundle
	$$p_j\colon M_j\to B$$
which is homeomorphic to the original~$M\to B$ as a bundle.
For negative~$j$,
we glue~$\abs j$ copies of~$M'_{-\gamma}\to S^{4k}$ to~$M\to B$.
We assume that~$F\to M$ is a unitarily flat vector bundle,
then after glueing,
we have homeomorphic unitarily flat vector bundles~$F_j\to M_j$
for all~$j\in\Z$.

Let~$g^H$ be a fixed metric on the bundle
	$$H^*(M_j/B;F_j)\cong H=H^*(M/B;F)\to B\;.$$
Then as in \HatcherGenExpFormel,
we compute
	$$\int_{M_j/B}\Cal T\(M_j/B;F_j,g^H\)
	=\int_{M/B}\Cal T\(M/B;F,g^H\)
		+2^{2-k}\,j\,b_k\,\zeta'(-2k)\,u\;,$$
where~$\Cal T\(M_j/B;F_j,g^H\)\in\Omega^\even(B)/d\Omega^\odd(B)$
is defined as in \HatcherGHTorsionDef\ by
	$$\Cal T (M/B;F,g^H)
	=\Bigl(\Cal T \(T^HM,g\TX,\nabla^F,g^F\)
		+\chslo\(\nabla^H,g^H,g^H_{L_2}\)\Bigr)\dg{\ge 2}\;.$$

This implies the following generalisations of \HatcherTheorem,
where~$\Diff(M;F)$ denotes the group of parallel lifts of arbitrary
diffeomorphisms of~$M$ to a given flat vector bundle~$F$,
and~$\Diff^+(M;F)$ denotes the subgroup coming from orientation preserving
diffeomorphisms whenever~$M$ is orientable.

\Theorem\TeilZweiHatcherTheorem.
Let~$p\colon M\to B$ be a proper submersion
and let~$(F,\nabla^F)\to M$ be a vector bundle with a parallel metric~$g^F$.
Assume that~$B$ is compact, orientable, and of dimension~$4k>0$.
Let the bundles~$\(q_j\colon M\to B\)_{j\in\Z}$ with~$q_0=p$
be constructed as in \HomeoDiffeoSubsection.
Assume that for~$i$, $j\in\Z$ with~$i\ne j$,
there exists diffeomorphisms~$\Phi\in\Diff(M;F)$ and~$\Psi\in\Diff^+(B)$
such that the diagramme
$$\CD
	M@>\Phi>>M\\
	@Vq_iVV@VVq_jV\\
	B@>\Psi>>B
\endCD$$
commutes.
Then~$\Psi\in\Diff^+(B;H)$ for~$H=H^*(M/B;\C)\to B$,
and
	$$\cho\(\nabla^{T_\Psi H}\)[T_\Psi B]
	=2^{2-k}\,(j-i)\,j_0\,b_k\,\zeta'(-2k)\,\rk F\;.$$
In particular,
this is only possible if~$H\to B$ does not carry a parallel metric,
and if~$\Psi$ does not represent a torsion element
in the mapping class group.

Clearly,
\TeilZweiHatcherTheorem\ implies the generalised second statement of \ApplThm\
by the same arguments as in \HomeoDiffeoSubsection.


\enddocument











==> igusa.tex <==
%auto-ignore
\input morse2.def

\document

\Kapitel\IgusaKapitel=8 Igusa's higher Franz-Reidemeister torsion

In this chapter,
we state and prove \IgleichMVBThm,
by which Igusa's higher Franz-Reidemeister torsion coincides
with the higher torsion constructed in \TChRGDef.

Using Igusa's two-index theorem,
the proof of \IgleichMVBThm\ is reduced to the case
of a family Thom-Smale complex~$V=V^0\oplus V^1$ living in only two degrees.
We also give a sketch of the proof in \TwoIndexSubsection.

We construct a family of flat superconnections
from a given flat superconnection on a bundle~$V=V^0\oplus V^1$
in \AltFamilySubsection.
This family is used to decompose~$T\(\nabla^V,A',g^V\)$ into four terms
in \AltCompSubsection.

One of these terms is a Bismut-Lott torsion class,
and we show in \IgusaIFSubsection\
that it is equal to Igusa's class~$F$ in~\IBuch.
The remaining three terms are polynomials in the components of~$A'$,
and their sum forms an $L$-class \`a la~\BGzwei,
cf.\ \MVBRigiditySubsection.
We identify these terms with Igusa's classes~$G$, $K$ and~$\overline K^*$
in Subsections~\NummerVon\IgusaPGSubsection\
and~\SubsectionLetter\IgusaQKSubsection.




\Abschnitt\TwoIndexSubsection Igusa's two-index theorem
and a proof of Theorem~8.1

We formulate the main result of this section
and reduce its proof to the special case
of a family Thom-Smale complex living in only two degrees.

Let~$\tau=\tau\(\Cal M_r(\C),U(r)\)$
and~$T=T\(\Cal M_r(\C),U(r)\)\in H^\even\bigl(\Wh^h\(\Cal M_r(\C),U(r)\)\bigr)$
denote Igusa's universal higher Franz-Reidemeister torsion,
and the class constructed in \TChRGDef\ above.

\Theorem\IgleichMVBThm.
The classes~$\tau$ and~$T$
in~$H^\even\bigl(\Wh^{h}\(\Cal M_r(\C),U(r)\)\bigr)$ coincide.

A proof of this theorem is given at the end of this subsection.

\Definition\TwoIndexWhDef
Let~$\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
be the full simplicial subcategory of the
differential Whitehead category~$\cWh^{\diff}\(\Cal M_r(\C),U(r)\)$
consisting in degree~$k$ of all objects~$(P,a')$
such that~$P=P^0\cup P^1$ and such that~$a'_0\colon\(\C^r\)^{P^0}
\to\(\C^r\)^{P^1}$ is invertible
at one (and thus at all) points of~$\Delta_k$.
Let the acyclic differential two-index
Whitehead space~$\Wh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
be the geometric realisation of~$\cWh^{\diff}\(\Cal M_r(\C),U(r)\)$.
\enddefinition

\Remark\TwoIndexRem
We can also construct simplicial
and mixed models~$\Wh^{\simp,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
and~$\Wh^{\mix,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
of the acyclic two-index Whitehead space as in \WhKapitel.
However,
the proof of \WhHomEqThm\ shows that these spaces are homotopy equivalent.
\endremark

\Fact\TwoIndexThm(Two-Index Theorem).
The acyclic two-index Whitehead space~$\Wh^{h,\{0,1\}}
\penalty0\(\Cal M_r(\C),U(r)\)$
is a deformation retract
of the full acyclic Whitehead space~$\Wh^{h}\(\Cal M_r(\C),U(r)\)$.

This implies that it is sufficient to prove \IgleichMVBThm\
for the restrictions of~$\tau$ and~$T$
to the acyclic two-index
Whitehead space~$\Wh^{h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$.

\demo{\Proof \rm of \IgleichMVBThm}
By the two-index theorem,
it is enough to check the equality of~$\tau$ and~$T$
on~$\Wh^{h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$.
All constructions in this and the following subsections
will be natural with respect to pull-back.
Thus,
me may and we will replace~$\Wh^{h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
for notational convenience
by an arbitrary manifold~$B$ equipped
with a family Thom Smale complex of the special form
	$$(V,\nabla^V,A')
	=\(V^0\oplus V^1,\nabla^{V^0}\oplus\nabla^{V^1}
		,\nabla^{V^0}\oplus\nabla^{V^1}+a_0+a_1^0+a_1^1+a_2\)\;,
	\Formel\TwoIndexComplex$$
where~$a_0$, $a_1^0$, $a_1^1$ and~$a_2$ are the components of~$A'-\nabla^V$.
We assume that~$V$ carries an adapted metric~$g^V$
as in \MorseMetricDef\ that is parallel.
We will forget about the family of endomorphisms~$h^V$;
we will however remember that the coefficients of~$A'-\nabla^V$
take values in a nilpotent subalgebra of~$\End V$
in a neighbourhood of each point of~$B$,
cf.\ \TChRem~(3) above.

There is a natural construction
of Igusa's higher Franz-Reidemeister torsion~$\tau=\tau(\nabla^V,A',g^V)$
in this situation,
which we will introduce in
Subsections~\NummerVon\IgusaIFSubsection--\SubsectionLetter\IgusaQKSubsection.
In fact, it follows from \AltCompProp\
and Lemmata~\NummerVon\IgusaFLemma, \NummerVon\IgusaGLemma\
and~\NummerVon\IgusaKLemma\ that
$$\align
	T\(\nabla^V,A',g^V\)\dg{\ge2}
%	&=\Bigl(T^{\roman{BL}}\(\overline A'|_{r=0},g^V\)
%		+G'+K'-\overline{K'}^*\Bigr)\dg{\ge2}
%		+d\widetilde T\\
	&=\(F+G+K-\overline K{}^*\)\dg{\ge2}
		+d\Bigl(\widetilde T+\widetilde G+\widetilde K
			-\overline{\widetilde K}^*\Bigr)\\
	&=\tau(\nabla^V,A',g^V)\dg{\ge2}
		+d\Bigl(\widetilde T+\widetilde G+\widetilde K
			-\overline{\widetilde K}^*\Bigr)
\endalign$$
for certain naturally defined forms~$\widetilde T$, $\widetilde G$
and~$\widetilde K$ depending only on~$\nabla^V$, $A'$, and~$g^V$.
This implies that the cochains obtained
by integrating~$\tau\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)\dg{\ge2}$
and~$T\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)\dg{\ge2}$ over the simplices
of~$\bigl|\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)\bigr|$
differ by an exact cochain.
On the other hand,
we know by \IBuch\ and \MVBTorsionThm\
that both~$\tau\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)\dg0$
and~$T\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)\dg0$
coincide with the classical fibre-wise Franz-Reidemeister torsion
of the complex~$(V,a_0)$.
Because both~$\tau$ and~$T$ are even classes,
this proves \IgleichMVBThm.
\qed\enddemo


\Abschnitt\AltFamilySubsection A family of flat superconnections

We now restrict our attention
to family Thom-Smale complexes of the form~\TwoIndexComplex.

%We will construct a projection~$\Wh^u\(\Cal M_r(\C),U(r)\)\to\Wh^h\(\Cal M_r(\C),U(r)\)$ in \ConeSubsection\
%that is also compatible with our higher torsion.
%This will then imply that the analytic torsion
%on the unitary Whitehead space inherits several important properties
%directly from Igusa's higher Franz-Reidemeister torsion.
%In particular,
%we can employ Igusa's framing principle
%to compare the higher analytic torsion with an extension Igusa's
%higher Franz-Reidemeister torsion
%on fibre bundles with a fibrewise Morse function
%and a unitarily flat bundle having a unitarily flat fibrewise cohomology.

Let us start by classifying all flat superconnections
of total degree one with a prescribed term in degree zero
on a vector bundle~$V=V^0\oplus V^1$.
If~$\nabla^{V^0}$ and~$\nabla^{V^1}$ are connections on~$V^0$ and~$V^1$
and~$a_0\colon V^0\to V^1$ is an isomorphism,
we define new connections
	$$a_0^\#\nabla^{V^1}=-a_0^{-1}\,\nabla^{V^1}\,a_0\Mand
	a_{0\#}\nabla^{V^0}=-a_0\,\nabla^{V^0}\,a_0^{-1}\;.
	\Formel\IgusaAnullXDef$$
By our sign convention,
these are indeed connections,
with
	$$\(a_0^\#\nabla^{V^1}\)_v=a_0^{-1}\,\nabla^{V^1}_v\,a_0
		\Mand
	\(a_{0\#}\nabla^{V^0}\)_v=a_0\,\nabla^{V^0}_v\,a_0^{-1}$$
for all~$v\in TB$.


\Lemma\FlatSupConnLemma.
Let~$V=V^0\oplus V^1\to B$ be a $\Z$-graded vector bundle,
let~$a_0\colon V^0\to V^1$ be a vector bundle isomorphism,
and let~$\nabla^1$ be a connection on~$V^1$.
Then
	$$A'=a_0+a_0^\#\nabla^1\oplus\nabla^1-a_0^{-1}\,\(\nabla^1\)^2$$
defines a flat superconnection of total degree~$1$ on~$V$.
Moreover,
all flat superconnections of total degree~$1$ on~$V$
with a given invertible~$a_0$ arise this way.

\Proof
Let~$A'=a_0+\nabla^0\oplus\nabla^1+a_2$
be a superconnection of total degree~$1$.
Flatness of~$A'$ is equivalent to the following three conditions:
$$\align
	a_0\,\nabla^0+\nabla^1\,a_0&=0\;,\tag1\\
	a_2\,a_0+\(\nabla^0\)^2=0\qquad\text{and}&\qquad
	a_0\,a_2+\(\nabla^1\)^2=0\;,\tag2\\
		\Land
	\nabla^0\,a_2+a_2\,\nabla^1&=0\;.\tag3
\endalign$$
We assume that~$a_0$ is invertible.
Then equation~(1) is equivalent to
	$$\nabla^0=a_0^\#\nabla^1\;.\tag{$1\mskip-1mu'$}$$
Given~(1) or~$(1\mskip-1mu')$,
we have~$a_0\,\(\nabla^0\)^2=\(\nabla^1\)^2\,a_0$,
so equation~(2) is equivalent to
	$$a_2=-a_0^{-1}\,\(\nabla^1\)^2\;.\tag{$2\mskip1mu'$}$$
Finally if~(1) or~$(1\mskip-1mu')$ and~(2) or~$(2\mskip1mu')$ hold,
then~(3) follows from the Bianchi identity for~$\nabla^1$,
because
	$$\nabla^0\,a_2+a_2\,\nabla^1
	=-a_0^{-1}\,\bigl[\nabla^1,(\nabla^1)^2\bigr]
	=0\;.\quad\qed$$
\enddemo


In order to compare Igusa's torsion class
in the Chern normalisation with~$T\(\nabla^V,A',g^V\)$,
we consider a family of flat superconnections
linking~$A'$ to a ``trivial'' flat superconnection.
Consider the bundle
	$$\overline V=V\times[0,1]\;\to\;\overline B=B\times[0,1]\;,$$
and extend the connection~$\nabla^V=\nabla^{V^0}\oplus\nabla^{V^1}$
and the superconnection~$A'$
trivially to~$\overline V$.
Let~$r$ be the coordinate of~$[0,1]$,
and suppose that the original superconnection takes the form
	$$A'=\nabla^V+a_0+a_1^0+a_1^1+a_2$$
with an invertible~$a_0$.
We define a new superconnection on~$\overline V$ by
	$$\overline  A'
	=a_0
		+a_0^\#\(\nabla^{\overline V^1}+r\,a_1^1\)
			\oplus\(\nabla^{\overline V^1}+r\,a_1^1\)
		-a_0^{-1}\(\nabla^{\overline V^1}+r\,a_1^1\)^2\;.
	\Formel\AltFamilyDef$$

\Lemma\AltFamilyLemma.
The superconnection~$\overline A'$ is flat,
and its restriction to~$r=1$ equals~$A'$.

\Proof
The first statement is a consequence of \FlatSupConnLemma.
The second statement also follows easily from  \FlatSupConnLemma,
because in both cases
it suffices to compare~$a_0$ and the connection acting on~$V^1$.
\qed\enddemo

\Remark\AxNullRem
Note that the coefficients
of~$\overline A'|_{r=1}-\nabla^{\overline V}=A'-\nabla^V$
take values in a nilpotent subalgebra of~$\End V$ by assumption.
Similarly,
we have
	$$\overline A'|_{r=0}-a_0^\#\nabla^{V^1}\oplus\nabla^{V^1}
	=a_0\quad\in\quad\Hom(V^0,V^1)\subset\End V\;,$$
and~$\Hom(V^0,V^1)$ is of course a nilpotent subalgebra.
Thus it makes sense to talk about the higher torsions
	$$T\Bigl(a_0^\#\nabla^{V^1}\oplus\nabla^{V^1}
		,\overline A'|_{r=0},g^V\Bigr)
	=T^{\roman{BL}}\Bigl(\overline A'|_{r=0},g^V\Bigr)
	\Mand
	T\Bigl(\nabla^V,\overline A'|_{r=1},g^V\Bigr)\;.
	\Formel\TwoTorsionsFormel$$
Note however that in general there will be no meaningful torsion
of~$A'|_r$ for some~$r\in(0,1)$.
Even worse,
in general there will be no flat connection on~$\overline V$
which restricts to~$a_0^\#\nabla^{V^1}\oplus\nabla^{V^1}$ at~$r=0$
and to~$\nabla^V$ at~$r=1$.
\endremark


Let~$\overline A''$ be the adjoint of~$\overline A'$ with respect to~$g^V$.
Since we assume that~$g^V$ is unitarily flat with respect to~$\nabla^V$,
we have~$\nabla^{V^1}=\nabla^{V^1,*}$.
We find that
	$$A''
	=a_0^*+a_{0\#}^*\(\nabla^{V^1}+ra_1^{1*}\)
			\oplus\(\nabla^{V^1}+ra_1^{1*}\)
		-\(\nabla^{V^1}+ra_1^{1*}\)^2\,(a_0^*)^{-1}\;,$$
where we agree that~$a_1^{1*}(v)=-\(a_1^1(v)\)$ for~$v\in TB$.

We extend the restrictions to the hyperplane~$T=1$
of the superconnections~$\^1\Asl$, $\^2\Asl$ and~$\^3\Asl$
of~\EinsAslFormel, \ZweiAslFormel\ und~\DreiAslFormel\
to the bundles
$$\alignat2
	\^1\overline V&\to
	\^1\overline B=B\times[0,1]^2\times[1,\infty)&
		\qquad&\text{with coordinates }
			(r,s,t)\in[0,1]^2\times[1,\infty)\;,\\
	\^2\overline V&\to
	\^2\overline B=B\times[0,1]^3&
		\qquad&\text{with coordinates }
			(r,s,u)\in[0,1]^3\;,\\
		\Land
	\^3\overline V&\to
	\^3\overline B=B\times[0,1]^3&
		\qquad&\text{with coordinates }
			(r,s,v)\in[0,1]^3\;.
\endalignat$$
Therefore, set
$$\align
\split
	\^1\Asl
%	&=(1-s)\,\Asl'_{t\over4(1-s)^2}+s\,\Asl''_{t\over4s^2}\\
	&={\sqrt t\over 2}\,\(a_0+a_0^*\)
		+(1-s)\,a_0^\#\(\nabla^{\overline V^1}+ra_1^1\)
			\oplus\(\nabla^{\overline V^1}+ra_1^1\)\\
	&\kern5em
		+s\,a_{0\#}^*\(\nabla^{\overline V^1}+ra_1^{1*}\)
			\oplus\(\nabla^{\overline V^1}+ra_1^{1*}\)\\
	&\qquad
		-{2\over\sqrt t}\,
		\Bigl((1-s)^2\,a_0^{-1}\,\(\nabla^{\overline V^1}+ra_1^1\)^2
		+s\,\(\nabla^{\overline V^1}+ra_1^{1*}\)^2\,(a_0^*)^{-1}\Bigr)\\
	&\qquad
		-2N^V\,ds+(2s-1)\,{N^V\over2t}\,dt\;,
\endsplit\Formel\EinsAslFamilyDef\\
\noalign{\smallskip}\allowdisplaybreak
\split
	\^2\Asl
	&={1\over 2}\,\((1-s+us)\,a_0+(u+s-us)\,a_0^*\)\\
	&\kern5em
		+(1-s)\,a_0^\#\(\nabla^{\overline V^1}+ra_1^1\)
			\oplus\(\nabla^{\overline V^1}+ra_1^1\)\\
	&\kern5em
		+s\,a_{0\#}^*\(\nabla^{\overline V^1}+ra_1^{1*}\)
			\oplus\(\nabla^{\overline V^1}+ra_1^{1*}\)\\
	&\qquad
		-2\,(1-us)\,(1-s)
			\,a_0^{-1}\,\(\nabla^{\overline V^1}+ra_1^1\)^2\\
	&\kern5em
		-2\,(1-u+us)\,s
		\,\(\nabla^{\overline V^1}+ra_1^{1*}\)^2\,(a_0^*)^{-1}
		-2u\,N^V\,ds\;,
\endsplit\Formel\ZweiAslFamilyDef\\
\noalign{\smallskip}\allowdisplaybreak
\split
	\^3\Asl
	&={v\over2}\,\((1-s)\,a_0+s\,a_0^*\)\\
	&\qquad
		+(1-s)\,\Bigl((1-r)\,a_0^\#\nabla^{\overline V^1}
			+r\,\(\nabla^{\overline V^0}+v\,a_1^0\)\Bigr)
		\oplus\(\nabla^{\overline V^1}+rva_1^1\)\\
	&\kern5em
		+s\,\Bigr((1-r)\,a_{0\#}^*\nabla^{\overline V^1}\)
			+r\,\(\nabla^{\overline V^0}+v\,a_1^{0*}\)\Bigr)
			\oplus\(\nabla^{\overline V^1}+rva_1^{1*}\)\\
	&\qquad
		-2\,(1-s)v
			\,a_0^{-1}\,\(\nabla^{\overline V^1}+ra_1^1\)^2
		-2\,sv
		\,\(\nabla^{\overline V^1}+ra_1^{1*}\)^2\,(a_0^*)^{-1}\;.
\endsplit\Formel\DreiAslFamilyDef
\endalign$$

We state some elementary properties of these superconnections.

\Proposition\FamilyAslProp.
The superconnections\/~$\^1\Asl$, $\^2\Asl$ and\/~$\^3\Asl$ above
satisfy the following properties.
\roster
\item
We have\/~$\^1\Asl|_{t=1}=\^2\Asl|_{u=1}$
and\/~$\^2\Asl|_{u=0}=\^3\Asl|_{v=1}$.
\item
The zero degree term of\/~$\^1\Asl^2$
with respect to~$N^B$ is given by~${t\over4}\,[a_0,a_0^*]$.
\item
The zero degree terms of\/~$\^3\Asl|_{s=0}$, $\^3\Asl|_{s=1}$
and\/~$\^3\Asl|_{v=0}$ are nilpotent.
\item
The curvatures of\/~$\^1\Asl|_{s=0}$, $\^1\Asl|_{s=1}$
and\/~$\^2\Asl|_{s=0}$, $\^2\Asl|_{s=1}$
do not contain the exterior variable~$dr$.
\endroster

\Proof
Claims~(1), (2) and~(3) are immediate from the definitions
and \FlatSupConnLemma.

To prove~(4),
note that at~$s=0$,
we have
$$\align
	\^1\Asl^2|_{s=0}
	&=\biggl[\biggl({t\over4}\biggr)\hochhalb{N^V}
			\,A'\,\biggl({t\over4}\biggr)\hochmhalb{N^V}
		\,,\;{\sqrt t\over 2}\,a_0^*\biggr]\;,\\
	\Land
	\^2\Asl^2|_{s=0}
	&=\Bigl[2^{-N^V}\,A'\,2^{N^V}
		\,,\;{u\over 2}\,a_0^*\Bigr]\;.\\
\endalign$$
The only term that could involve~$dr$ is in both cases a multiple of
	$$\bigl[a_0^{-1}\,a_1^1\,dr\,,\;\,a_0^*\bigr]\;.$$
But the only nozero components of~$a_0^{-1}\,a_1^1\,dr$ and~$a_0^*$
map~$V^1$ to~$V^0$,
so the supercommutator vanishes.
Clearly, a similar statement holds at~$s=1$.
\qed\enddemo


\Abschnitt\AltCompSubsection A comparison of two finite-dimensional
higher torsions

In this subsection,
we describe how we can use the above superconnections
to construct and compare the two higher torsions
of~\TwoTorsionsFormel\ in \AltCompProp.
This allows us to compare the definitions of \TorsionKapitel\
with those of Bismut and Lott in~\BL\ in~\AltFamRem~(2).
It also gives an expression for~$T\(\nabla^V,A',g^V\)$
as a sum of four terms.
Our strategy in the proof of \IgleichMVBThm\
will be a comparison of each of these terms
with one term in Igusa's definition of~$\tau$,
which  will take the remainder of this section.

We start by constructing some elements in~$\Omega^*(B;\End V^0)$
from the coefficient of the original superconnections~$A'$ and its dual.
These elements are used by Igusa to construct certain correction terms.
If we write~$A'=a_0+(\nabla^{V^0}+a_1^0)\oplus(\nabla^{V^1}+a_1^1)+a_2$
as before,
we set
$$\alignat3
	x&=a_0^{-1}\,\bigl[\nabla^V,a_0\bigr]\;,
		&\qquad
	y&=-a_1^0\;,
		&\qquad
	z&=-a_2a_0=\(\nabla^{V^0}+a_1^0\)^2\;,
	\Formel\IgusaXYZDef\\
		\Land
	x^*&=\bigl[\nabla^V,a^*_0\bigr]\,(a_0^*)^{-1}\;,
		&\qquad
	y^*&=-a_1^{0*}\;,
		&\qquad
	z^*&=-a_0^*a_2^*=\(\nabla^{V^1}+a_1^{0^*}\)^2\;.
\endalignat$$
Here we have used
that~$\nabla^V$ was assumed to be parallel with respect to~$g^V$.
Note that~$x$, $y$, $z$ above
correspond up to sign to the $\End V^0$-valued
forms~$X$, $V$, $W$ in~\IBuch, Section~2.4,
whereas~$x^*$ above corresponds to~$Y$ in~\IBuch.
Igusa's~$U$ can be expressed in terms of~$X$, $V$, $W$ and~$a_0$.

Using flatness of~$A'$ and the Bianchi-Identity,
we can also compute the derivatives of the forms~$x$, $y$, $z$.
With our sign convention, we find
$$\split
	\bigl[\nabla^{V^0},x\bigr]
	&=a_0^{-1}\,\bigl[\nabla^V\,a_0\bigl]
		\,a_0^{-1}\,\bigl[\nabla^V,a_0\bigr]
	=x^2\;,\\
	\bigl[\nabla^{V^0},y\bigr]
	&=-\(\nabla^{V^0}-y\)^2+y^2
	=y^2-z\;,\\
		\Land
	\bigl[\nabla^{V^0},z\bigr]
	&=\bigl[\nabla^{V^0}-y,\(\nabla^{V^0}-y\)^2\bigr]
		+\bigl[y,\(\nabla^{V^0}-y\)^2\bigr]
	=[y,z]\;.
\endsplit\Formel\IgusaDXYZFormel$$
The derivatives of the adjoint forms~$x^*$, $y^*$, $z^*$
are given by similar formulas.

With these preliminaries,
we can give yet another expression of the higher Chern analytic torsion
of \ChernNormDef\ and \ChTorsionThm.
We restrict our attention to classes of forms on~$B$ in degree~$\ge2$,
because we want to ignore all the correction terms in \ChTorsionThm.


\Proposition\AltCompProp.
The higher Bismut-Lott torsion
of\/~$\overline A'|_{r=0}=a_0+a_0^\#\nabla^{V^1}\oplus\nabla^{V^1}$
is up to exact forms given by
$$\split
	T^{\roman{BL}}
		\(\overline A'|_{r=0},g^V\)\dg{\ge2}
	&=-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,t)\in[0,1]\times[1,\infty)}{1\over2}
			\,\strace_V\Bigl(e^{-\^1\Asl^2|_{r=0}}\Bigr)\dg{\ge2}\\
	&\qquad
		-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,u)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^2\Asl^2|_{r=0}}\Bigr)\dg{\ge2}\\
	&\qquad
		-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,v)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^3\Asl^2|_{r=0}}\Bigr)
			\dg{\ge2}\;.
\endsplit\tag1$$
The higher torsion of~$\overline A'|_{r=1}=A'$ is up to exact forms
given by
$$\split
	T\(\nabla^V,A',g^V\)\dg{\ge2}
	&=-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,t)\in[0,1]\times[1,\infty)}{1\over2}
			\,\strace_V\Bigl(e^{-\^1\Asl^2|_{r=1}}\Bigr)\dg{\ge2}\\
	&\qquad
		-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,u)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^2\Asl^2|_{r=1}}\Bigr)\dg{\ge2}\\
	&\qquad
		-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(s,v)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^3\Asl^2|_{r=1}}\Bigr)
			\dg{\ge2}\;.
\endsplit\tag2$$
There is a naturally defined form~$\widetilde T$ such that
$$\split
	T^{\roman{BL}}\(\overline A'|_{r=0},g^V\)\dg{\ge2}\kern-4em
	&\kern4em-T\(\nabla^V,A',g^V\)\dg{\ge2}
	=\(G'+K'-\overline{K'}^*\)\dg{\ge2}+d\widetilde T\;,\\
		\Ltext{with}
	G'&=(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(r,s)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^3\Asl^2|_{v=0}}\Bigr)\;,\\
		\Land
	K'&=-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(r,v)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^3\Asl^2|_{s=0}}\Bigr)\;,\\
%	\overline{K'}^*&=(2\pi i)^{-\textstyle{N^B\over2}}
%		\,\int_{(r,v)\in[0,1]^2}{1\over2}
%			\,\strace_V\Bigl(e^{-\^3\Asl^2|_{s=1}}\Bigr)\;,
\endsplit\tag3$$
where~$\overline{K'}^*$ is constructed as in \BarStarDef.
\parr
The forms~$G'$, $K'$ and~$\overline{K'}^*\in\Omega^*(B)$
are even.
The form~$G'_{2k}$
is the supertrace of a polynomial in~$x$ and~$x^*$ for each~$k$,
and
$$\split
	dG'
	=\cho\(a_0^\#\nabla^{V^0},g^{V^0}\)
		&-(2\pi i)\hochhalb{1-N^B}\int_0^1{1\over2}\,
			\trace_{V^0}\Bigl(x\,e^{r(1-r)\,x^2}\Bigr)\,dr\\
		&+(2\pi i)\hochhalb{1-N^B}\int_0^1{1\over2}\,
			\trace_{V^0}\Bigl(x^*\,e^{r(1-r)\,(x^*)^2}\Bigr)\,dr\;.
\endsplit\tag4$$
The form~$K'_{2k}$
is the supertrace of a polynomial in~$x$, $y$, $z$, and~$w$ for each~$k$,
and
	$$dK'
	=(2\pi i)\hochhalb{1-N^B}\int_0^1{1\over2}\,
			\trace_{V^0}\Bigl(x\,e^{r(1-r)\,x^2}\Bigr)\,dr\;.
	\tag5$$
The form~$\overline{K'}^*_{2k}$
is the supertrace of a polynomial in~$x^*$, $y^*$, $z^*$, and~$w^*$
for each~$k$,
and
	$$d\overline{K'}^*
	=(2\pi i)\hochhalb{1-N^B}\int_0^1{1\over2}\,
			\trace_{V^0}\Bigl(x^*\,e^{r(1-r)\,(x^*)^2}\Bigr)\,dr\;.
	\tag6$$

Note that~$x$, $y$, $z$ do not a priori commute pairwise.
Thus, in each monomial, the order of variables is important.

\Remark\AltFamRem
\roster
\item
This proposition is the first step in a comparison
of Igusa's torsion class~$\tau$ with our~$T$.
The finite-dimensional Bismut-Lott
torsion class~$T^{\roman{BL}}(\overline A'|_{r=0},g^V)$
corresponds to Igusa's class~$F$,
see \IgusaFLemma\ below.
The class~$G'$ corresponds to the class~$G$ in~\IBuch, Chapter~1,
which is called~$K$ in~\IBuch, Chapter~2,
see \IgusaGLemma\ below.
The class~$K'$ corresponds to~$L$ in~\IBuch,
see \IgusaKLemma\ below.
We have chosen to use the letter~$K$ instead,
so that we do not confuse the class~$L$ of~\BGzwei\
and \LDef\ above with Igusa's~$L$.
\item
We want to show that the classes~$G$, $K$, and~$\overline K^*$ together
can be interpreted as an $L$-class in the sense of~\BGzwei, Section~2.
Recall that we defined another superconnection~$\^3\Asl$ in~\DreiAslFormel,
this fits with our present~$\^3\Asl$
along the common domain of definition~$B\times\{1\}^2\times[0,1]^2$,
where~$r=T=1$
and the coordinates of~$[0,1]^2$ are~$s$ and~$v$.
Let us define a family of flat
superconnections~$\bigl({\overline A}{}'_{\ell}\bigr)_{\ell\in[0,1]}$
using~\DreiAslFormel\ and~\DreiAslFamilyDef\ as
	$${\overline A}{}'_\ell
	=\cases
		\^3\Asl|_{(r,s,v)=\left(0,0,3\ell\right)}
			&0\le\ell\le{1\over3}\;,\\
		\^3\Asl|_{(r,s,v)=\left(3\ell-1,0,1\right)}
			&{1\over3}\le\ell\le{2\over3}\;,\Rtext{and}\\
		\^3\Asl|_{(s,T,v)=\left(0,3-3\ell,1\right)}
			&{2\over3}\le\ell\le1\;.
	\endcases$$
Since the coefficient~$a_0$ degenerates at~$\ell=0$ and at~$\ell=1$,
the integral defining the $L$-class
as in \LDef\ and~\ChernNormDef\ diverges in degree~$0$.
Still, we can apply Stokes' theorem to~$B\times D_3$
and proceed as in the proof of \ChTorsionThm\
to find that
$$\align
	\kern2em&\kern-2em
	\(G'+K'-\overline{K'}^*\)\dg{\ge2}\\
	&\equiv{1\over2}\,(2\pi i)\hochmhalb{N^B}
		\,\biggl(-\int_{(s,v)\in[0,1]^2}
			\strace_V\Bigl(e^{-\^3\Asl^2|_{r=0}}\Bigr)
		+\int_{(r,s)\in[0,1]^2}
			\strace_V\Bigl(e^{-\^3\Asl^2|_{v=1}}\Bigr)\\
	&\kern8em
		+\int_{(s,v)\in[0,1]^2}
			\strace_V\Bigl(e^{-\^3\Asl^2|_{r=1}}\Bigr)
		\biggr)\dg{\ge2}\\
\noalign{\smallskip}\allowdisplaybreak
	&\equiv{1\over2}\,(2\pi i)\hochmhalb{N^B}
		\,\biggl(-\int_{(s,v)\in[0,1]^2}
			\strace_V\Bigl(e^{-\^3\Asl^2|_{r=0}}\Bigr)
		+\int_{(r,s)\in[0,1]^2}
			\strace_V\Bigl(e^{-\^3\Asl^2|_{v=1}}\Bigr)\\
	&\kern8em
		+\int_{(s,T)\in[0,1]^2}
			\strace_V\Bigl(e^{-\^3\Asl^2|_{v=1}}\Bigr)
		\biggr)\dg{\ge2}\\
\noalign{\smallskip}
	&=-L_{\ch}\({\overline A}{}'_\ell,g^V\)\dg{\ge2}
\endalign$$
modulo exact forms.
This allows us to compare the finite-dimensional Bismut-Lott torsion
classes with our torsion classes of \MVBTorsionDef\ and \TChRem\ by
	$$%T\(A',g^V,h^V\)=
	T\(\nabla^V,A',g^V\)
	=T^{\roman{BL}}\(a_0+a_0^\#\nabla^{V^1}\oplus\nabla^{V^1},g^V\)
		+L_{\ch}\({\overline A}{}'_\ell,g^V\)\dg{\ge2}\;.
	\Formel\BLgleichMVBFormel$$
\endroster
\endremark


\demo{Proof \rm of \AltCompProp}
We recall that by \ChBLTorCor\ and \AxNullRem,
we have
	$$T^{\roman{BL}}\(\overline A'|_{r=0},g^V\)
	=T\(a_0^\#\nabla^{V^1}\oplus\nabla^{V^1},\overline A'|_{r=0},g^V\)\;.$$
Now, our claims~(1) and~(2) are simple consequences of \ChTorsionThm\
and the definitions of~$\^1\Asl$, $\^2\Asl$ and~$\^3\Asl$
in~\EinsAslFamilyDef, \ZweiAslFamilyDef\ and~\DreiAslFamilyDef.

To prove assertion~(3),
we apply Stokes theorem.
We use~(1) and~(2) to find that
$$\split
	T\(\nabla^V,A',g^V\)\dg{\ge2}\kern-2em
	&\qquad-T^{\roman{BL}}\(\overline A'|_{r=0},g^V\)\dg{\ge2}\\
	&=-(2\pi i)\hochmhalb{N^B}\lim_{T\to\infty}
		\int_{(s,t)\in[0,1]\times[1,T]}{1\over2}\,\biggl(
			\strace_V\Bigl(e^{-\^1\Asl^2|_{r=1}}\Bigr)
				-\strace_V\Bigl(e^{-\^1\Asl^2|_{r=0}}\Bigr)
			\biggr)\\
	&\qquad-(2\pi i)\hochmhalb{N^B}
		\int_{(s,u)\in[0,1]^2}{1\over2}\,\biggl(
			\strace_V\Bigl(e^{-\^2\Asl^2|_{r=1}}\Bigr)
				-\strace_V\Bigl(e^{-\^2\Asl^2|_{r=0}}\Bigr)
			\biggr)\\
	&\qquad-(2\pi i)\hochmhalb{N^B}
		\int_{(s,v)\in[0,1]^2}{1\over2}\,\biggl(
			\strace_V\Bigl(e^{-\^3\Asl^2|_{r=1}}\Bigr)
				-\strace_V\Bigl(e^{-\^3\Asl^2|_{r=0}}\Bigr)
			\biggr)\;.
\endsplit\Formel\AltCompFormelEins$$

We now investigate the integrals
over the remaining faces of~$B\times\del\([0,1]^2\times[1,T]\)$
and~$B\times\del\([0,1]^3\)$, respectively.
By \FamilyAslProp~(1),
we have
$$\split
	0&=\int_{(r,s)\in[0,1]^2}{1\over2}\,\biggl(
		\strace_V\Bigl(e^{-\^1\Asl^2|_{t=1}}\Bigr)
			-\strace_V\Bigl(e^{-\^2\Asl^2|_{u=1}}\Bigr)\biggr)\\
	&=\int_{(r,s)\in[0,1]^2}{1\over2}\,\biggl(
		\strace_V\Bigl(e^{-\^2\Asl^2|_{u=0}}\Bigr)
			-\strace_V\Bigl(e^{-\^3\Asl^2|_{v=1}}\Bigr)\biggr)\;.
\endsplit\Formel\AltCompFormelZwei$$
By \FamilyAslProp~(2),
	$$0
	=\lim_{T\to\infty}\int_{(r,s)\in[0,1]^2}{1\over2}\,
		\strace_V\Bigl(e^{-\^1\Asl^2|_{t=T}}\Bigr)
	\Formel\AltCompFormelDrei$$
because~$[a_0,a_0^*]\in\End V$ is invertible.
By \FamilyAslProp~(4),
we find
$$\split
	0&=\int_{(r,t)\in[0,1]\times[1,T]}{1\over2}\,
		\strace_V\Bigl(e^{-\^1\Asl^2|_{s=0}}\Bigr)
	=\int_{(r,t)\in[0,1]\times[1,T]}{1\over2}\,
		\strace_V\Bigl(e^{-\^1\Asl^2|_{s=1}}\Bigr)\\
	&=\int_{(r,u)\in[0,1]^2}{1\over2}\,
		\strace_V\Bigl(e^{-\^2\Asl^2|_{s=0}}\Bigr)
	=\int_{(r,u)\in[0,1]^2}{1\over2}\,
		\strace_V\Bigl(e^{-\^2\Asl^2|_{s=1}}\Bigr)\;.
\endsplit\Formel\AltCompFormelVier$$

By Stokes theorem and~\AltCompFormelEins--\AltCompFormelVier,
$$\split
	T^{\roman{BL}}\(\overline A'|_{r=0},g^V\)\dg{\ge2}\kern-4em
	&\kern4em-T\(\nabla^V,A',g^V\)\dg{\ge2}\\
	&=(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(r,s)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^3\Asl^2|_{v=0}}\Bigr)
			\dg{\ge2}\\
	&\qquad-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(r,v)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^3\Asl^2|_{s=0}}\Bigr)
			\dg{\ge2}\\
	&\qquad+(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(r,v)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^3\Asl^2|_{s=1}}\Bigr)
			\dg{\ge2}\;.
\endsplit\tag3$$
Because
	$$\overline{K'}^*
	=-(2\pi i)^{-\textstyle{N^B\over2}}
		\,\int_{(r,v)\in[0,1]^2}{1\over2}
			\,\strace_V\Bigl(e^{-\^3\Asl^2|_{s=1}}\Bigr)\;,$$
this proves~(3),
with
$$\split
	\widetilde T
	&=(2\pi i)\hochmhalb{N^B+1}
		\int_{(r,s,t)\in[0,1]^2\times[1,\infty)}{1\over 2}
			\,\strace_V\Bigl(e^{-\^1\Asl^2}\Bigr)\\
	&\qquad
	+(2\pi i)\hochmhalb{N^B+1}
		\int_{(r,s,u)\in[0,1]^3}{1\over 2}
			\,\strace_V\Bigl(e^{-\^2\Asl^2}\Bigr)\\
	&\qquad
	+(2\pi i)\hochmhalb{N^B+1}
		\int_{(r,s,v)\in[0,1]^3}{1\over 2}
			\,\strace_V\Bigl(e^{-\^3\Asl^2}\Bigr)\;.
\endsplit$$
	
We want to express~$G'$ in terms of~$x$ and~$x^*$.
The connection~$\^3\Asl|_{v=0}$
acts on~$\overline V^1$ as~$\nabla^{\overline V^1}$,
and on~$\overline V^0$ as
$$\split
	\(\^3\Asl|_{v=0}\)\bigr|_{\overline V^0}
	&=(1-r)\,\Bigl((1-s)\,a_0^\#\nabla^{\overline V^1}
			+s\,a_{0\#}^*\nabla^{\overline V^1}\Bigr)
		+r\,\nabla^{V^0}\\
%	&=\nabla^{\overline V^0}
%		-(1-r)\,\Bigl((1-s)\,\(\nabla^{\overline V^0}
%				+a_0^{-1}\,\nabla^{\overline V^1}\,a_0\)
%			+s\,\(\nabla^{\overline V^0}
%				+a_0^*\,\nabla^{\overline V^1}\,(a_0^*)^{-1}\)
%			\Bigr)\\
	&=\nabla^{\overline V^0}-(1-r)\,\((1-s)\,x+sx^*\)\;.
\endsplit\Formel\AltCompCyclicFormelEins$$
Together with~\IgusaDXYZFormel,
we find that~$\(\^3\Asl|_{v=0}\)^2|_{\overline V^0}$
%$$\multline
%	\(\^3\Asl|_{v=0}\)^2|_{\overline V^0}
%	=(1-r)^2\,\((1-s)\,x+sx^*\)^2\\
%		-(1-r)\((1-s)\,x^2+s\,(x^*)^2+(x-x^*)\,ds\)
%		-\((1-s)\,x+sx^*\)\,dr
%\endmultline\tag\FormelNummer\IgusaGCurvatureFormel$$
is an element of the subalgebra of~$\Omega^*(B;\End V^0)$
generated by~$x$, $x^*$ and~$r$, $s$, $dr$, $ds$.
Because the term~$\^3\Asl^2|_{v=0}$ is of total degree~$2$,
the form~$G'_ k$
is the trace of a polynomial in~$x$, $x^*$
for each~$k$.

By Stokes' theorem
and because~$\^3\Asl|_{v=0}|_{\overline V^1}=\nabla^{\overline V^1}$ is flat,
$$\split
	dG'
	&=(2\pi i)\hochhalb{1-N^B}\int_{s=0}^1{1\over2}\,
		\trace_{V^0}\Bigl(e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{r=0\atop v=0}}}
			-e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{r=1\atop v=0}}}\Bigr)\\
	&\qquad
	-(2\pi i)\hochhalb{1-N^B}\int_{r=0}^1{1\over2}\,
		\trace_{V^0}\Bigl(e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{s=0\atop v=0}}}
			-e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{s=1\atop v=0}}}\Bigr)\;.
\endsplit\Formel\AltCompStokesEins$$
We analyse the right hand side term by term.

At~$r=0$,
we have the connection
	$$\^3\Asl|{}_{{r=0\atop v=0}}\bigr|_{\overline V^0}
	=(1-s)\,a_0^\#\nabla^{\overline V^1}
			+s\,a_{0\#}^*\nabla^{\overline V^1}\;.$$
Note that~$a_{0\#}^*\nabla^{\overline V^1}$
is the adjoint connection of~$a_0^\#\nabla^{\overline V^1}$
wit respect to~$g^{V^0}$ by~\IgusaAnullXDef.
By \ChoDef,
this implies that
$$%\multline
	(2\pi i)\hochhalb{1-N^B}\int_{s=0}^1{1\over2}\,
		\strace_V\Bigl(e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{r=0\atop v=0}}}\Bigr)%\\
%\split
%	&=(2\pi i)\hochhalb{1-N^B}\int_0^1\strace_V
%		\Biggl({a_{0\#}^*\nabla^{\overline V^1}
%				-a_0^\#\nabla^{\overline V^1}\over2}
%			\,e^{s(1-s)\,\left(a_{0\#}^*\nabla^{\overline V^1}
%				-a_0^\#\nabla^{\overline V^1}\right)^2}
%		\Biggr)\,ds\\   &
	=\cho\(a_0^\#\nabla^{V^1},g^{V^0}\)\;.
%	=\cho\(a_0^\#\nabla^{V^1}\oplus\nabla^{V^1},g^V\)
%\endsplit\endmultline\tag\FormelNummer
\Formel\AltCompFormelFuenf$$

At~$r=1$,
the connection~$\^3\Asl|{}_{{r=1\atop v=0}}=\nabla^{\overline V}$
is flat,
and we have
	$$\int_{s=0}^1{1\over2}\,
		\trace_{V^0}\Bigl(e^{\botsmash{-\^3\Asl^2|_{r=1\atop v=0}}}\Bigr)
	=0\;.\Formel\AltCompFormelSechs$$

At~$s=0$,
we find the connection~$\^3\Asl|{}_{{s=0\atop v=0}}\bigr|{}_{\overline V^0}
=\nabla^{\overline V^0}-(1-r)\,x$
with curvature given by
	$$\^3\Asl^2\bigr|{}_{{s=0\atop v=0}}
	=-r(1-r)\,x^2-x\,dr$$
by~\BGZweiInterpolationFormel.
Thus,
we have
	$$-(2\pi i)\hochhalb{1-N^B}\int_{r=0}^1{1\over2}\,
		\strace_V\Bigl(e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{s=0\atop v=0}}}\Bigr)
	=-(2\pi i)\hochhalb{1-N^B}\int_0^1{1\over2}\,
		\trace_{V^0}\Bigl(x\,e^{r(1-r)\,x^2}\Bigr)\,dr\;.
	\Formel\AltCompFormelSieben$$
Passing to adjoints with respect to~$g^{V^1}$ proves the analogous
equation
	$$(2\pi i)\hochhalb{1-N^B}\int_{r=0}^1{1\over2}\,
		\strace_V\Bigl(e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{s=1\atop v=0}}}\Bigr)
	=(2\pi i)\hochhalb{1-N^B}\int_0^1{1\over2}\,
		\trace_{V^0}\Bigl(x^*\,e^{r(1-r)\,(x^*)^2}\Bigr)\,dr\;.
	\Formel\AltCompFormelAcht$$
Now, statement~(4) follows from~\AltCompStokesEins--\AltCompFormelAcht.



The remaining statements are proven analogously.
Since we wish to describe the superconnection~$\^3\Asl|_{s=0}$
and its curvature by elements of~$\Omega^*(B;\End V^0)$,
we use~$a_0$ to identify~$V^1$ with~$V^0$,
and continue to work with two copies of~$V^0$.
We may write~$\^3\Asl|_{s=0}-\nabla^{V^0}\oplus a_{0\#}\nabla^{V^0}$
as a $2\times2$-matrix with coefficients in~$\Omega^*(B;V^1)$ by
	$$\^3\Asl|_{s=0}
	=\pmatrix
		\nabla^{\overline V^0}-(1-r)\,x-rv\,y
		&-2v\,\bigl(\nabla^{\overline V^0}-(1-r)\,x-r\,y\bigr)^2\\
		{v\over2}
		&-\nabla^{\overline V^0}+(1-rv)\,x+rv\,y\endpmatrix\;.
	\Formel\AltCompZushgsMatrix$$
Recall that due to our sign convention,
$a_0^{-1}\,\nabla^{V^1}\,a_0$ is the negative of a connection;
this fact is responsible for the strange signs in the lower right corner.
Together with~\IgusaDXYZFormel,
this shows that the curvature of~$\^3\Asl|_{s=0}$
is a $2\times2$-matrix with coefficients
in the subalgebra of~$\Omega^*(B;\End V^0)$
generated by~$x$, $y$, $z$ and~$r$, $v$, $dr$, $dv$.
Because the term~$\^3\Asl^2|_{v=0}$ of degree~$0$ with respect to~$N^B$
is nilpotent,
	$$\biggl(\int_{(r,v)\in[0,1]^2}
		\strace\Bigl(e^{-\^3\Asl^2|_{s=0}}\Bigr)\biggr)\dg k$$
is the supertrace of a polynomial in~$x$, $y$, $z$
for each~$k$.

We prove~(5) using Stokes' theorem.
We have
$$\split
	dK'
	&=(2\pi i)\hochhalb{1-N^B}\int_{r=0}^1{1\over2}\,
		\strace_V\Bigl(e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{s=0\atop v=0}}}
			-e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{s=0\atop v=1}}}\Bigr)\\
	&\qquad
	-(2\pi i)\hochhalb{1-N^B}\int_{s=0}^1{1\over2}\,
		\strace_V\Bigl(e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{r=0\atop s=0}}}
			-e^{\botsmash{-\left.\^3\Asl^2\right|
				{}_{r=1\atop s=0}}}\Bigr)\;.
\endsplit\Formel\AltCompStokesZwei$$
The contribution from the line with~$s=0$ and~$v=0$
has been given in~\AltCompFormelSieben.
We will show that the three remaining faces of~$\del([0,1]^2)$
do not contribute to~$dK'$.

At~$v=1$, we have the flat superconnection
$$\split
	\^3\Asl\Bigr|{}_{s=0\atop v=1}
	&={1\over2}\,a_0
		+a_0^\#\,\(\nabla^{\overline V^1}+r\,a_1^1\)
			\oplus\(\nabla^{\overline V^1}+r\,a_1^1\)
		-2a_0^{-1}\,\(\nabla^{\overline V^1}+r\,a_1^1\)\\
	&=2\hochmhalb{N^V}\,\overline A'\,2\hochhalb{N^V}\;, %\\
%\noalign{\smallskip}
%	\^3\Asl^2\Bigr|{}_{s=0\atop v=1}
%	&=0
\endsplit$$
by \DreiAslFamilyDef,
so this face does not contribute to~$dK'$.

At~$r=0$ and~$r=1$,
we get
$$\split
	\^3\Asl\Bigr|{}_{r=0\atop s=0}
	&={v\over2}\,a_0
		+a_0^\#\,\nabla^{\overline V^1}
			\oplus\nabla^{\overline V^1}\;,\\
		\Land
	\^3\Asl\Bigr|{}_{r=1\atop s=0}
	&={v\over2}\,a_0
		+\(\nabla^{\overline V^0}+v\,a_1^0\)
			\oplus\(\nabla^{\overline V^1}+v\,a_1^1\)
		+2v\,a_2\;.
\endsplit$$
The curvatures~$\^3\Asl^2\Bigr|{}_{r=0\atop s=0}$
and~$\^3\Asl^2\Bigr|{}_{r=1\atop s=0}$
are constructed only from~$a_0$, $a_1$, and~$a_2$,
which belong to a nilpotent subalgebra of~$\End V$.
Thus,
these two faces do not contribute to~$dK'$ either,
and the only contribution to~$dK'$ stems from
the face~$v=0$,
and was calculated (up to sign) in \AltCompFormelAcht.

Because~$K'$ and~$\overline{K'}^*$ are related by \BarStarDef,
the remaining claims about~$\overline{K'}^*$ follow immediately.
\qed\enddemo





\Abschnitt\IgusaIFSubsection Igusa's classes~$I$ and~$F$

We prove that Igusa's class~$I$ is a variant of the odd Chern class~$\cho$,
and that by transgression,
the class~$F$ equals the Bismut-Lott torsion class~$T^{\roman{BL}}(A',g^V)$.
This is the first step in  the programme outlined in \AltFamRem~(1).
%We recall the definition of Igusa's universal torsion
%class~$\tau\in H^*\Wh^h\(\Cal M_r(\C),U(r)\)$.
%Each single term in Igusa's definition of~$\tau$ is reconstructed
%using transgressed Chern characters as in \BGzwei.
%In a final step,
%we show that~$\tau$ and~$T$ are cohomologous.
%For convenience,
%we work in the normalisation of~\BGzwei\ throughout the rest of this chapter.

%We still work with the acyclic two-index
%Whitehead space~$\Wh^{h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
%introduced in \TwoIndexWhDef.
%We assume that~$R=M_r(\C)$ and that~$G\subset U(r)$,
%so that the tautological complex
%vector bundle~$\Cal V\to\Wh^{h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
%of rank~$r+r$ carries a natural parallel
%metric~$g^{\Cal V}=g^{\Cal V^0}\oplus g^{\Cal V^1}$.
%Since all the following constructions are natural
%under the pull-back operation,
%we may instead work with a unitarily flat vector bundle~$V=V^0\oplus V^1\to B$
%over an arbitary base space~$B$,
%equipped with a flat
%superconnection~$A'=a_0+(\nabla^{V^0}+a_1^0)\oplus(\nabla^{V^1}+a_1^1)+a_2$,
%where at each point of~$b$,
%the coefficients~$a_0$, $a_1^0$, $a_1^1$, $a_2$ are differential forms
%with values in a nilpotent subalgebra of~$\End V_b$,
%see \TChRem~(2) and the comments at the beginning of \AltFamilySubsection.

We start with the classes~$c_{2k+1}$ and~$I_{2k+1}$ defined in~\IBuch,
Section~1.2,
but using the Chern normalisation of \BGzwei.
Let~$V=V^0\oplus V^1\to B$ be a $\Z$-graded complex vector bundle
with~$\rk V^0=\rk V^1=n$,
with a flat connection~$\nabla^V=\nabla^{V^0}\oplus\nabla^{V^1}$
and a parallel metric~$g^V=g^{V^0}\oplus g^{V^1}$.
Let~$a_0\in\Gamma\(B,\Iso(V^0,V^1\)\subset\Omega^0(B;\End^1V)$
be a family of isomorphisms.

Igusa's form~$I_{2k+1}\in\Omega^{2k+1}(B)$
is the real valued differential form given by
	$$I_{2k+1}
	={k!\over2\,(2\pi i)^k\,(2k+1)!}
		\,\trace\Bigl(\((a_0^{\phantom{*}}a_0^*)^{-1}
			\,\bigl[\nabla^1,a_0^{\phantom{*}}a_0^*\bigr]
			\)^{2k+1}\Bigr)\;.\Formel\IgusaIDefinition$$
We put~$I=\sum_{k=0}^\infty I_{2k+1}\in\Omega^\odd(B)$.

The form~$I$ is closed
because its exterior differential is the supertrace of a non-zero even power
of an odd operator.
Note that in order to have the same normalisation as in~\BGzwei,
we have changed the coefficients with respect to~\IBuch.
%In particular, $c_{2k+1}=\cho(d,g^\tau)\dg{2k+1}$,
%where~$g^\tau$ denotes the tautological metric
%and~$d$ denotes the trivial flat connection
%on the trivial bundle~$H^n\times \C^n\to H^n$.
%
%We recall that~$I_{2k+1}$ does not depend on the choice
%of parallel framing, see~\IBuch.
%In fact,
%let~$h=a_0^{\phantom{*}}a_0^*$ be associated to a particular framing.
%If we choose another framing,
%we obtain instead~$h'=g_0\,h\,g_0^*$ for some fixed~$g_0\in\GL(n,\C)$.
%However, $c_{2k+1}$ is invariant under the action of~$\GL(n,\C)$
%by~$h\mapsto g_0\,h\,g_0^*$,
%so the form~$I_{2k+1}$ is indeed well-defined.
Integrating~$I$
and~$\cho(a_0^\#\nabla^{\Cal V^1},g^{\Cal V_0})$ over~$I$
gives simplicial cochains on~$\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
that we still denote by~$I$
and~$\cho(a_0^\#\nabla^{\Cal V^1},g^{\Cal V_0})$.

\Lemma\IgusaILemma.
We have
	$$I
%	=\cho\(a_0^\#\nabla^{V^1}\oplus\nabla^{V^1},g^V\)
	=\cho\(a_0^\#\nabla^{V^1},g^{V^0}\)\;.$$
In particular,
the simplicial cocycles~$I$
and~$\cho(a_0^\#\nabla^{\Cal V^1},g^{\Cal V_0})$
agree on~$\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$.

\Proof
Because~$\nabla^{V^1}$ is selfadjoint with respect to~$g^{V^1}$,
the adjoint connection of~$a_0^\#\nabla^{V^1}$ with respect to~$g^{V^0}$
is given by~$a_{0\#}^*\nabla^{V^1}$,
cf.~\IgusaAnullXDef.
This implies that
	$$\(a_0^\#\nabla^{V^1}\)^*-a_0^\#\nabla^{V^1}
	=a_0^*\,\(a_0a_0^*\)^{-1}\,
		\bigl[\nabla^{V^1},a_0a_0^*\bigr]
		\,(a_0^*)^{-1}\;.$$
Our claims follow because by~\AltCompFormelFuenf, because
$$\align
	I
	&=\int_0^1\trace_{V^1}
		\Biggl({(a_0a_0^*)^{-1}\,
			\bigl[\nabla^{V^1},a_0a_0^*\bigr]\over2}
		\,e^{s(1-s)\textstyle{\left(\(a_0a_0^*\)^{-1}\,
				\left[\nabla^{V^1}
					,a_0a_0^*\right]\right)^2
			\over 2\pi i}}
		\Biggr)\,ds\\
	&=\int_0^1\trace_{V^0}
		\Biggl({\(a_0^\#\nabla^{V^1}\)^*-a_0^\#\nabla^{V^1}\over2}
		\,e^{s(1-s)\textstyle{\left(\(a_0^\#\nabla^{V^1}\)^*
				-a_0^\#\nabla^{V^1}\right)^2
			\over 2\pi i}}
		\Biggr)\,ds
	=\cho\(a_0^\#\nabla^{V^1},g^{V^0}\)\;.\quad\qed
\endalign$$
\enddemo


Using~$I_{2k+1}$,
Igusa defines another class~$F_{2k}$ by transgression in~\IBuch, (1.4).
Let~$\overline B=B\times[0,1]$,
pull~$V$ and~$\nabla^1$ back to~$\overline B$,
and with the coordinate~$u$ of~$[0,1]$,
put
	$$\overline I_{2k+1}
	={k!\over2\,(2\pi i)^k\,(2k+1)!}
		\,\trace\Bigl(\((a_0^{\phantom{*}}a_0^*)^{-u}
			\,\bigl[\,\overline\nabla{}^1,
				(a_0^{\phantom{*}}a_0^*)^u\bigr]
			\)^{2k+1}\Bigr)\;.$$

Igusa's form~$F_{2k}\in\Omega^\even(B)$ is defined as
	$$F_{2k}
	=-\int_{\overline B/B}\overline I_{2k+1}\;.\Formel\IgusaFDefinition$$
We put~$F=\sum_{k=0}^\infty F_{2k}\in\Omega^\even(B)$.

\Remark\IgusaFRem
We note that~$\overline I_{2k+1}$ is closed
and~$\overline I_{2k+1}|_{u=0}$ vanishes identically.
It thus follows from Stokes' theorem that
	$$d\,F_{2k}=\overline I_{2k+1}|_{u=1}-\overline I_{2k+1}|_{u=0}
	=I_{2k+1}\;.$$
\endremark

We define a superconnection of total degree one on~$V\to B$
by
	$$A'_0
	=\overline A'|_{r=0}
	=a_0+a_0^\#\nabla^{V^1}\oplus\nabla^{V^1}\;,
	\Formel\AxNullDef$$
cf.~\AxNullRem.
Let~$T^{\roman{BL}}\(A'_0,g^V\)$ denote the Bismut-Lott torsion form
of~\TwoTorsionsFormel.
As above,
we denote  the corresponding forms and simplicial cochains
on~$\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
by~$F$ and~$T^{\roman{BL}}\(\Cal A'_0,g^{\Cal V}\)$.

\Lemma\IgusaFLemma.
There is a natural form~$\widetilde F\in\Omega^\odd(B)$ such that
	$$F
	=T^{\roman{BL}}\(A'_0,g^V\)+d\widetilde F\;.$$
In particular,
the simplicial cochains~$F$ and~$T^{\roman{BL}}(\Cal A'_0,g^{\Cal V})$
on~$\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$ differ by an exact cochain.

%\Remark\IgusaLRem
%Because~$g^{V^0}$ is not parallel with respect to~$a_0^\#\nabla^{V^1}$,
%the form~$F=T^{\roman{BL}}\(A'_0,g^V\)$ is not closed.
%Igusa corrects this by adding two correction terms whose exterior
%derivative equals~$dF=I$.
%We will show in the following subsections that
%the sum of these correction terms are equal to the
%class~$L_{\ch}\(bigl(1-s)\,a_0^\#\nabla^{V^1}+s\,\nabla^{V^0},g^{V^0}\bigr)$
%up to an exact form.
%By \MVBTorsionRigidityThm,
%this implies that Igusa's torsion class~$\tau\in H^*(\Wh^{h,\{0,1\}})$
%equals~$T^{\roman{BL}}\(A',g^V,h^V\)$ up to an exact form.
%\endremark

\Proof
On the pullback of~$V$ to~$B\times[0,1]$,
consider the metric
	$$\overline g^V
	=\(s\,g^{V^0}+(1-s)\,a_0^\# g^{V^1}\)\oplus g^{V^1}
	=\(s\,g^{V^0}+(1-s)\,g^{V^1}(a_0\punkt,a_0\punkt)\)\oplus g^{V^1}\;.$$
Note that we have not used parallelity of~$g^{V^0}$
in the definitions of~$I$ and~$F$.
Thus, let~$\overline I$,
$\overline F$ and~$T\(\overline A'_0,\overline g^{V^0}\oplus\overline g^{V^1})$
denote the corresponding forms on~$B\times[0,1]$.
Then clearly
	$$\overline F|_{B\times\{0\}}
	=T^{\roman{BL}}\(\overline A'_0,\overline g^V\)|_{B\times\{0\}}
	=0\;.$$
We put
	$$\widetilde F
	=-\int_{s\in[0,1]}\Bigl(\overline F
		-T^{\roman{BL}}\(\overline A'_0,\bar g^V\)\Bigr)\;.$$
Then by \IgusaILemma, \IgusaFDefinition, \IgusaFRem\
and Stokes' Theorem,
we have
$$\align
	F-T^{\roman{BL}}\(A'_0,g^V\)
	&=\Bigl(\overline F-T^{\roman{BL}}\(A'_0,g^V\)\Bigr)\Bigr|_{s=1}\\
	&=\int_{s\in[0,1]}d\Bigl(\overline F
			-T^{\roman{BL}}\(\overline A'_0,\bar g^V\)\Bigr)
		-d\int_{s\in[0,1]}\Bigl(\overline F
			-T^{\roman{BL}}\(\overline A'_0,\bar g^V\)\Bigr)\\
	&=\int_{s\in[0,1]}\Bigl(\overline I
			-\cho\(a_0^\#\nabla^1,\bar g^V\)\Bigr)
		+d\widetilde F
	=d\widetilde F\;.\quad\qed
\endalign$$
\enddemo


\Abschnitt\IgusaPGSubsection Igusa's polynomial~$P$ and the class~$G$

We interpret the classes~$G_{2k}$ of Chapter~1
(respectively~$K_{2k}$ in Chapter~2) of~\IBuch\ in our smooth setting
and show that they equal the classes~$G'_{2k}$ of \AltCompProp.
This follows from  \AltCompProp~(4)
and the acyclicity of a certain cyclic cochain complex
already studied in~\IBuch.


Recall the definition of~$x$, $x^*\in\Omega^1(B;\End V^0)$
in~\IgusaXYZDef.
These forms correspond to~$-x$ and~$y$ in~\IBuch, Lemma~1.3.1.
%This is because by our sign convention,
%	$$x(v)=-a_0^{-1}\,\bigl[\nabla^V_v,a_0\bigr]
%		\Mand
%	x^*(v)=\bigl[\nabla^V_v,a_0^*\bigr]\,(a_0^*)^{-1}$$
%for all~$v\in TB$.
%Note that the formulas for~$\bigl[\nabla^{V^0},x\bigr]$
%and~$\bigl[\nabla^{V^0},x^*\bigr]$ in~\IgusaDXYZFormel\
%fit with Igusa's lemma.
%Moreover
It follows from the proof of \IgusaILemma\ that
	$$I=\cho\(a_0^\#\nabla^{V^1},g^{V^0}\)
	=-(2\pi i)\hochhalb{1-N^B}\int_0^1{1\over 2}
		\,\trace\Bigl((x^*-x)\,e^{s(1-s)\,(x^*-x)^2}\Bigr)\,ds\;.
	\Formel\IgusaIXYFormel$$

The construction of~$G_{2k}$ relies on the existence
of a certain homogeneous polynomial~$P_{2k}$ of degree~$2k$
with
	$$d\,\trace\(P_{2k}(x,x^*)\)
	={k!\over2\,(2k+1)!}\,
		\Bigl(\trace\((x^*)^{2k+1}\)-\trace\(x^{2k+1}\)
			-\trace\((x^*-x)^{2k+1}\)\Bigr)\;.
		\Formel\IgusaGPolynom$$
Note that~$x$ and~$x^*$ do not commute,
so the order of the~$x$es and~$x^*$s in each monomial is important.
There will in general be several monomials with the same number of~$x$es
and~$x^*$s involved.

We recall the definition of the polynomials~$P_{2k}$ in~\IBuch, Section~1.3.1.
Let~$A=\C\times\C$ be the direct sum of two copies
of the algebra~$\C$,
generated by~$u=(1,0)$ and~$v=(0,1)$.
As in~\IBuch,
we consider the $\Z$-graded cyclic complex
	$$C^*
	=\prod_{j=0}^\infty A^{\otimes(j+1)}\bigm/\((-1)^jz_j-\id\)\;,
		\Formel\IgusaCyclicDef$$
where~$z_j\(a_0\otimes\cdots\otimes a_j\)
=\(a_1\otimes\cdots\otimes a_j\otimes a_0\)$.

Let~$b\colon C^*\to C^{*-1}$ denote the cyclic boundary operator,
	$$b\(a_0\cdots a_j\)
	=\sum_{i=0}^{j-1}(-1)^ia_0\cdots(a_ia_{i+1})
		\cdots a_j
		+(-1)^j\,(a_ja_0)\,a_1\cdots a_{j-1}\;.
	\Formel\IgusaBFormel$$
We define a coboundary operator~$\delta$
by~$\delta u=u\cdot u$, $\delta v=v\cdot v$, and
	$$\delta\(a_0\cdots a_j\)
	=\sum_{i=0}^j(-1)^ia_0\cdots a_{i-1}
		\cdot\delta a_i\cdot a_{i+1}\cdots a_j\;.$$
Clearly~$\delta u^{\punkt k}=u^{\punkt(k+1)}$ if~$k$ is odd
and~$\delta u^{\punkt k}=0$ if~$k$ is even,
and similarly for~$v$.
Let the ``weight''~$w\in\End C^*$ be the linear endomorphism
that multiplies a monomial~$a_0\cdots a_j$
with~$a_i\in\{u,v\}$ for all~$i$
by the number of indices~$i$ modulo~$j+1$,
such that~$a_i\ne a_{i+1}$.
By~\IBuch,
we have
	$$b\circ\delta+\delta\circ b=w\;.
	\Formel\IgusaGHomotopieFormel$$
Note that~$w$ commutes with~$\delta$ and~$b$.
In particular,
the subcomplex generated by all mixed monomials
(i.e., by all monomials of non-zero weight)
is acyclic both with respect to~$b$ and with respect to~$\delta$.

Because~$\delta(v-u)=[v+u,v-u]$,
we have
	$$
	\delta\((v-u)^{2k+1}\)
	=\sum_{i=0}^{2k}(-1)^i(v-u)^i\cdot[v+u,v-u]\cdot(v-u)^{2k-i}=0\;.$$
Similarly,
	$$\delta\(u^{2k+1}\)=\delta\(v^{2k+1}\)=0\;.$$
Igusa defines
	$$P_{2k}(u,v)
	=-{k!\over2\,(2k+1)!}\,{b\over w}\,\((v-u)^{2k+1}
		+u^{2k+1}-v^{2k+1}\)
	\Formel\IgusaPDef$$
in~\IBuch.
Because~$(v-u)^{2k+1}+u^{2k+1}-v^{2k+1}$ contains no mixed monomials,
the polynomial~$P$ satisfies
	$$\del P=-{k!\over2\,(2k+1)!}\,\((v-u)^{2k+1}+u^{2k+1}-v^{2k+1}\)\;.
	\Formel\IgusaPProperty$$
by~\IgusaGHomotopieFormel\ and~\IgusaPhiDFormel.
We put~$P=\sum_{k=1}^\infty P_{2k}$.

There is a $\C$-linear
map~$\phy\colon A\to\Omega^1(B,\End F)$
with~$\phy(u)=x$ and~$\phy(v)=x^*$.
Define
	$$\Phi\colon C^*\to\Omega^*(B)
		\Mtext{with}
	\Phi\(a_0\cdots a_j\)
	=(2\pi i)\hochmhalb{N^B}\trace\(\phy(a_0)\cdots\phy(a_j)\)\;.$$
The sign factor~$(-1)^j$ in~\IgusaCyclicDef\ is compatible with
this construction
because~$x$ and~$y$ are of odd degree.
By~\IgusaCyclicDef,
we clearly have
	$$d\circ\Phi=\sqrt{2\pi i}\,\Phi\circ\delta\;.
	\Formel\IgusaPhiDFormel$$

Igusa's form~$G$ is defined as
	$$G
	=\Phi(P)\;.
	\Formel\IgusaGDefinition$$
%By \AltCompProp~(4), and equations~\IgusaIXYFormel, \IgusaGPolynom,
%both~$G$ and~$G'$ satisfy
%$$\split
%	dG=dG'
%	&=\cho\(a_0^\#\nabla^{V^0},g^{V^0}\)
%		-(2\pi i)\hochhalb{1-N^B}\int_0^1
%			\trace_{V^0}\Bigl(x\,e^{r(1-r)\,x^2}\Bigr)\,dr\\
%	&\qquad+(2\pi i)\hochhalb{1-N^B}\int_0^1
%			\trace_{V^0}\Bigl(x^*\,e^{r(1-r)\,(x^*)^2}\Bigr)\,dr\;.
%\endsplit\Formel\IgusaGProperty$$
Let~$G$ and~$G'$ also denote the cochains
obtained by integrating~$G$ and~$G'$
over each simplex in~$\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$.

\Lemma\IgusaGLemma.
The forms~$G$ and~$G'$ agree
up to the differential of a naturally defined form~$\widetilde G$.
In particular,
the cochains~$G$ and~$G'$ on~$\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
agree up to an exact cochain.

\Proof
We are going to prove the existence of polynomials~$P'_{2k}\in C^{2k}$
in~$u$ and~$v$
with the following properties.
\roster
\item $G'_{2k}=\Phi(P'_{2k})$.
\item $\del P'_{2k}={k!\over2\,(2k+1)!}
\bigl(v^{2k+1}-v^{2k+1}-(v-u)^{2k+1}\bigr)$, and
\item $P'_{2k}$ contains only mixed monomials.
\endroster
In this case,
we concluce that~$\del\(P-P'\)=0$ by~\IgusaPProperty\ and~(2).
Moreover,
by~\IgusaPDef\ and~(3),
the polynomial~$P_{2k}-P'_{2k}$ contains no mixed monomials.
Putting~$\widetilde P={b\over w}\,\(P-P'\)$,
we find~$\del\widetilde P=P-P'$ by~\IgusaGHomotopieFormel.
Using~\IgusaPhiDFormel, \IgusaGDefinition\ and~(1),
our claim follows with~$\widetilde G=(2\pi i)\hochmhalb1
\,\Phi\bigl(\widetilde P\bigr)$,
because
	$$d\widetilde G
	=\Phi\(\del\widetilde P\)
	=\Phi\(P-P'\)
	=G-G'\;.$$

We work in the algebra~$\Omega^*([0,1]^2,C^*)$.
Let us set
	$$P'
	=\int_{(r,s)\in[0,1]^2}{1\over2}\,
		e^{-{\textstyle(}\delta+d-(1-r)\,\((1-s)\,u+s\,v\)
			{\textstyle)}^2}
	\quad\in\quad C^*\;,
	\Formel\AltPChDef$$
where~$d$ denotes the exterior differential on~$[0,1]^2$.
By \AltCompProp\ and~\AltCompCyclicFormelEins,
we get~(1).

In the proof of \AltCompProp~(4),
we have only used \IgusaDXYZFormel,
and the cyclic properties of the trace.
This implies that all calculations remain valid in~$\Omega^*([0,1]^2;C^*)$,
in particular,
(2) follows from
$$\split
	\delta P'
	&=\int_{(r,s)\in[0,1]^2}{1\over2}\,
		\Bigl[\delta+d-(1-r)\,\((1-s)\,u+s\,v\)\,,\;
		e^{-\left(\delta+d-(1-r)\,\((1-s)\,u+s\,v\)\right)^2}\Bigr]\\
	&\qquad
	-\int_{(r,s)\in[0,1]^2}{1\over2}\,\Bigl[d\,,\;
		e^{-\left(\delta+d-(1-r)\,\((1-s)\,u+s\,v\)\right)^2}\Bigr]\\
	&=-\int_0^1{v-u\over2}
		\,e^{s(1-s)\,(v-u)^2}\,ds
	+\int_0^1{v\over2}\,e^{r(1-r)\,v^2}\,dr
	-\int_0^1{u\over2}\,e^{r(1-r)\,u^2}\,dr\\
	&=\sum{k!\over2\,(2k+1)!}
		\,\Bigl(v^{2k+1}-u^{2k+1}-(v-u)^{2k+1}\Bigr)\;.
\endsplit\Formel\AltDPChFormel$$

Because positive even powers of~$u$ and~$v$ vanish in~$C^*$,
the polynomial~$P'$ contains only mixed monomials.
This finishes the proof.
\qed\enddemo



\Abschnitt\IgusaQKSubsection Igusa's polynomial~$Q$ and the class~$K$

We translate some definitions of~\IBuch, Chapter~2, to the language
of flat superconnections.
The reader is warned at this point that for compatibility with~\BL,
we work with bundles of cochain complexes.
This means that the bundles~$C_0$, $C_1$ of~\IBuch\
are now named~$V^1$ and~$V^0$.
This is compatible with our definitions
in Subsections~\SubsectionLetter\IgusaIFSubsection\
and~\SubsectionLetter\IgusaPGSubsection.

Let~$V^0$, $V^1\to B$ be flat bundles with connection~$\nabla$,
let~$f\colon V^0\to V^1$ be a vector bundle isomorphism.
Igusa assumes that for nearby points~$p$, $q\in B$,
there are smooth families~$E^0$, $E^1$
of isomorphisms~$E^i(p,q)\colon V^i(q)\to V^i(p)$
with~$E^i(q,p)=\(E^i(p,q)\)^{-1}$ such that
$$\CD
	V^1(p)		@<E^1(p,q)<<	V^1(q)\\
	@Af(p)AA			@Af(q)AA\\
	V^0(p)		@<E^0(p,q)<<	V^0(q)
\endCD\Formel\IgusaIsomorphismFormula$$
commutes.

Igusa also assumes that there is a family~$S$
of linear maps~$S(p,q,r)\colon V^1(r)\to V^0(p)$
for nearby points~$p$, $q$, $r\in B$
such that
\NeueFormel\IgusaHomotopyFormula
$$\split
	S(p,q,r)\,f(r)
	&=E^0(p,q)\,E^0(q,r)-E^0(p,r)\;,
		\Rand\\
	f(p)\,S(p,q,r)
	&=E^1(p,q)\,E^1(q,r)-E^1(p,r)\;.
\endsplit\HierFormel\IgusaHomotopyFormula$$
Moreover,
he requires the following behaviour under permutations of~$p$, $q$, $r$:
	$$S(q,p,r)=-E^0(q,p)\,S(p,q,r)\;,
		\Mand
	S(p,r,q)=-S(p,q,r)\,E^1(r,q)\;.
		\Formel\IgusaPermutationFormula$$
Igusa demands that the coefficients of~$f$, $E^0-\id$, $E^1-\id$ and~$S$
are given by upper triangular matrices with respect to some local bases
of~$V$.
This corresponds to property~(3) in \MVBDef.

We use the data~$f$, $E$ and~$S$ to construct a flat superconnection
of total degree~$1$.
We denote by~$\nabla^{V^i,q}$, $\nabla^{V^i,r}$ the derivation
with respect to the variables~$q$ and~$r\in B$.
Then we define~$a_0\in\Hom(V^0,V^1)$, $a_1^i\in\Omega^1\(B;\End(V^i)\)$
and~$a_2\in\Omega^2\(B;\Hom(V^1,V^0)\)$ by
$$\align
	a_0(p)
	&=f(p)\;,\\
	a_1^i(p)(X)
	&=\nabla^{V^i,q}_X\bigr|_{q=p}E^i(p,q)\;,\\
		\Land
	a_2(p)(X,Y)
	&=-\(\nabla^{V,q}_X\,\nabla^{V,r}_Y
		-\nabla^{V,q}_Y\,\nabla^{V,r}_X
		-\nabla^{V,r}_{[X,Y]}\)\bigr|_{r=q=p}S(p,q,r)\;,
\endalign$$
and define a superconnection of total degree~$1$ on~$V=V^0\oplus V^1$ by
	$$A'=\nabla+a_0+a_1+a_2\;.
	\Formel\IgusaAeinsFormel$$
Then the coefficients of~$A'$ are all strictly upper triangular.

\Proposition\IgusaFlatnessProposition.
The superconnection~$A'$ is flat.

\Proof
Note that~$A'$ is of total degree~$1$,
so~$(A')^2$ could have contributions in~$\Omega^k\(B,\End V^*\)$,
where~$k=1$, $2$, $3$.

Because~$E(q,p)=E(p,q)^{-1}$, we have~$E(p,p)=\id$.
We derive~\IgusaIsomorphismFormula\ with respect to~$q$ at~$q=p$ and obtain
	$$0
	=\nabla^{V,q}_X\bigr|_{q=p}\(E(p,q)\,f(q)
		-f(p)\,E(p,q)\)
	=\bigl[\nabla+a_1,a_0\bigr](p)\;,
	\Formel\IgusaFeinsFormel$$
so~$(A')^2$ has no component in degree~$1$.

By~\IgusaPermutationFormula, we have~$S(p,p,q)=S(p,q,q)=0$.
We derive \IgusaHomotopyFormula\ twice,
and find
$$\multline
	0=\(\nabla^{V,q}_X\,\nabla^{V,r}_Y
		-\nabla^{V,q}_Y\,\nabla^{V,r}_X
		-\nabla^{V,r}_{[X,Y]}\)\bigr|_{r=q=p}\\
	\(E(p,q)\,E(q,r)-E(p,r)-f(p)\,S(p,q,r)-S(p,q,r)\,f(r)\)\\
	=\((\nabla^V+a_1)^2+[a_0,a_2]\)(p)(X,Y)\;,
\endmultline\tag\FormelNummer\IgusaFzweiFormel$$
so the homogeneous component of~$(A')^2$ of degree~$2$ vanishes, too.

As in the proof of \FlatSupConnLemma,
the Bianchi identity for~$\nabla+a_1$ and equations~\IgusaFeinsFormel\
and~\IgusaFzweiFormel\ imply
that~$(A')^2$ has no component in degree~$3$ either.
This proves the Proposition.
\qed\enddemo


\Remark\IgusaFunctorRem
%On the other hand, given a flat superconnection as in~\IgusaAeinsFormel,
%we can reconstruct the data~$E$ and~$S$ at least near the principal diagonal,
%however, there are some choices involved.
%However, we only need the derivatives~$a_1$ of~$E$ and~$a_2$ of~$S$
%in order to construct Igusa's torsion forms.
%
In other words,
there is a functor from Igusa's category~$\Cal W^\diff\(\C^m,n\)$
introduced in~\IBuch, Chapter~2.2,
to our category~$\cWh^{\diff,h,\{0,1\}}\(R,G\)$.
Igusa proved that~$\Cal W^\diff\(\C^m,n\)$
is homotopy equivalent to the category~$\cWh^{\simp,h,\{0,1\}}\(R,G\)$.
It is easy to check that these functors are compatible
with the homotopy equivalences constructed in \WhHomEqThm.

Moreover,
the final correction term~$K$ (called~$L$ in~\IBuch)
is constructed using the variables~$x$, $y$, $z$ of \IgusaXYZDef\
that are defined using the coefficients of the superconnection~$A'$.
In Igusa's notation in~\IBuch, Section~2.4.1,
we have~$X=x$, $V=-y$, and~$W=z$.
The form~$U\in\Omega^1(B,\End V^1)$
can be represented by~$U=a_0\,(y-x)\,a_0^{-1}$,
however,
a careful analysis of Igusa's construction shows
that~$U$ is not really used in the definition of~$K$.
It is now clear from the above
that Igusa's torsion class on~$\Cal W^\diff\(\C^m,n\)$
pulls back from~$\cWh^{\diff,h,\{0,1\}}\(R,G\)$.
\endremark

The construction of~$K$ relies on a sequence
of homogeneous polynomials~$Q_{2k}$ in~$x$, $y$, $z$ of degree~$2k$,
where~$\deg x=\deg y=1$ and~$\deg w=2$.
These polynomials should satisfy
	$$d\,\trace\(Q_{2k}(x,y,z)
	={k!\over2\,(2k+1)!}\trace\(x^{2k+1}\)\;.$$
Again,
the order of the variables in each monomial is important.

Let us recall some details of the construction of~$Q$ in~\IBuch.
We consider the subalgebra~$A\subset M_3(\C)$ generated by the elements
	$$o=\spmatrix 1\\&0\\&&0\endspmatrix\;,\qquad
	p=\spmatrix 0\\&0\\&&1\endspmatrix\;,\Mand
	q=\spmatrix 0\\&0&1\\&&0\endspmatrix\;.$$
This is a subalgebra of the algebra used in~\IBuch, Section~2.4.1,
where~$o$, $p$, and~$q$ correspond to the generators~$x$, $v$, $w$ in~\IBuch.
The corresponding algebra in~\IBuch\ has another generator~$u$,
however, $u$ is never used in~\IBuch,
so we do not introduce a name for it here.
We assign degrees~$\abs o=\abs p=1$ and~$\abs q=2$.
As in~\IBuch, Section~2.4.1,
we consider a new cyclic complex
$$\split
	C^*
	&=\prod_{j=0}^\infty A^{\otimes(j+1)}\big/(z_j-\id)\;,\\
		\Ltext{where}
	z_j\(a_0\otimes\cdots\otimes a_j\)
	&=(-1)^{\abs{a_0}\,(\abs{a_1}+\dots+\abs{a_j})}
		\,(a_1\otimes\cdots\otimes a_j\otimes a_0)\;.
\endsplit\Formel\IgusaKCyclicDef$$

We define a coboundary operator~$\delta$ on generators by
	$$\delta o=o\cdot o\;,
		\qquad
	\delta p=p\cdot p-q\;,
		\Mand
	\delta q=p\cdot q-q\cdot p\;,
		\Formel\IgusaKDDef$$
and in general by
	$$\delta(a_0\cdots a_j)
	=\sum_{i=0}^j(-1)^i
		\,a_0\cdots a_{i-1}\cdot\delta a_i\cdot a_{i+1}\cdots a_j\;.$$
Then~$\delta$ increments the total degree by~$1$.
Let~$b$ be the cyclic boundary operator given as in~\IgusaBFormel,
%$$\split
%	b(a_0\cdots a_j)
%	&=\sum_{i=0}^{j-1}(-1)^{\abs{a_0}+\dots+\abs{a_{i-1}}}
%			\,a_0\cdots(a_ia_{i+1})\cdots a_j\\
%	&\qquad
%		+(-1)^{\abs{a_j}\,(\abs{a_0}+\dots+\abs{a_{j-1}})}
%			\,(a_ja_0)\cdot a_1\cdots a_{j-1}\;.
%\endsplit$$
and note that~$b$ decrements the total degree by~$1$
because~$q\cdot q=0$.
Let~$w\in\End C^*$ be the {\em colour weight\/}
that multiplies each monomial~$a_0\cdots a_j$
by twice the number of indices~$i$ modulo~$j+1$
such that~$a_i=o$ and~$a_{i+1}\ne o$.
It is proved in~\IBuch, Lemma~2.4.2,
that
	$$b\circ\delta+\delta\circ b=w\;.\Formel\IgusaKHomotopieEins$$
Note that~$w$ commutes with~$b$ and~$\delta$,
and that the subcomplex spanned by all mixed monomials~$a_0\cdots a_j$
is acyclic.
Here, a monomial is called {\em mixed\/}
iff~$a_i=o$ for at least one index~$i$,
and~$a_k\ne o$ for at least one index~$k$,
i.e.,
iff~$w(a_0\cdots a_j)\ne 0$.

We now regard the subcomplex~$(C^{\prime *},\delta)\subset(C^*,\delta)$
spanned by~$p$ and~$q$.
It follows that if a monomial has colour weight~$w=0$,
then it is either of the form~$x^{2k+1}$,
or it belongs to~$C^{\prime *}$.
By \IgusaKDDef,
the subcomplex~$C^{\prime *}$ admits a filtration
	$$C^{\prime *}
	=F^{\prime 0}\supset F^{\prime 1}\supset\dots\;,
		\Formel\IgusaKFiltration$$
where~$F^{\prime k}$ is spanned by all monomials in~$p$ and~$q$
that contain~$q$ at least $k$ times.
As in~\IBuch,
we may write~$\delta|_{C^{\prime *}}=\delta'+\delta''$,
where
$$\alignat 3
	\delta'&\colon F^{\prime k}\to F^{\prime k}\;,&
		\Mtext{with}
	p&\mapsto p^2\;,\qquad&
	q&\mapsto pq-qp\;,\\
		\Land
	\delta''&\colon F^{\prime k}\to F^{\prime k+1}\;,&
		\Mtext{with}
	p&\mapsto -q\;,\qquad&
	q&\mapsto 0\;.
\endalignat$$

We define a new cyclic boundary operator~$b'$ on~$C^{\prime *}$
of total degree~$-1$ by
$$\split
	b'(a_0\cdots a_j)
	&=\sum_{i=0}^{j-1}(-1)^{\abs{a_0}+\dots+\abs{a_{i-1}}}
			\,a_0\cdots(a_i*a_{i+1})\cdots a_j\\
	&\qquad
		+(-1)^{\abs{a_j}\,(\abs{a_0}+\dots+\abs{a_{j-1}})}
			\,(a_j*a_0)\cdot a_1\cdots a_{j-1}\;,
\endsplit$$
which is on generators given by
	$$p*p=p\;,\qquad p*q=q*p=q\;,\Mand q*q=0\;.$$
Let~$w'$ be the weight operator that multiplies each monomial~$a_0\cdots a_j$
by the number of indices~$i$ modulo~$j+1$
such that~$a_i=p$, $a_{i+1}=q$.
Then it it proved in~\IBuch, Lemma~2.4.4, that
	$$b'\circ\delta'+\delta'\circ b'=-w'\;.
		\Formel\IgusaKHomotopieZwei$$
Because the only monomial of weight~$w'=0$ of total degree~$2k+1$
is~$v^{2k+1}$,
a simple spectral sequence argument gives
	$$H^{\odd}\(F^{\prime k},\delta\)=0
		\Rtext{for all~$k\ge 1$.}
	\Formel\IgusaCxAcyclicity$$

Note that~$C^*$ admits an involution~$\iota$ given by
	$$o\buildrel\iota\over\longleftrightarrow -o\;,\qquad
	p\buildrel\iota\over\longleftrightarrow p-o\;,\Mand
	q\buildrel\iota\over\longleftrightarrow q\;.
		\Formel\IgusaKiotaDef$$
To show that~$\iota$ is a cochain map,
note that
	$$\delta\buildrel\iota\over\longleftrightarrow\delta-[o,\punkt]$$
on generators,
however
$$\multline
	\sum_i(-1)^{\abs{a_0}+\dots+\abs{a_{i-1}}}
		\,a_0\cdots a_{i-1}\cdot\(\delta a_i-o\cdot a_i
			-(-1)^{\abs{a_i}}a_i\cdot o\)
		\cdot a_{i+1}\cdots a_j\\
	=\sum_i(-1)^{\abs{a_0}+\dots+\abs{a_{i-1}}}
		\,a_0\cdots a_{i-1}\cdot\delta a_i
		\cdot a_{i+1}\cdots a_j\;,
\endmultline$$
so the action of~$\delta$ on~$C^*$ commutes with~$\iota$.
However,
the multiplication on~$A$ and thus the operators~$b$ and~$w$ are changed.
In fact,
the involution~$\iota$ corresponds to passing from the superconnection~$A'$
of degree~$1$
to a superconnection
	$$a_0^{-1}+\(\nabla^{V^0}+a_1^0\)\oplus\(\nabla^{V^1}+a_1^1\)
		a_0\,a_2\,a_0$$
of degree~$-1$.

Finally,
we define a linear map~$\phy\colon A\to\Omega^*(B;\End V^0)$
on generators by~$\phy(o)=x$, $\phy(p)=y$, and~$\phy(q)$.
%	$$\phy(o)=x=a_0^{-1}\,\bigl[\nabla^{V^0},a_0\bigr]\;,
%		\qquad
%	\phy(p)=y=-a_1^0\;,
%		\Mand
%	\phy(q)=z=-a_2a_0\;.$$
Define
	$$\Phi\colon(C^*,\delta)\to(\Omega^*(B),d)
		\Mtext{by}
	\Phi\(a_0\cdots a_j\)
	=(2\pi i)\hochmhalb{N^B}\,\trace\(\phy(a_0)\cdots\phy(a_1)\)\;.
		\Formel\IgusaKPhiDef$$
Then by~\IgusaDXYZFormel\ and~\IgusaKDDef,
we have
	$$d\circ\Phi=\sqrt{2\pi i}\,\Phi\circ\delta\;.
		\Formel\IgusaPhiDFormelZwei$$

The map~$\Phi$ has a large kernel.
We note that~$\phy(p)=a_1^0$ and~$\phy(q)=a_2a_0$
are strictly triangular with respect to the eigenspaces of~$h^{V^0}$.
We also note that
	$$\phy(o-p)
	=\(\nabla^{V^0}+a_1^0\)+a_0^{-1}\,\nabla^{V^1}\,a_0
	=-a_0^{-1}\,a_1^1\,a_0$$
and~$\phy(q)=a_0^{-1}\,(a_0a_2)\,a_0$
are strictly triangular
with respect to the eigenspaces of~$a_0^{-1}h^{V^1}a_0$.
In other words,
	$$C^{\prime *}\subset\ker(\Phi)
		\Mand
	\iota(C^{\prime *})\subset\ker(\Phi)\;.
		\Formel\IgusaKkerPhiFormel$$

As noted after Lemma~2.4.5 in~\IBuch,
Igusa's polynomials~$Q_{2k}$ in our normalisation satisfy
	$$\delta Q_{2k}
	={k!\over 2\,(2k+1)!}\,o^{2k+1}
		+R_{2k+1}-\iota R_{2k+1}
	\Formel\IgusaQProperty$$
for some~$R_{2k+1}\in C^{\prime *}$,
where
	$$R_{2k+1}\equiv{k!\over2(2k+1)!}\,p^{2k+1}
		\Rtext{modulo }F^{\prime 1}\;.
	\Formel\IgusaRProperty$$

Igusa's form~$K_{2k}$ is defined as
	$$K_{2k}=\Phi(Q_{2k})
		\quad\in\Omega^{2k}\(\Wh^{h,\{0,1\}}\(\Cal M_r(\C),U(r)\)\)\;.
	\Formel\IgusaKDefinition$$
We put~$K=\sum_kK_{2k}$.
%By~\IgusaQProperty,
%	$$dK=dK'
%	=(2\pi i)\hochhalb{1-N^B}\int_0^1{1\over2}
%		\,\trace_{V^0}\Bigl(x\,e^{r(1-r)\,x^2}\Bigr)\,dr\;.
%	\Formel\IgusaKProperty$$
Let~$K$ and~$K'$ also denote the cochains
obtained by integrating~$K$ and~$K'$
over each simplex in~$\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$.


\Lemma\IgusaKLemma.
The forms~$K$ and~$K'$ agree
up to the differential of a naturally defined form~$\widetilde K$.
In particular,
the cochains~$K$ and~$K'$ on~$\cWh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$
agree up to an exact cochain.

\Proof
We want to construct polynomials~$Q'_{2k}\in C^*$
and~$R'_{2k+1}\in C^{\prime*}$
with the following properties.
\roster
\item $K'_{2k}=\Phi(Q'_{2k})$.
\item $\delta Q'_{2k}={k!\over2\,(2k+1)!}\,o^{2k+1}+R'_{2k+1}-\iota R'_{2k+1}$.
\item $R'_{2k+1}\equiv{k!\over2\,(2k+1)!}\,p^{2k+1}$ modulo~$F^{\prime 1}$.
\endroster
Given~$Q'_{2k}$ and~$R'_{2k+1}$ as above,
we proceed as follows.
First, using~\IgusaCxAcyclicity, \IgusaRProperty, and~(3),
we find an even
formal power series~$\widetilde R\in F^{\prime 1}\subset C^{\prime *}$
such that
	$$R-R'=\delta \widetilde R\;.$$
From~\IgusaQProperty\ and~(2) we conclude
that~$\delta\(Q-Q'-\widetilde R+\iota \widetilde R\)=0$.
We let~$(\punkt)\nr{w>0}$ denote the components of colour weight~$\ne 0$
and define
	$$\widetilde K
	=(2\pi i)\hochmhalb{1}\,\Phi\biggl({b\over w}
		\,\(Q-Q'-\widetilde R+\iota\widetilde R\)\nr{w>0}\biggr)\;.$$
By~\IgusaKHomotopieEins, \IgusaPhiDFormelZwei, \IgusaKDefinition\ and~(1),
and because~$o^{2k}=0\in C^*$ for all~$k>0$
and~$C^{\prime *}$, $\iota C^{\prime*}\subset\ker\Phi$ by~\IgusaKkerPhiFormel,
we find that
	$$d\widetilde K
	=\Phi\(Q-Q'-\widetilde R+\iota \widetilde R\)
	=\Phi\(Q-Q'\)
	=K-K'\;,$$
which proves the lemma.

It remains to construct~$Q'$, $R'$ satisfying~(1--3).
Our final formula for~$Q'$
will be the sum of two formal power serieses~$\^1Q'+\^2Q'$,
such that
	$$\Phi(\^1Q')=K'
		\Mand
	\Phi(\^2Q')=0\;,
		\Formel\IgusaQChComponents$$
which implies~(1).
To construct~$\^1Q'$,
we work in~$\Omega^*\([0,1]^2;C^*\)$.
As in~\AltCompZushgsMatrix,
we construct a superconnection
on the trivial bundle with fibre~$(C^*)^2$ by
	$$\^3\Asl'
	=\pmatrix
		d+\delta-(1-r)\,o-rv\,p
		&-2v\,\bigl(d+\delta-(1-r)\,o-r\,p\bigr)^2\\
\noalign{\smallskip}
		v/2
		&-d-\delta+(1-rv)\,o+rv\,p\endpmatrix\;,
	\Formel\AltKEinsAslDef$$
where~$d$ denotes the exterior differential on~$[0,1]^2$.
Again,
the signs in the lower right corner make sense if we agree that
the total degree in the second copy of~$C^*$ is shifted by~$1$.
We can now translate parts of the proof of \AltCompProp~(5).

We set
	$$\^1Q'
	=\int_{(r,v)\in[0,1]^2}{1\over 2}
		\,\strace\Bigl(e^{-\^3\Asl^{\prime 2}}\Bigr)\;.$$
The first equation in~\IgusaQChComponents\
follows from \AltCompProp~(3), \DreiAslFamilyDef,
\IgusaKPhiDef, \AltKEinsAslDef.
By Stokes' theorem,
$$\split
	\delta \^1Q^{\prime*}
	&=\int_{(r,v)\in[0,1]^2}{1\over 2}\,\strace\Bigl(\Bigl[\^3\Asl',
			e^{-\^3\Asl^{\prime 2}}\Bigr]\Bigr)
		-\int_{(r,v)\in[0,1]^2}{1\over 2}
			\,d\strace\Bigl(e^{-\^3\Asl^{\prime 2}}\Bigr)\\
	&=\int_{r=0}^1{1\over2}
			\,\strace\Bigl(e^{-\^3\Asl^{\prime 2}|_{v=0}}
				-e^{-\^3\Asl^{\prime 2}|_{v=1}}\Bigr)
		-\int_{v=0}^1{1\over2}
			\,\strace\Bigl(e^{-\^3\Asl^{\prime 2}|_{r=0}}
				-e^{-\^3\Asl^{\prime 2}|_{r=1}}\Bigr)\;.
\endsplit\Formel\AltKStokesFormel$$

As in~\BGZweiInterpolationFormel, we have
	$$\^3\Asl^{\prime2}|_{v=0}
	=\pmatrix
		d+\delta-(1-r)\,o&0\\
\noalign{\smallskip}
		0&-d-\delta+o\endpmatrix^2
	=\pmatrix
		-r(1-r)\,o^2-o\,dr\\
		&0\endpmatrix\;.$$
Thus,
	$$\int_{r=0}^1{1\over2}
			\,\strace\Bigl(e^{-\^3\Asl^{\prime 2}|_{v=0}}\Bigr)
	=\int_{r=0}^1{o\over2}\,e^{r(1-r)\,o^2}\,dr\;.
	\Formel\AltKFormelEins$$

At~$v=1$, we find
	$$\^3\Asl^{\prime2}|_{v=1}
	=\pmatrix
		d+\delta-(1-r)\,o-r\,p
		&-2\,\bigl(d+\delta-(1-r)\,o-r\,p\bigr)^2\\
\noalign{\smallskip}
		1/2
		&-d-\delta+(1-r)\,o+r\,p\endpmatrix^2
	=0$$
by \FlatSupConnLemma,
so there is no contribution from this side.

The formal connection~$d+\delta-o$ is flat either by~\IgusaKDDef\
or because it corresponds to~$a_0^\#\nabla^{\overline V^1}$.
This implies
	$$\^3\Asl^{\prime2}|_{r=0}
	=\pmatrix
		d+\delta-o
		&0\\
\noalign{\smallskip}
		v/2
		&-d-\delta+o\endpmatrix^2
	=\pmatrix 0\\dv/2&0\endpmatrix\;,$$
so
	$$\int_{r=0}^1{1\over2}
			\,\strace\Bigl(e^{-\^3\Asl^{\prime 2}|_{v=1}}\Bigr)
	=\int_{v=0}^1{1\over2}
			\,\strace\Bigl(e^{-\^3\Asl^{\prime 2}|_{r=0}}\Bigr)
	=0\;.
	\Formel\AltKFormelZwei$$

In the proof of \AltCompProp~(5),
the face~$r=1$ did not contribute because the corresponding curvature
had coefficients in a nilpotent subalgebra of~$\End V$.
We do not have this argument here.
Instead,
the contribution to~$\delta\^1Q'$ at~$r=1$ will be cancelled
by the second polynomial~$\^2Q'$.
To that end,
we define yet another superconnection on~$V\times[0,1]^2$ by
	$$\^4\Asl
	={v\over 2}\,a_0
		+\(\nabla^{V^0}+v\,a_1^0\)\oplus\(\nabla^{V^1}+v\,a_1^1\)
		+2v(1-w)\,a_2\;,$$
and as its preimage under~$\Phi$,
we take
	$$\^4\Asl'
	=\pmatrix
		d+\delta-v\,p
		&-2v(1-w)\,\bigl(d+\delta-p\bigr)^2\\
\noalign{\smallskip}
		v/2
		&-d-\delta+(1-v)\,o+v\,p\endpmatrix\;.
	\Formel\AltKEinsAslDef$$
We set
	$$\^2Q'
	=\int_{(w,v)\in[0,1]^2}{1\over2}
		\,\strace\Bigl(e^{-\^4\Asl^{\prime 2}}\Bigr)\;.$$
Note that the definition of~$\^4\Asl$ only involves the coefficients~$a_0$,
$a_1^0$, $a_1^1$ and~$a_2$,
which are all strictly triangular with respect to~$h^V$.
This gives the second equation in~\IgusaQChComponents.

The analogue of~\AltKStokesFormel\ holds for~$\delta\^2Q'$.
One easily checks that
	$$\^3\Asl'|_{r=1}=\^4\Asl'|_{w=0}\;,$$
so the contributions to~$\delta\^1Q'$ at~$r=1$
and  to~$\delta\^2Q'$ at~$w=0$ cancel
as announced above.

We recall that by~\IgusaKDDef,
the formal connection~$d+\delta-p$ has curvature~$q$.
At~$v=1$,
we thus have
	$$\^4\Asl^{\prime 2}
	=\pmatrix
		d+\delta-p
		&-2(1-w)\,q\\
\noalign{\smallskip}
		1/2
		&-d-\delta+v\,p\endpmatrix^2
	=\pmatrix
		w\,q&*\\
\noalign{\smallskip}
		0&w\,q
	\endpmatrix\;.$$
Because this matrix is triangular
and the diagonal terms do not involve~$dw$,
there will be no contribution to~$\delta\^2Q'$ from the side~$v=1$.
At~$v=0$,
things are even simpler because~$\^4\Asl'$ is evidently flat.
So,
we find
	$$\int_{w=0}^1{1\over2}
		\,\strace\Bigl(e^{-\^4\Asl^{\prime 2}|_{v=0}}\Bigr)
	=\int_{w=0}^1{1\over2}
		\,\strace\Bigl(e^{-\^4\Asl^{\prime 2}|_{v=1}}\Bigr)
	=0\;.
	\Formel\AltKFormelDrei$$

Finally, at~$w=1$,
we compute
$$\split
	\^4\Asl^{\prime 2}
	&=\pmatrix
		d+\delta-v\,p
		&0\\
\noalign{\smallskip}
		v/2
		&-d-\delta+o+v\,(p-o)\endpmatrix^2\\
	&=\pmatrix
		-v(1-v)\,p^2+v\,q+p\,dv&0\\
\noalign{\smallskip}
		*&-v(1-v)\,(p-o)^2+v\,q+(p-o)\,dv
	\endpmatrix\;.
\endsplit$$
Let us define
	$$R'=\int_0^1{p\over2}\,e^{r(1-r)\,p^2-r\,q}\,dr\;,$$
then by~\IgusaKiotaDef, we find
	$$\int_{v=0}^1{1\over2}
		\,\strace\Bigl(e^{-\^4\Asl^{\prime 2}|_{w=1}}\Bigr)
	=-R'+\iota R'\;.
	\Formel\AltKFormelVier$$

Combining equations~\AltKStokesFormel--\AltKFormelZwei,
\AltKFormelDrei, \AltKFormelVier,
we obtain~(2).
%find that
%	$$\delta Q'
%	=\delta\(\^1Q'+\^2Q'\)
%	=\int_0^1{o\over2}\,e^{r(1-r)\,o^2}\,dr
%		+R'-\iota R'$$
%as requested in~\IgusaQchProperty.
Moreover, $R'$ clearly satisfies~(3).
%Moreover, we have
%	$$R'\equiv\int_0^1{p\over2}\,e^{r(1-r)\,p^2}\,dr
%		\Rtext{modulo }F^{\prime 1}$$
%as requested in~\IgusaRchProperty.
%By the arguments after~\IgusaRchProperty,
This finishes the proof of \IgusaKLemma.
\qed\enddemo



\enddocument




\Abschnitt\IgusaSummary A proof of \MainTheoremZwei\ in the acyclic case

We summarize the work of Subsections~\NummerVon\AltFamilySubsection%
--\NummerVon\IgusaQKSubsection\
and give a proof of our main result \MainTheoremZwei\ in the fibre-wise
acyclic case.

Let~$\tau\in H^\even\bigl(\Wh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)\bigr)$
denote Igusa's torsion class.
We recall that
	$$\tau=F-G-K+\overline K^*$$
in our normalisation,
where~$F$, $G$ and~$K$ were constructed
as in~\IgusaFDefinition, \IgusaGDefinition\ and~\IgusaKDefinition.
We also recall Igusa's two-index theorem (\IBuch, Theorem~5.7.1).

\Fact\TwoIndexThm(Two-Index Theorem).
The acyclic  two-index Whitehead space~$\Wh^{h,\{0,1\}}
\penalty0\(\Cal M_r(\C),U(r)\)$
is a deformation retract
of the full acyclic  Whitehead space~$\Wh^{h}\(\Cal M_r(\C),U(r)\)$.

This theorem allows Igusa to extend his definition of~$\tau$
to~$H^\even\bigl(\Wh^{h}\(\Cal M_r(\C),U(r)\)\bigr)$.
On the other hand,
the class~$T\in H^\even\bigl(\Wh^h\(\Cal M_r(\C),U(r)\)\bigr)$
constructed in \TChRGDef\ is compatible with stabilisation,
because it vanishes for the trivial superconnection~$a_0+d\otimes d$
on the trivial bundle~$B\times(\C\oplus\C)$,
where~$a_0$ is the identity from the first to the second direct summand.

Apart from the definition of~$T$,
the main result of the present chapter is the following

\demo{Proof of \IgleichMVBThm}
Both classes~$\tau$ and~$T$
are pulled back from the unstabilised acyclic two-index
pre-Whitehead space~$\Wh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$ in its differential realisation.
Thus it is sufficient to compare them on~$\Wh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$.
Because both classes can be defined by defining certain naturally defined
forms over the simplices of~$\Wh^{\diff,h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$,
it suffices to show that the corresponding forms
differ by the exterior differential of a naturally defined form.
In view of these preliminaries,
our Theorem is proven in degrees~$\ge 2$
by \AltCompProp~(3) and the Lemmata~\NummerVon\IgusaFLemma,
\NummerVon\IgusaGLemma\ and~\NummerVon\IgusaKLemma.
On the other hand,
in degree~$0$,
both torsions coincide with the Franz-Reidemeister torsion
of the complex~$(V,a_0)$ by~\IBuch\ and \MVBTorsionThm.
\qed\enddemo

To prove \MainTheoremZwei,
let us recall Igusa's framing principle (\IBuch, Theorem~6.1.1)
in the special case of a fibre-wise Morse function~$h\colon M\to B$.
We recall that~$\hat p\colon C\to B$ denotes the set of critical points
of~$h$,
that~$T^sX$, $T^uX\to C$ are the stable and unstable vertical tangent bundles,
and that we have defined an additive genus
	$$\^0J={1\over2}\sum_{k\ge 1}\zeta'(-2k)\,\ch\dg{4k}\;.$$

\Fact\IgusasFramingPrinciple(Framing Principle).
Assume that~$F\to M$ is a unitarily flat vector bundle
that is acyclic on the fibre of~$p\colon M\to B$,
and assume that~$h\colon M\to\R$ be a fibre-wise Morse function.
Then the higher Franz-Reidemeister torsion of~$p\colon M\to B$ and~$F\to M$
is given by
	$$\tau(M/B;F)
	=T(A',g^V,h^V)+\hat p_*\((-1)^{\ind_h}\,\^0J$$
\?weiter?



	





==> intro2.tex <==
%auto-ignore
\input morse2.def

\topmatter
\title Morse theory and higher torsion invariants II%\\
%--- Please, do not distribute ---
\endtitle
\author Sebastian Goette\endauthor
\address NWF 1 Mathematik, Universit\"at Regensburg,
93040 Regensburg, Germany\endaddress
\email sebastian.goette\@mathematik.uni-regensburg.de\endemail
\thanks Research at MSRI is supported in part by NSF-grant DMS-9701755\endthanks
\keywords analytic torsion forms, higher Franz-Reidemeister torsion,
Cheeger-M\"uller theorem, Whitehead space,
Witten deformation\endkeywords
\abstract
Let~$p\colon M\to B$ be a family of compact manifolds
equipped with a unitarily flat vector bundle~$F\to M$.
We generalize Igusa's higher Franz-Reidemeister torsion~$\tau(M/B;F)$
to the case that the fibre-wise cohomology~$H^*(M/B;F)\to B$
carries a parallel metric.
If moreover~$M$ admits a fibre-wise Morse function,
we compute the difference of~$\tau(M/B;F)$
and the higher analytic torsion~$\Cal T(M/B;F)$.
We also generalise the examples given in~\TeilEins.





\endabstract
\subjclass\nofrills\rm 2000 \it Mathematics Subject Classification.\/
\rm Primary 58J52; Secondary 57R22, 57Q10\endsubjclass
\endtopmatter

\rightheadtext{Morse theory and higher torsion invariants II}


\document

This is the second of
two papers devoted to a comparison of Igusa's and Klein's
higher Franz-Reidemeister torsion~$\tau$ with
Bismut's and Lott's higher analytic torsion~$\Cal T$.
In the first part~\TeilEins,
we evaluated the Bismut-Lott torsion form~$\Cal T$ for families
that carry a fibre-wise Morse function,
thus extending earlier work with Bismut (\BGzwei).
Here,
we relate~$\tau$ and~$\Cal T$ for families with fibre-wise Morse functions
in those situations where both invariants are defined.
%In a tentative third part,
%we extend the results of the first two papers to general families,
%using Igusa's existence result for framed generalised Morse functions
%(\Iframed).

We start by recalling some notation and results of~\TeilEins.
Let~$p\colon M\to B$ be a family of compact manifolds,
let~$F\to M$ be a flat vector bundle,
and let~$h\colon M\to\R$ be a fibre-wise Morse function.
Then the fibre-wise critical points of~$h$
form a covering~$\hat p\colon C\to B$.
Let~$o(T^uX)\to C$ denote the orientation bundle of the unstable
vertical tangent bundle at~$C$,
and construct a vector bundle
	$$V=\hat p_*\(F|_C\otimes o(T^uX)\)\;.$$
Then~$V$ carries a flat connection~$\nabla^V$ induced by~$\nabla^F$.
In~\TeilEins,
we defined a family Thom-Smale complex by constructing
a flat superconnection~$A'$ on~$V$.
We also constructed a generalised ``integration over the fibre'',
i.e., an $\Omega^*(B)$-linear
cochain map~$I\colon\(\Omega^*(M;F),\nabla^F\)\to\(\Omega^*(B;V),A'\)$.
This cochain map naturally identifies
the fibre-wise cohomology~$H=H^*(M/B;F)\to B$,
equipped with the flat Gau\ss-Manin connection~$\nabla^H$,
with the bundle~$H^*(V,a'_0)\to B$ as follows.
Both~$\Omega^*(M;F)$ and~$\Omega^*(B;V)$ can be filtered by horizontal degree.
The cochain map~$I$ respects these filtrations
and induces isomorphisms of the $E_p$-terms
of the associated spectral sequences for~$p\ge 1$.
The $E_1$-term of both spectral sequences
is isomorphic to~$\(\Omega^*(B;H),\nabla^H\)$.

A metric~$g^F$ on~$F$ induces a metric~$g^V$ on~$V$,
and the Morse function~$h$ induces an endomorphism~$h^V$ of~$V$.
Using these data,
we defined an analytic torsion form
	$$T(A',g^V,h^V)\in\Omega^*(B)\;.$$
The metric~$g^V$ induces a metric~$g^H_V$ on~$H$ by finite-dimensional
Hodge theory.
Let~$\cho(\nabla^F,g^F)$ denote the characteristic form of~$F\to M$
defined in~\BL,
written in the normalisation of~\BGzwei.
Then
	$$dT(A',g^V,h^V)
	=\cho(\nabla^V,g^V)-\cho(\nabla^H,g^H_V).$$
In particular,
$T(A',g^V,h^V)$ generalises the analytic torsion forms on flat families
of chain complexes defined in~\BL.

In order to state the main theorem of~\TeilEins,
let~$T^HM\subset TM$ be a horizontal complement of the vertical
tangent bundle~$TX\to M$ of~$M$,
and let~$g\TX$ be a vertical metric on~$TX$.
Then there exists a unique natural connection~$g\TX$ on~$TX$
which generalises the Levi-Civita connection on a single manifold~$X$.
Let
	$$\Cal T(T^HM,g\TX,\nabla^F,g^F)\in\Omega^*(B)\;.$$
be the analytic torsion form of Bismut and Lott (\BL).
The metrics~$g\TX$ and~$g^F$ induce an $L_2$-metric
on the space~$\Omega^*(M/B;F)$ of fibre-wise differential forms.
By Hodge theory,
we get a metric~$g^H_{L_2}$
by identifying~$H\to B$ with the bundle of fibre-wise harmonic forms.
Let~$\chslo\(\nabla^H,g^H_{L_2},g^H_V)$ be the Chern-Simons class
associated to the characteristic class~$\cho(\nabla^H)$.
Let~$\psi(\nabla\TX,g\TX)$ denote the Matthai-Quillen current
on the bundle~$TX\to M$.
Finally,
we define an additive characteristic class
	$$\^0J={1\over2}\sum_{k\ge 1}\zeta'(-2k)\,\ch\dg{4k}$$
as in~\BGzwei,
where~$\zeta$ is the Riemann zeta function
and~$\ch\dg{4k}$ is the homogeneous part of the Chern class with coefficients
in~$\R$ of degree~$4k$.
The following theorem generalises the main theorem of~\BGzwei,
where we assumed in addition that~$h$
admits a fibre-wise Smale gradient field.

\Theorem\TeilEinsTheorem(\TeilEins).
Modulo exact forms on~$B$,
$$\multline
	\Cal T\(T^HM,g\TX,\nabla^F,g^F\)
		-T\(A',g^V,h^V\)
		-\chslo\(\nabla^H,g^H_{L_2},g^H_V\)\\
	=-\int_{M/B}\cho\(\nabla^F,g^F\)
			\,\(\nabla\TX h\)^*\psi\(\nabla\TX,g\TX\)
		+\hat p_*\((-1)^{\ind_h}\,\^0J(T^sX-T^uX)\)\,\rk F\;.
\endmultline$$

As application,
we used analytic torsion forms to detect infinite families
of pairwise homeomorphic but not diffeomorphic fibre bundles,
which were constructed using Hatcher's example of a topologically trivial,
but smoothly non-trivial bundle over~$4k$ with fibre~$S^{2l-1}$.
The version we present here is slightly more general,
since in the second statement,
we can now work with an arbitrary unitarily flat~$F$ in place
of the trivial bundle.

\Theorem\ApplThm{(cf.\ \TeilEins)}.
For each integer~$k>0$ there exists~$l_0>0$ such that the following holds.
Let~$p\colon M\to B$ be a smooth fibre bundle
with compact, connected, oriented base~$B$ of dimension~$4k$
and with compact, connected fibres of dimension~$2l-1$,
where~$l\ge l_0$.
Then there exist smooth fibre bundles
$p_j\colon M\to B$ for all~$j\in Z$ with~$p_0=p$,
which are all homeomorphic to~$p$ as fibre bundles
and have diffeomorphic fibres,
but which are pairwise not diffeomorphic as fibre bundles.
\parr
If~$M$ moreover carries a unitarily flat vector bundle~$F$
such that the fibre-wise cohomology bundle~$H^*(M/B;F)\to B$ admits
a parallel metric with respect to the Gau\ss-Manin connection,
then the~$p_j$ are pairwise not diffeomorphic as maps.


In the present paper,
we restrict our attention to the case
that both bundles~$F\to M$ and~$H\to B$ carry parallel metrics.
In this case,
we can use the higher analytic
torsion~$\Cal T\(T^HM,g^{TX},\nabla^F,g^F\)$
to define a cohomology class~$\Cal T(M/B;F)\in H^*(B;\R)$,
see~\TeilEins, \HigherChernTorsionDef.
We compare this class
to a generalisation~$\tau(M/B;F)\in H^*(B;\R)$
of Igusa's higher Franz Reidemeister torsion
in a normalisation adapted to~\BGzwei.

\Theorem\MainTheoremZwei.
Let~$M\to B$ be a family of compact manifolds,
and let~$(F,\nabla^F)\to M$ be
a flat complex vector bundle with a parallel Hermitian metric,
such that~$(H,\nabla^H)$ also admits a parallel metric.
Assume that there exists a function~$h\colon M\to\R$
that is fibre-wise Morse,
then
	$$\Cal T(M/B;F)
	=\tau(M/B;F)
		+\int_{M/B}e(TX)\;\^0J(TX)\,\rk F
	\quad\in H^*(B;\R)\;.$$

We also prove that~$\tau(M/B;F)$ and~$\Cal T(M/B;F)$ induce the same
universal class~$\tau(\Cal M(\C),U)$
on the unitary Whitehead space~$\Wh^u(\Cal M(\C),U)$,
which contains a copy of Igusa's acyclic Whitehead space~$\Wh^h(\Cal M(\C),U)$.

Note that the fibre-wise Morse function does not appear in the conclusion
of \MainTheoremZwei.
We conjecture
that the theorem holds without the assumption
that such a function exists.
By~\Iframed,
after taking the fibre-wise product with~$\R P^{2N}$
for~$N$ sufficiently large,
we get the same higher torsion
and there exists a function~$h\colon M\to\R$
whose fibre-wise singularities are either of Morse type
or birth-death singularities.
In order to treat the general case,
it thus remains to incorporate birth-death singularities into
Theorems~\NummerVon\TeilEinsTheorem\ und~\NummerVon\MainTheoremZwei.

%\Theorem\ApplThmZwei.
%For each integer~$k>0$ there exists~$l_0>0$ such that the following holds.
%Let~$p\colon M\to B$ be a smooth fibre bundle
%with compact, connected, oriented base~$B$ of dimension~$4k$
%and with compact, connected fibres of dimension~$2l-1$,
%where~$l\ge l_0$.
%Let~$F\to M$ be a unitarily flat vector bundle
%such that the fibre-wise cohomology bundle~$H^*(M/B;F)$ admits
%a parallel metric with respect to the Gau\ss-Manin connection.
%Then there exist smooth fibre bundles
%$p_j\colon M\to B$ for all~$j\in Z$ with~$p_0=p$,
%which are all homeomorphic to~$p$ as fibre bundles
%and have diffeomorphic fibres,
%but which are pairwise not diffeomorphic as maps.

\bigskip

The present paper contains the proof of \MainTheoremZwei\
and the new version of \ApplThm,
together with a generalisation of Igusa's approach
to the situation that the two flat bundles~$F\to M$ and~$H\to B$
admit a parallel metric.
It is organised as follows.

We show in~\WhKapitel\
that the construction of~$(V,A',h^V)$ in \ComplexKapitel\ of~\TeilEins\
gives rise to a map~$\xi$ from the base space~$B$ 
to Igusa's Whitehead space~$\Wh\(\Cal M(\C),GL(\C)\)$ up to homotopy,
which equals Igusa's map~$\xi_{p,h,F}\colon B\to\Wh\(\Cal M(\C),GL(\C)\)$. 
Here, $GL(\C)=\lim_{\to} GL_n(\C)=\Cal M(\C)^\times$
denotes the stabilised general linear group.
Conversely, each such map~$\xi_{p,h,F}$ up to homotopy
determines a $\Z$-graded flat vector bundle~$V\to B$
with a flat superconnection~$A'=\nabla^V+a'$ and an endomorphism~$h^V$.
Thus, $\Wh\(\Cal M(\C),GL(\C)\)$ is a universal space
for flat vector bundles with the extra structure described above.
%If the image of~$\xi$
%lies in the subspace~$\Wh^h\(\Cal M(\C),U\)\subset\Wh\(\Cal M(\C),GL(\C)\)$,
%where the~``$h$'' stands for acyclicity and~$U=\lim_{\to} U(n)$
%is the stabilised unitary group,
%then~$V$ admits a parallel metric~$g^V$ that is adapted to~$h^V$ and~$A'$,
%and the fibre-wise cohomology~$H=H^*(V,a'_0)\to B$ vanishes.

We give a different describtion of the finite dimensional
torsion~$T(A',g^V,h^V)$ in \ChernKapitel,
where we show that~$T(A',g^V,h^V)=T(\nabla^V,A',g^V)$
depends only on the existence of local filtrations,
not on~$h^V$.
If~$g^V$ is parallel and the fibre-wise cohomology~$H\to B$ vanishes,
then~$T(\nabla^V,A',g^V)$ is the pull-back~$\xi_{p,h,F}^*T\(\Cal M(\C),U\)$
of a universal higher torsion class~$T\(\Cal M(\C),U\)$
on the acyclic Whitehead space~$\Wh^h\(\Cal M(\C),U\)$.
We also decompose the higher torsion~$T(\nabla^V,A',g^V)$
of a globally filtered family of complexes into the higher torsions
of the steps of the associated spectral sequence,
mimicking Ma's result in~\Ma.

We show in \IgusaKapitel\
that the Igusa's universal torsion class~$\tau\(\Cal M(\C),U\)$
on the Whitehead space~$\Wh^h\(\Cal M(\C),U\)$
coincides up to normalisation with our universal class~$T\(\Cal M(\C),U\)$.
By Igusa's two-index theorem,
it is enough to compare the two classes on the stabilised acyclic
two-index Whitehead space~$\Wh^{h,\{0,1\},s}\(\Cal M(\C),U\)$,
which is homotopy equivalent to~$\Wh^h\(\Cal M(\C),U\)$.
The construction of~$\tau\(\Cal M(\C),U\)$ relies heavily on cyclic homology,
whereas~$T\(A',g^V,h^V\)$ is constructed using a double transgression
of the Chern character.
The comparison of both classes proceeds
by showing that the components of Igusa's class~$\tau\(\Cal M(\C),U\)$
have the same transgression properties as the corresponding terms
in~$T\(\Cal M(\C),U\)$,
and can thus be identified in suitable abstract acyclic cochain complexes.
In the fibre-wise acyclic case,
\MainTheoremZwei\ now follows from Igusa's framing principle
and \TeilEinsTheorem.

We discuss the case
that the two flat bundles~$F\to M$ and~$H\to B$
admit a parallel metrics.
In \UniKapitel,
we construct another Whitehead space~$\Wh^u\(\Cal M(\C),U\)$
which is the universal space of flat bundles~$V\to B$ with the additional
structures~$(A',g^V)$ described  above,
together with a parallel metric~$g^H$ on the fibre-wise cohomology~$H\to B$.
The space~$\Wh^u\(\Cal M(\C),U\)$ is homotopy equivalent to a covering
of Igusa's original~$\Wh\(\Cal M(\C),U\)$.
The universal torsion class~$T\(\Cal M(\C),U\)$ can be extended naturally
to~$\Wh^u\(\Cal M(\C),U\)$.
We also give an acyclic cone construction,
by which the the torsion form~$T\(\Cal M(\C),U\)$ can be pulled back from
a fibre-wise acyclic situation.

Moreover,
the class~$T\(M/B;F,h\)$ of \MorseTorsionDef\ in~\TeilEins\
pulls back from a universal class on~$\Wh^u\(\Cal M(\C),U\)$.
%which is itself a pull-back of the
%class~$\tau\(\Cal M(\C),U\)=T\(\Cal M(\C),U\)$
%on~$\Wh^h\(\Cal M(\C),U\)$.
Combining this with a natural lift
of Igusa's map~$\xi$ to the unitary Whitehead space~$\Wh^u\(\Cal M(\C),U\)$,
we obtain a new class~$\tau(M/B;F)\in H^*(B;\R)$
for all families~$M\to B$ of smooth compact manifolds
with boundary~$\del M=M_0\cup M_1$
which carry unitarily flat vector bundles~$F\to M$
whose relative homology~$H^*(M/B,M_0/B;F)$ is again unitarily flat.

%We add some comments on the structure group~$G$ of~$V$
%and the coefficient ring~$R$ of a simplicial version of~$A'$,
%and we discuss how Lott's secondary $K$-theory developped in~\LottSecOnly\
%fits into our picture.

Finally in \FramingKapitel,
we show that Igusa's framing principle of~\IBuch\ extends
to the case that~$F\to M$ and~$H\to B$ carry parallel metrics.
We then use Igusa's framed function theorem of~\Iframed\
and the framing principle to finally establish \MainTheoremZwei.
We prove a cut-and-paste formula for~$\tau(M/B;F)$
and apply it to extend the examples considered in \BeispielKapitel\
of~\TeilEins\ and prove the generalised second statement
of \ApplThm.
Note that a more precise quantitative statement is given
in \TeilZweiHatcherTheorem.
The proof of \TeilZweiHatcherTheorem\ uses \MainTheoremZwei\
to switch from~$\tau(M/B;F)$ to~$\Cal T(M/B;F)$ as needed.

We will generously cite~\TeilEins.
Therefore,
the numbering of the sections in this paper start with~\NummerVon\WhKapitel.
Sections~\NummerVon\ComplexKapitel\ to \NummerVon\BeispielKapitel\
always refer to~\TeilEins,
as well as all theorems, propositions, equations \dots\
whose first number is~\NummerVon\ComplexKapitel--\NummerVon\BeispielKapitel.

We are grateful to J.-M. Bismut, U. Bunke and K. Igusa for
fruitful discussions and their interest in this project.
We also thank the Mathematical Sciences and Research Institute
at Berkeley
and Igusa's family for their hospitality.

\enddocument





==> morse2.tex <==
\input papermacs

% Flags fuer das Macropaket
\finaltrue
\onefiletrue
\draftfalse

% Neutralisiere alle Flag-Befehle
\let\drafttrue\relax
\let\draftfalse\relax
\let\onefiletrue\relax
\let\onefilefalse\relax
\let\finaltrue\relax
\let\finalfalse\relax

% Lies Projektspezifische Definitionen und Referenzen
\input morse2.def

% Neutralisiere Input- und Ende-Befehle
\let\lies\input
\redefine\input #1 {\relax}
\let\Ende\enddocument
\let\enddocument\endinput

% Lies die einzelnen Textteile
%\lies intro.tex
%\lies complex.tex
%\lies torsion.tex
%\lies main.tex
%\lies witten.tex
%\lies example.tex
\lies intro2.tex
\lies wh.tex
\lies chtor.tex
\lies igusa.tex
\lies unitary.tex
\lies framing.tex
%\lies cubic.tex
\lies refs.tex


\Ende


==> paperdef.tex <==
%auto-ignore
% Caligraphic Letters
\define\calC{{\Cal C}}
\define\calE{{\Cal E}}
\define\calN{{\Cal N}}

% Blackboard Bold Letters
\define\C{{\Bbb C}}
\define\N{{\Bbb N}}
\define\Q{{\Bbb Q}}
\define\R{{\Bbb R}}
\define\Z{{\Bbb Z}}

% Other special letters
\let\eps\varepsilon
\let\phy\varphi
\let\del\partial
\let\thet\vartheta

% Delimiter
\define\fordisplay#1#2{\mathchoice{#1}{#2}{#2}{#2}}
\define\({\fordisplay{\bigl(}(}
\define\){\fordisplay{\bigr)})}
\let\<=\langle
\let\>=\rangle
\define\absl{\left|}
\define\absr{\right|}
\define\abs#1{\absl#1\absr}
\define\norm#1{\left\|#1\right\|}

% Operatoren
\redefine\Re{\operatorname{Re}}
\redefine\Im{\operatorname{Im}}
\define\trace{\operatorname{tr}}
\define\strace{\operatorname{str}}
\define\sign{\operatorname{sign}}

% Sonstiges
\define\dd#1{{\del\over\del#1}}
\define\ddzwo#1{{\del^2\over\del#1^2}}
\let\tensor=\otimes
\define\inn{\mathaccent"7017 }

% halbe Zahlen im Exponenten
\define\hochhalb#1{\fordisplay{^{\textstyle{#1\over2}}}{^{#1\over2}}}
\define\hochmhalb#1{\fordisplay{^{-\textstyle{#1\over2}}}{^{-{#1\over2}}}}

% Integralkerne von Operatoren
\define\bigk<#1|#2|#3>{\bigl\<#1\bigm|#2\bigm|#3\bigr\>}
\define\Bigk<#1|#2|#3>{\Bigl\<#1\Bigm|#2\Bigm|#3\Bigr\>}
\define\biggk<#1|#2|#3>{\biggl\<#1\biggm|#2\biggm|#3\biggr\>}
\define\Biggk<#1|#2|#3>{\Biggl\<#1\Biggm|#2\Biggm|#3\Biggr\>}

% kleine Zwischentexte
\define\Ltext#1{\text{#1}\hskip2em minus1em\relax}
\define\Rtext#1{\hskip2em minus1em\relax\text{#1}}
\define\Mtext#1{\hskip2em minus1em\relax\text{#1}\hskip2em minus1em\relax}
\define\Land{\Ltext{and}}
\define\Mand{\Mtext{and}}
\define\Rand{\Rtext{and}}

% laengere Pfeile im Display
\redefine\to{\fordisplay{\;\longrightarrow\;}\rightarrow}
\define\into{\fordisplay{\;\lhook\joinrel\longrightarrow\;}\hookrightarrow}
\redefine\mapsto{\fordisplay{\;\mapstochar\longrightarrow\;}%
  {\;\mapstochar\rightarrow\;}}
\redefine\colon{\fordisplay{\mathchar"603A\;}{\mathchar"603A}}

% Kleine Matrizen
\define\spmatrix{\left(\smallmatrix}
\define\endspmatrix{\endsmallmatrix\right)}





==> refs.tex <==
%auto-ignore
\input morse2.def

\document

\Refs
\widestnumber\key{DWW}

\Quelle\BB[BB]\Journal
A.~Berthomieu, J.-M.~Bismut:
Quillen metrics and higher analytic torsion forms,
J.\ reine angew.\ Math.~457 (1994), 85--184

\Quelle\BGzwei[BG]\Journal
J.-M. Bismut, S. Goette:
Families torsion and Morse functions,
Ast\'erisque~275 (2001),

\Quelle\BL[BL]\Journal
J.-M.\ Bismut, J.\ Lott:
{Flat vector bundles, direct images and higher real analytic torsion},
J.\ Am.\ Math.\ Soc.~8 (1995), 291--363

\Quelle\BuZwei[Bu]\Journal
\bysame: %U.~Bunke:
Equivariant higher analytic torsion and equivariant Euler characteristic,
Amer.\ J. Math.~122 (2000), 377--401

\Quelle\Dai[D]\Journal
X.~Dai:
Adiabatic limits, non-multiplicativity of signature
and Leray spectral sequence,
J. Am. Math. Soc.~4 (1991), 265--321

\Quelle\TeilEins[G]\Preprint
S.~Goette:
Morse theory and higher torsion invariants I,
\finalinfo preprint (2001), \tt math.DG/0111222

\Quelle\Iframed[I1]\Journal
K.~Igusa:
The space of framed functions,
Trans. Am. Math. Soc.~301 (1987), 431--477

\Quelle\IBuch[I2]\Buch
\bysame:
Higher Franz-Reidemeister Torsion,
International Press
\bookinfo AMS/IP Studies in Advanced Mathematics \vol31 (2002)

\Quelle\ITwisted[I3]\Preprint
\bysame:
Twisted Cochains and Higher Torsion,
\finalinfo preprint (2002), \tt math.AT/0212383

\Quelle\IKomplex[I4]\Preprint
\bysame:
Higher complex torsion and the framing principle,
\finalinfo preprint (2003), \tt math.KT/0303047

\Quelle\Loday[Lo]\Buch
J.-L. Loday:
Cyclic homology,
Springer, Berlin (1992)

\Quelle\Ma[Ma]\Journal
X.\ Ma:
Functoriality of real analytic torsion forms,
Israel J. Math.~131 (2002), 1--50

\Quelle\MM[MM]\Journal
R.~Mazzeo, R.~Melrose:
The adiabatic limit, Hodge cohomology and Leray's spectral sequence
of a fibration,
J. Diff. Geom.~31 (1990), 185--213

\endRefs

\enddocument






==> unitary.tex <==
%auto-ignore
\input morse2.def

\document


\Kapitel\UniKapitel=9 The unitary Whitehead space and its torsion class

We generalise the constructions of \WhKapitel\
to allow family Thom-Smale complexes such that the fibrewise cohomology
carries a unitarily flat metric.
In  \WhUniSubsection,
we contruct a unitary Whitehead space~$\Wh^u(R,G)$
that naturally covers the full Whitehead space~$\Wh(R,G)$.
The cohomology bundle~$\Cal H\to\Wh^u(R,G)$
carries a natural metric~$g^{\Cal H}$.
In \UniTorSubsection,
we extend the universal torsion class defined in \TorsionKapitel\
and studied in \IgusaKapitel\
to a class~$\tau(R,G)\in H^\even\Wh^u(R,G)$.

Suppose that~$p\colon M\to B$ is a family equipped with a fibre-wise Morse
function~$h$ and a flat vector bundle~$F\to M$. % that is fibre-wise acyclic.
Then the lifts~$\xi^u$
of the associated map~$\xi=\xi_{p,h,F}\colon B\to\Wh(R,G)$ to~$\Wh^u(R,G)$
are in one-to-one correspondence
with the parallel metrics on the fibre-wise cohomology~$H=H^*(M/B;F)\to B$.
The class~$(\xi^u)^*\tau(R,G)$ does not depend
on the choice of the lift in degree~$\ge2$,
and we recover the unitary Morse torsion class~$T(M/B;F,h)$
of \MorseTorsionDef\ as~$(\xi^u)^*\tau(R,G)\dg{\ge2}$.
Because all our constructions are compatible with stabilisation,
we can generalise Igusa's constructions in~\IBuch\ to arbitrary families
of manifolds equipped with unitarily flat vector bundles
such that the fibrewise cohomology carries a parallel metric.

Finally,
we give a natural map~$\pi\colon\Wh^u(R,G)\to\Wh^h(R,G)$,
such that~$\tau(R,G)$ is preserved by~$\pi^*$.
This shows in particular that we recover Igusa's torsion~$\tau(M/B;F)$,
which is defined similarly under the assumption that~$H\to B$ is trivial
or has nilpotent structure group.


\Abschnitt\WhUniSubsection The unitary Whitehead space

We construct the unitary Whitehead space~$\Wh^u(R;G)$
as a covering of the Whitehead space~$\Wh(R,G)$.
Note that the unitary Whitehead space should be viewed as a generalisation
of Igusa's acyclic Whitehead space~$\Wh^h(R;G)$.

We have seen that the higher torsion forms of \TorsionKapitel\ can be used to
construct cohomology classes if both flat bundles~$F|_C\to C$ and~$H\to B$
carry parallel metrics.
Therefore,
we need a variant of the Whitehead space that contains information
about metrics on the tautological bundle~$\Cal V\to\Wh(R;G)$
and the universal cohomology bundle~$\Cal H\to\Wh(R;G)$.

The bundle~$F|_C$ admits a parallel metric
iff we can choose its discrete structure group
to be subgroup of the unitary group,
so it is sufficient to choose a group~$G\subset R^\times$
and a complex representation~$\rho\colon G\to GL_n(\C)$
such that~$\rho(G)\subset U(r)$.
On the other hand,
if we regard~$\rho(G)\subset U(r)$,
then the complexified bundle~$\Cal V\to\Wh(R,G)$ carries
a natural Hermitian metric induced by the standard metric on~$\C^r$.

All fibre-wise metrics on~$\Cal H$ form a fibre bundle over~$\Wh(R,G)$
with a natural flat bundle connection for any~$R$ and~$G$.
We can take the \'etale space of the sheaf
of horizontal sections of this bundle,
which become parallel metrics on~$\Cal H$,
as a classifying space for Morse vector bundles
with a given parallel metric on the fibre-wise cohomology.
In fact,
we will refine this concept just a little
by fixing a parallel Hermitian basis of~$\Cal H$ over each simplex
of our unitary Whitehead space~$\Wh^u(R,G)$.

To keep things simple,
we will take the point of view
that unitary higher torsion is defined on~$\Wh^u\(\Cal M_r(\C),U(r)\)$.
For arbitrary~$R$ and~$G$,
we obtain the unitary Whitehead space~$\Wh^u(R,G)$
and its universal torsion class~$\tau(R,G)\in H^\even(R,G)$
from a pullback construction
$$\CD
	\Wh^u(R,G)@>>>\Wh^u\(\Cal M_r(\C),U(r)\)\\
	@VVV@VVV\\
	\Wh(R,G)@>>>\Wh\(\Cal M_r(\C),U(r)\)&\;,
\endCD$$
where the lower right arrow is induced by
a representation~$\rho\colon R\to\Cal M_r(\C)$ with~$\rho(G)\subset U(r)$,
the space~$\Wh^u(R,G)$ is constructed as a pullback bundle,
and~$\tau(R,G)$ is the pullback of~$\tau=\tau\(\Cal M_r(\C),U(r)\)$
by the upper right arrow.

For convenience,
we give a simplicial model for~$\Wh^u\(\Cal M_r(\C),U(r)\)$.
Recall that the $\Z$-graded flat vector bundles~$\Cal V\to\Wh\(\Cal M_r(\C),U(r)\)$
and~$\Cal H\to\Wh\(\Cal M_r(\C),U(r)\)$
were described in \WhFlatBdlRem.

\Definition\WhUniDef
The {\em unitary simplicial pre-Whitehead
category\/}~$\cWh^{\prime\simp,u}\(\Cal M_r(\C),U(r)\)$ is defined as follows.
\roster
\item
Objects of~$\cWh^{\simp,u}_k\(\Cal M_r(\C),U(r)\)$ are
given by triples~$(P,a,e)$,
where~$(P,a)$ is an object of~$\cWh^\simp_k\(\Cal M_r(\C),U(r)\)$
and~$e=(e^p(i))_{p,i}$
is a family of complex bases~$e^p_1(i)$, \dots, $e^p_{\rk H^p}(i)$
on the spaces~$H^p\bigl((\C^r)^P,a(i)\bigr)$ that are compatible
with the natural isomorphisms
	$$\(\id+a(i,j)\)_*\colon H^*\((\C^r)^P,a(j)\)\to H^*\((\C^r)^P,a(i)\)$$
for~$0\le i\le j\le k$.
\item
Morphisms from~$(P,a,e)$ to~$(Q,b,e')\in\cWh^{\simp,u}$
are given by pairs~$(f,g)$
such that~$(f,g)$ is a $\cWh^\simp\(\Cal M_r(\C),U(r)\)$-morphism from~$(P,a)$ to~$(Q,b)$,
and the induced isomorphisms
	$$(f,g)_*\colon H^*\((\C^r)^P,a(i)\)\to H^*\((\C^r)^Q,b(i)\)$$
are given in the bases~$e$ and~$e'$
by unitary matrices for one (and thus for all)~$0\le i\le k$.
\item
Generalised face operators are given by re-indexing as
in \WhSimpDef.
\endroster
The {\em simplicial unitary pre-Whitehead
space\/}~$\Wh^{\prime\simp,u}\(\Cal M_r(\C),U(r)\)$
%=\bigl|N\cWh^{\prime\simp,u}\(\Cal M_r(\C),U(r)\)\bigr|
is the geometric realisation of the simplicial unitary pre-Whitehead category.
\enddefinition

We stabilise the unitary Whitehead space as in \WhStabDef.
Note that if~$(P\dg l,a\dg l)$ is the elementary object of vertical degree~$l$,
then we naturally identify
	$$H^*\((\C^r)^P,a(j)\)
	\cong H^*\Bigl((\C^r)^{P\cup P\dg l},\(a\oplus a\dg l\)(j)\Bigr)\;.$$
In particular,
we can compare bases on both sides.

\Definition\UniStabDef
The {\em (stabilised) simplicial unitary Whitehead
category\/}~$\cWh^{\simp,u}\(\Cal M_r(\C),U(r)\)$ has the same objects
and face operators as~$\cWh^{\prime\simp,u}\(\Cal M_r(\C),U(r)\)$.
Its morphisms are iterated formal compositions
of~$\cWh^{\prime\simp,u}\(\Cal M_r(\C),U(r)\)$-morphisms and elementary expansions
	$$(P,a,e)\to(P\cup P\dg j,a\oplus a\dg j,e)\;.$$
The {\em simplicial unitary Whitehead space\/}~$\Wh^{\simp,u}\(\Cal M_r(\C),U(r)\)$
%=\bigl|N\cWh^{\simp,s}\(\Cal M_r(\C),U(r)\)\bigr|
is the geometric realisation of the simplicial unitary Whitehead category.
\enddefinition


\Remark\WhUniRem
We collect some properties of the definition above.
\roster
\item
By its construction in \WhFlatBdlRem~(1),
the bundle~$\Cal V\to\Wh'\(\Cal M_r(\C),U(r)\)$
inherits a parallel metric~$g^{\Cal V}$
from the standard metric on~$\C^r$.
A similar construction yields a unitarily
flat bundle~$\(\Cal V,g^{\Cal V}\)\to\Wh^{\prime\simp,u}\(\Cal M_r(\C),U(r)\)$.
We also let~$\Cal H$ denote fibre-wise cohomology as in \WhFlatBdlRem~(2),
which is a flat vector bundle that is compatible with stabilisation,
so we get~$\Cal H\to\Wh^{\simp,u}\(\Cal M_r(\C),U(r)\)$.
\item
The bundle~$\Cal H\to\Wh^{\simp,u}\(\Cal M_r(\C),U(r)\)$ carries a unique
parallel metric~$g^{\Cal H}$ for which the bases~$e$ are unitary.
%\item
%There is a forgetful
%functor from~$\cWh^{\simp,u}\(\Cal M_r(\C),U(r)\)$
%to a category where the bases~$e$ in \WhUniDef~(1)
%are replaced by a collection of Hermitian metric~$g^H$
%on~$H^p\bigl((\C^r)^P,a(i)\bigr)$.
%The geometric realisation of this category is in turn
%a bundle over~$\Wh\(\Cal M_r(\C),U(r)\)$
%with fibre the space of unitary metrics on the fibre of~$\Cal H$,
%equipped with the discrete topology.
%In other words,
%the space~$\Wh^{\simp,u}\(\Cal M_r(\C),U(r)\)$ is a refinement of the \'etale space
%of the sheaf of parallel Hermitian metrics
%on the bundle~$\Cal H\to\Wh^{\simp}\(\Cal M_r(\C),U(r)\)$ of \WhFlatBdlRem~(2).
%The metric~$g^{\Cal H}$ on the bundle~$\Cal H\to\Wh^{\simp,u}\(\Cal M_r(\C),U(r)\)$
%that is defined by the bases~$e$
%corresponds to the tautological metric.
%It turns out that the extra information encoded in the bases~$e$
%is needed mostly for bookkeeping purposes.
%\item
%If~$\xi^\simp_{p,h,F}\colon B\to\Wh^{\prime\simp}\(\Cal M_r(\C),U(r)\)$
%is constructed as in \WhFunctorProp\ and \WhSimpUniversalRem,
%then the homotopy classes
%of lifts~$\xi^{\simp,u}_{p,h,F}\colon B\to\Wh^{\prime\simp,u}\(\Cal M_r(\C),U(r)\)$
%of~$\xi^\simp_{p,h,F}$ correspond precisely to the parallel metrics
%on the bundle~$H\to B$.
%This is because we are free to choose a parallel Hermitian basis of~$H\to B$
%over each simplex of~$B$.
\item
Recall that~$\cWh^{\simp,h}\(\Cal M_r(\C),U(r)\)$
is the full subcategory of~$\cWh^{\simp}\(\Cal M_r(\C),U(r)\)$
consisting of those objects~$(P,a)\in\cWh^{\simp}\(\Cal M_r(\C),U(r)\)$
for which~$a(i)$ is acyclic for one (and thus for all)~$i$.
Then~$\cWh^{\simp,h}\(\Cal M_r(\C),U(r)\)$ is a full subcategory
of~$\cWh^{\simp,u}\(\Cal M_r(\C),U(r)\)$,
and the forgetful functor to~$\cWh^{\simp,h}\(\Cal M_r(\C),U(r)\)$
is just the identity.
This way,
we may view~$\cWh^{\simp,u}\(\Cal M_r(\C),U(r)\)$ as a generalisation
of the category~$\cWh^{\simp,h}\(\Cal M_r(\C),U(r)\)$ considered in~\IBuch.
\item
There are similar definitions for~$\cWh^{\diff,u}\(\Cal M_r(\C),U(r)\)$,
$\cWh^{\mix,u}\(\Cal M_r(\C),U(r)\)$ and their unstabilised variants
if~$R$ is an $\R$-algebra.
Again,
%$\Wh^{\diff,u}\(\Cal M_r(\C),U(r)\)$ is just the \'etale space of the sheaf
%of parallel Hermitian metrics on~$\Cal H\to\Wh^{\diff}\(\Cal M_r(\C),U(r)\)$,
%and~
$\Wh^{\diff,u}\(\Cal M_r(\C),U(r)\)$ is the classifying space
for Morse vector bundles~$(V,A',h^V)\to B$ whose fibre-wise cohomology~$H\to B$
is equipped with a parallel metric~$g^H$.
It is now easy to check that all results of \MixedWhSubsection\
carry over to unitary Whitehead categories,
so we have homotopy equivalences
$$\CD
	&\Wh^{\prime\simp,u}\(\Cal M_r(\C),U(r)\)
	@<\Phi_1^u<\botsim<\Wh^{\prime\mix,u}\(\Cal M_r(\C),U(r)\)
	@>\Phi_2^u>\botsim>\Wh^{\prime\diff,u}\(\Cal M_r(\C),U(r)\)\\
		\Land
	&\Wh^{\simp,u}\(\Cal M_r(\C),U(r)\)
	@<\Phi_1^u<\botsim<\Wh^{\mix,u}\(\Cal M_r(\C),U(r)\)
	@>\Phi_2^u>\botsim>\Wh^{\diff,u}\(\Cal M_r(\C),U(r)\)\;.
\endCD$$
In particular,
we may talk about ``the'' unitary pre-Whitehead
space~$\Wh^{\prime u}\(\Cal M_r(\C),U(r)\)$,
which is well-defined up to homotopy equivalence
and carries unitarily flat vector bundles~$(\Cal V,\nabla^{\Cal V},g^{\Cal V})$
and~$(\Cal H,\nabla^{\Cal H},g^{\Cal H})$.
\endroster
\endremark

Let us examine the homotopy type of the unitary Whitehead space.
We denote by~$\Cal G(\Cal H)$
the space of Hermitian metrics on~$\Cal H\to\Wh\(\Cal M_r(\C),U(r)\)$.
We topologize~$\Cal G(\Cal H)$
as the \'etale space of the sheaf of locally parallel  metrics on~$\Cal H$.
In other words,
the map~$\Cal G(\Cal H)\to\Wh\(\Cal M_r(\C),U(r)\)$
is a covering,
and local sections are given precisely by parallel metrics.
A simplicial model for~$\Cal G(\Cal H)$ can be constructed
as in \WhUniDef,
but using parallel metrics~$g^H$ on~$H^*\bigl((\C^r)^P,a'_0\bigr)$
over each simplex of~$\Wh\(\Cal M_r(\C),U(r)\)$
instead of parallel bases~$e$ of this bundle.

\Proposition\UniWhProp.
There is a natural map~$\Wh^u\(\Cal M_r(\C),U(r)\)\to\Cal G(\Cal H)$
given by assigning
to a local parallel basis~$e$ of~$\Cal H$ the Hermitian metric
for which~$e$ is unitary.
This map is a fibre bundle with contractible fibres.
\parr
In particular,
if~$\xi\colon B\to\Wh\(\Cal M_r(\C),U(r)\)$ is a map
and~$\(V,\nabla^V,A',g^V\)=\xi^*\(\Cal V,\nabla^{\Cal V},\Cal A',g^{\Cal V}\)$,
then homotopy classes of lifts~$\xi^u\colon B\to\Wh^u\(\Cal M_r(\C),U(r)\)$
are in bijection with globally parallel metrics~$g^H$
on~$H=H^*\(V,a'_0\)=\xi^*\Cal H\to B$.

In other words,
we could have defined~$\Wh^u\(\Cal M_r(\C),U(r)\)$
simply as the covering space~$\Cal G(\Cal H)\to\Wh\(\Cal M_r(\C),U(r)\)$.
Nevertheless,
the extra information about a local framing on~$\Cal H$ will be helpful
later on.

\Proof
Over each simplex~$\sigma\in\Wh^{\simp,u}$,
the fibre of the map~$\Wh^u\(\Cal M_r(\C),U(r)\)\to\Cal G(\Cal H)$
is the geometric realisation of the category of all unitary basis
and unitary base changes
with respect to the tautological metric~$g^{\Cal H}$
on the pullback of~$\Cal H$ to~$\Cal G(\Cal H)$.
But this fibre is just the classifying bundle~$E\(U(\Cal H|_\sigma)\)$
of the unitary group acting on the fibre of~$\Cal H|_\sigma$,
which is contractible.

The second claim follows
because globally parallel metrics~$g^H$ on~$H\to B$
correspond precisely to lifts of~$\xi$
to the space~$\Cal G(\Cal H)$.
\qed\enddemo


\Abschnitt\UniTorSubsection The universal torsion class
on the unitary Whitehead space

%For the rest of this chapter,
%we have to assume that~$R$ is an $\R$-subalgebra of~$M_r(\C)$,
%and that~$G\subset R^\times\cap U(r)$ is a subgroup of a unitary group.
We generalise our definition
of~$T\(\Cal M_r(\C),U(r)\)\in H^\even\(\Wh^h\(\Cal M_r(\C),U(r)\)\)$
in \TChRGDef\ to the unitary setting.
Because we have seen in \IgleichMVBThm\
that~$T\(\Cal M_r(\C),U(r)\)=\tau\(\Cal M_r(\C),U(r)\)$
on~$\Wh^h\(\Cal M_r(\C),U(r)\)$,
we will name our
new class~$\tau\(\Cal M_r(\C),U(r)\)\in H^\even\(\Wh^u\(\Cal M_r(\C),U(r)\)\)$,
or just~$\tau$.
The letter~$T$ will be reserved for torsion forms associated
directly to superconnections as in \MVBSubsection.
Note that in general,
the forms~$T\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)$ are not closed,
so they do not define cohomology classes.
However,
since~$g^{\Cal V}$ and~$g^{\Cal H}$ are unitarily flat,
the form~$T\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)
+\chslo\(\nabla^{\Cal H},g^{\Cal H},g^{\Cal H}_{\Cal V}\)$ is closed,
and  defines a class~$\tau$ on~$\Wh^u\(\Cal M_r(\C),U(r)\)$
by Stokes theorem.
Finally,
we show that~$\tau$ is compatible with respect to stabilisation in~$r$
and thus extends to a form on~$\Wh^u\(\Cal M(\C),U\)$
with~$\Cal M(\C)=\lim_{\to}\Cal M_r(\C)$ and~$U=\lim_{\to}U(r)$.

\Definition\UniTorDef
Define~$\tau=\tau\(\Cal M_r(\C),U(r)\)
\in H^{\even}\bigl(\Wh^{\prime u}\(\Cal M_r(\C),U(r)\),\R\bigr)$
to be the class represented by the cocycle
which assigns to every simplex~$\Delta$ in~$\cWh^{\prime\diff,u}\(\Cal M_r(\C),U(r)\)$
the integral
	$$\int_\Delta\Bigl(T\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)
		+\chslo\(\nabla^{\Cal H},g^{\Cal H}
			,g^{\Cal H}_{\Cal V}\)\Bigr)\;.$$
%We will abbreviate~$\tau=\tau\(\Cal M_r(\C),U(r)\)$
%for~$R=\Cal M_r(\C)=\lim_{\to}\Cal M_r(\C)$ and~$G=U=\lim_{\to}U(r)$.
\enddefinition

Then~$\tau\dg0$ measures the difference of the Franz-Reidemeister metric
on~$\det H$ and the metric~$g^{\det H}$ induced by~$g^{\Cal H}$.
Let~$(V,A',h^V)$ be a family Thom-Smale complex over~$B$
such that~$\nabla^V$ is unitarily flat
and such that~$H\to B$ admits a parallel metric.
If~$S$ is a simplicial structure on~$B$,
there exists a ``classifying functor''
$\Xi\colon S\to\cWh^{\prime\diff,u}\(\Cal M_r(\C),U(r)\)$,
inducing a classifying map~$\xi\colon B\to\Wh^{\prime u}\(\Cal M_r(\C),U(r)\)$ up to homotopy,
such that
	$$\(V,\nabla^V,A',g^V\)
	\cong\xi^*\(\Cal V,\nabla^{\Cal V},\Cal A',g^{\Cal V}\)
		\Mand
	\(H,\nabla^H,g^H\)\cong\xi^*\(\Cal H,\nabla^{\Cal H},g^H\)\;.$$
We have an immediate generalisation of \ChTorsionCor.

\Corollary\UniTorCor.
Let~$S$ be a simplicial complex on~$B$
and let~$\Xi\colon S\to\cWh^{\prime \diff,u}\(\Cal M_r(\C),U(r)\)$ be a simplicial map.
Let~$(V,\nabla^V,A',g^V)
=\abs\Xi^*\(\Cal V,\nabla^{\Cal V},\Cal A',g^{\Cal V}\)$
and~$(H,\nabla^H,g^H)
=\abs\Xi^*\(\Cal H,\nabla^{\Cal H},g^H\)$,
then
	$$T\(\nabla^V,A',g^V\)+\chslo\(\nabla^H,g^H,g^H_V\)
	=\abs\Xi^*\tau
	\quad\in H^{\even}(\abs S,\R)\;.\tag1$$
\parr
In particular,
if~$p\colon M\to B$ is a proper submersion
with a fibrewise Morse-function~$h\colon M\to\R$,
if~$(F,\nabla^F,g^F)\to M$ is a unitarily flat vector bundle,
such that the bundle~$H=H^*(V,a_0)\to B$ admits a parallel metric,
and if~$\xi^u\colon B\to\Wh^{\prime u}\(\Cal M_r(\C),U(r)\)$
is constructed as in \WhUniRem~(3),
then
	$$T(M/B,F,h)=\xi^{u*}\tau\dg{\ge2}\;.\tag2$$

This follows from the same kind of arguments as \ChTorsionCor.
Note here that since the parallel metric on~$H$ can be varied,
we cannot define the ordinary Franz-Reidemeister torsion in degree~$0$.
On the other hand,
$\xi^{u*}\tau\dg{\ge2}$ is independent of the particular lift~$\xi^u$
by \ChernBLCor.
For this reason,
the constant function~$\xi^{u*}\tau\dg0$
is explicitly excluded from~(2).

\Proposition\UniTorStableProp.
The unitary torsion class~$\tau=\tau\(\Cal M_r(\C),U(r)\)
\in H^\even\(\Wh^{\prime u}\(\Cal M_r(\C),U(r)\),\R\)$
is compatible with stabilisation
and descends to~$\Wh^{u}\(\Cal M_r(\C),U(r)\)$.

\Proof
We have to show that~$\tau$ is compatible with the elementary
expansions in~$\cWh^{\diff,u}$.
Therefore,
let~$P\dg l$ and~$a^{\prime\dg l}
=\bigl(\smallmatrix0&1\\&0\endsmallmatrix\bigr)$ as in \DiffElExDef.
We take the trivial metric on~$(\C^r)^{P\dg l}$.
%and set~$h^{V^{P\dg l}}=N^{V^{P\dg l}}$.
Then by \ChBLTorCor,
	$$T\(d,d+a^{\prime[l]},g^{\triv}\)
	=T^{\roman{BL}}\(d+a^{\prime[l]},g^{\triv}\)
	=0\;.$$
It follows that the explicit cocycle for~$\tau$ in \UniTorDef\
takes the same value on~$(P,a,g^H)$
as on~$(P\cup P\dg l,a'\oplus a^{\prime[l]},g^H)$.
The proposition follows from the definition of the stabilised differential
unitary Whitehead space.
\qed\enddemo


We will use the
universal torsion class~$\tau\in H^\even\(\Wh^u\(\Cal M_r(\C),U(r)\)\)$
in \FramingKapitel\
to extend Igusa's higher Franz-Reidemeister torsion to smooth fibre bundles
with unitarily flat fibre-wise cohomology.
%Let~$p\colon M\to B$ be a smooth fibre bundle with~$\dim M>2\,\dim B$,
%and let~$h\colon M\to\R$ be a proper framed function
%with finitely many critical points on each fibre of~$p$.
%Let~$F\to M$ be a bundle of free left $R$-modules with structure group~$G$.
%Then Igusa constructs a map~$\xi_h\colon B\to\Wh\(\Cal M_r(\C),U(r)\)$ in~\IBuch, Chapter~4,
%whose homotopy is independent of fibre-wise compactly supported changes of~$h$.
%By \WhUniRem~(3) the lifts of~$\xi_h$ to~$\Wh^u\(\Cal M_r(\C),U(r)\)$ are in one-to-one
%correspondence with the possible flat metrics on~$H=H^*(M/B;F)\to B$.
%
%\Lemma\UniWellDefLemma.
%If there exists a lift~$\xi_h\colon B\to\Wh^u\(\Cal M_r(\C),U(r)\)$,
%then
%	$$\xi_h^*\tau\dg{\ge2}$$
%is independent of the choice of that lift~$\xi_h$.
%
%\?weiter?
%
%\Proof
%This follows from \MorseTorsionCor.
%\qed\enddemo
%
%\Definition\UniIgusaDef
%Let~$p\colon M\to B$ be a smooth fibre bundle with
%a proper framed function~$h\colon M\to\R$ with finitely many critical
%points on each fibre.
%Let~$F\to M$ be a unitarily flat vector bundle
%such that~$H^*(M/B;F)\to B$ admits a parallel metric.
%Then we define the higher Franz-Reidemeister torsion
%	$$\tau_h(M/B;F)=\xi_h^*\tau\dg{\ge2}\;.$$
%\enddefinition
%
%\Remark\UniIgusaRem
%\roster
%\item
%If~$p\colon M\to B$ is proper,
%then~$\tau_h(M/B;F)$ is independent of~$h$.
%\item
%If we fix parallel metrics~$g^F$ and~$g^H$,
%we can extend~$\tau_h(M/B;F)$ in degree~$0$ by the classical Franz-Reidemeister
%torsion.
%\endroster\endremark

For all~$r$, $r'\ge 0$,
there are well-known natural homomorphisms
	$$\Cal M_r(\C)\to\Cal M_{r+r'}(\C)
		\Mand
	U(r)\to U(r+r')$$
given by extending a matrix in~$\Cal M_r(\C)$ by zero,
and an element~$g\in U(r)$ to~$g\oplus\id_{\C^{r'}}$.
Let
	$$\Cal M(\C)=\lim_{r\to\infty}\Cal M_r(\C)
		\Mand
	U=\lim_{r\to\infty}U(r)$$
denote the direct limits with respect to these maps.

The maps~$\Cal M_r(\C)\to\Cal M_{r+r'}(\C)$
and~$U(r)\to U(r+r')$ induce a functor
	$$\cWh\(\Cal M_r(\C),U(r)\)
	\to\cWh\(\Cal M_{r+r'}(\C),U(r+r')\)\;.
	\Formel\WhDimStabMap$$
This gives rise to a pullback diagramme
$$\CD
	\Cal V\oplus\C^{r'\rk\Cal V/r}@>>>\Cal V\\
	@VVV@VVV\\
	\Wh\(\Cal M_r(\C),U(r)\)@>>>\Wh\(\Cal M_{r+r'}(\C),U(r+r')\)&\;.
\endCD$$
The additional trivial bundle~$\C^{r'\,\rk\Cal V/r}$
carries the trivial connection~$d$,
and since all coefficients~$a'_*$ of~$\Cal A'$ are extended trivially,
the pull-back of~$\Cal A'$ acts as~$d$ on~$\C^{r'\,\rk\Cal V/r}$.
Thus,
we have another pullback diagramme
$$\CD
	\Cal H\oplus\C^{r'\rk\Cal V/r}@>>>\Cal H\\
	@VVV@VVV\\
	\Wh\(\Cal M_r(\C),U(r)\)@>>>\Wh\(\Cal M_{r+r'}(\C),U(r+r')\)&\;.
\endCD\Formel\WhDimStabHFormel$$

We extend the functor~\WhDimStabMap\ to a functor
	$$\cWh^u\(\Cal M_r(\C),U(r)\)
	\to\cWh^u\(\Cal M_{r+r'}(\C),U(r+r')\)
	\Formel\WhUniDimStabMap$$
by specifying the standard basis
on the additional summand~$\C^{r'\rk\Cal V/r}$ in~\WhDimStabHFormel.

\Proposition\WhUniDimStabProp.
The universal unitary higher torsion class~$\tau$
is compatible with stabilisation
	$$\Wh^u\(\Cal M_r(\C),U(r)\)
	\to\Wh^u\(\Cal M_{r+r'}(\C),U(r+r')\)\;.$$

\Proof
We use the differential model of the Whitehead space.
On a single simplex~$\sigma=(P,a',e)\in\cWh^{\diff,u}\(\Cal M_r(\C),U(r)\)$,
the pullback of~$\tau\(\Cal M_{r+r'}(\C),U(r+r')\)$
is given by
$$\multline
	\int_\Delta\Bigl(T\(\nabla^{\Cal V}\oplus d
		,\Cal A'\oplus d,g^{\Cal V}\oplus g^{\triv}\)
		+\chslo\(\nabla^{\Cal H}\oplus d,
			g^{\Cal H}\oplus g^{\triv},
			g^{\Cal H}_{\Cal V}\oplus g^{\triv}\)\Bigr)\\
\split
	&=\int_\Delta\Bigl(T\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)
		+T^{\roman{BL}}\(d,g^{\triv}\)
		+\chslo\(\nabla^{\Cal H},
			g^{\Cal H},
			g^{\Cal H}_{\Cal V}\)\Bigr)\\
	&=\int_\Delta\Bigl(T\(\nabla^{\Cal V},\Cal A',g^{\Cal V}\)
		+\chslo\(\nabla^{\Cal H},
			g^{\Cal H},
			g^{\Cal H}_{\Cal V}\)\Bigr)
	=\tau\(\Cal M_r(\C),U(r)\)(\sigma)\;,
\endsplit\endmultline$$
because the Bismut-Lott torsion vanishes for a trivial superconnection.
\qed\enddemo

\Definition\WhUniDimStabDef
We define the {\em universal unitary Whitehead category\/} by
	$$\cWh^u\(\Cal M(\C),U\)
	=\lim_{r\to\infty}\cWh^u\(\Cal M_r(\C),U(r)\)$$
using the functors~\WhUniDimStabMap,
and let the {\em universal unitary Whitehead space\/}~$\Wh^u\(\Cal M(\C),U\)$
be its geometric realisation.
We still denote the {\em universal unitary higher torsion class\/}
by
	$$\tau\in H^\even\bigl(\Wh^u\(\Cal M(\C),U\)\bigr)\;.$$
\enddefinition


\Abschnitt\ConeSubsection The cone construction
%and Igusa's two-index theorem

In this section,
let~$(V,A',h^V)\to B$ be an arbitrary family Thom-Smale complex
and let~$g^V$ be an arbitrary adapted metric on~$V$ which need
not be parallel.
We construct a fibre-wise acyclic  family Thom-Smale
complex~$\bigl(\widehat V,\widehat A',h^{\hat V}\bigr)$
on the vector bundle~$\widehat V=V\oplus H$.
In the next subsection,
we will compare the torsion classes~$T\(\nabla^V,A',g^V\)$
and~$T\bigl(\nabla^{\hat V},\widehat A',g^{\hat V}\bigr)$.

We fix an adapted metric~$g^V$ on~$V$ in the sense of \MorseMetricDef\
and let~$a''_0$ denote the adjoint of~$a'_0$ with respect to~$g^V$.
By finite-dimensional Hodge theory,
we have a $g^V$-orthogonal splitting
	$$V=\ker\(a'_0+a''_0\)\oplus\im\(a'_0\)\oplus\im\(a_0''\)\;,$$
which is preserved by the combinatorial Laplacian~$[a'_0,a''_0]$.
Let~$\iota\colon H\to\ker\(a'_0+a''_0)\subset V$
denote the identification of~$H$ with the harmonic elements,
which we extend $\Omega^*(B)$-linearly
to a map~$\iota\colon\Omega^*(B;H)\to\Omega^*(B;V)$.

We can find a smooth function~$\eps\colon B\to\R_>$
such that~$\abs\lambda>\eps$ for all non-zero eigenvalues~$\lambda$
of~$[a'_0,a''_0]$.
Then we define a generalised
spectral projection~$\Pi$ on~$\Omega^*(B;V)$ by
	$$\Pi
	={1\over2\pi i}
		\,\int_{\eps S^1}{d\lambda\over\lambda-(A'+a_0'')^2}\;.$$
Similar operators were already considered in~\BGzwei,
Definition~10.13.
The analogue of Theorem~10.9 in~\BGzwei\ implies in particular
that~$\Pi^2=\Pi$,
that~$\Pi$ is of total degree~$0$,
and that~$\Pi$ commutes with~$A'$, $a_0''$ and~$\Omega^*(B)$.
Moreover,
the projection~$\Pi\dg0$ in degree~$0$ with respect to~$N^B$ coincides
with the orthogonal projection onto the harmonic elements of~$V$.

Let~$W\subset\Omega^*(B;V)$ be the image of~$\Pi$,
then~$W$ is an $A'$-invariant $\Omega^*(B)$-submodule of~$\Omega^*(B;V)$
and~$\Pi\circ\iota\colon\Omega^*(B;H)\to W$ is an isomorphism.
Let
	$$A^{\prime H}=(\Pi\circ\iota)^{-1}\circ A'\circ(\Pi\circ\iota)
	\Formel\UniAxHDef$$
be the pullback superconnection on~$H$.

\Lemma\ConeLemma.
The superconnection~$A^{\prime H}$ takes the form
	$$A^{\prime H}=\nabla^H+a^{\prime H}
		\Rtext{with }a^{\prime H,[k]}\in\Omega^{\ge2}(B;\End H)\;.
	\tag1$$
Moreover,
$\Pi\circ\iota$ induces an $\Omega^*(B)$-linear isomorphism
of cochain complexes
	$$\Pi\circ\iota
	\colon\(\Omega^*(B;H),A^{\prime H}\)
	\to (W,A')\subset\(\Omega^*(B;V),A'\)\;.\tag2$$

We will see later
that~(1) means that the difference
between~$A^{\prime H}$ and~$\nabla^H$ is almost negligible.

\Proof
Both~$\Pi$ and~$\iota$ are $\Omega^*(B)$-linear.
Because~$\Pi\dg0$ coincides with the projection
onto the $(a'_0+a''_0)$-harmonic elements of~$V$,
it is clear that we obtain an %$\Omega^*(B)$-linear
isomorphism.
Because~$\Pi$ commutes with~$A'$,
it is clear that~$A'$ acts on~$W$.
It remains to show that the restriction of~$A'$ to~$W$
pulls back to a flat superconnection on~$H$,
which starts with~$\nabla^H$ in degree~$1$.

%because~$a'_0$ commutes with~$\nabla^V+a'_1$.
%The curvature of the superconnection~$A'+a''_0$ is given by
%	$$(A'+a''_0)^2
%	=[A',a''_0]
%	=\bigl[\nabla^V,a''_0\bigr]+\sum_{i\ge0}[a'_i,a''_0]\;.$$
%Let us study the image of~$\eta$ under~$\Pi$.
%Because~$\eta\in\ker\(a_0'+a_0''\)$,
%we have
%$$\split
%	\Pi\,\eta
%	&={1\over2\pi i}
%		\,\int_{\eps S^1}{1\over\lambda-\(A'+a''_0\)^2}
%			\,\eta\,d\lambda\\
%	&=\eta+\sum_{n\ge1}{1\over2\pi i}\,\int_{\eps S^1}
%		{1\over\lambda-[a'_0,a''_0]}
%		\,\biggl(\biggl[\nabla^V+\sum_{i\ge1}a'_i,a''_0\biggr]
%			\,{1\over\lambda-[a'_0,a''_0]}\biggr)^n\eta
%		\,d\lambda\;.
%\endsplit$$
%In particular, the contributions to~$\Pi\,\eta$
%in~$\Omega^j(B;V)$ for~$j=0$, $1$ are given by
%$$\split
%	(\Pi\,\eta)\dg0&=\eta\;,\\
%		\Land
%	(\Pi\,\eta)\dg1
%	&={1\over2\pi i}\,\int_{\eps S^1}{1\over\lambda-[a'_0,a''_0]}
%		\,\bigl[\nabla^V+a'_1,a''_0\bigr]
%		\,{1\over\lambda-[a'_0,a''_0]}\,\eta\,d\lambda\\
%	&={1\over2\pi i}\,\int_{\eps S^1}
%		{1\over\lambda\,\(\lambda-[a'_0,a''_0]\)}
%		\,a''_0\,\(\nabla^V+a'_1\)\,\eta\,d\lambda\\
%	&\in\,\Omega^1\(B;\im(a''_0)\)\;.
%\endsplit$$
%Thus,
%the contributions to~$A'\,\Pi\,\eta$ in~$\Omega^{0,1}(B;V)$ are given by
%$$\split
%	\(A'\,\Pi\,\eta\)\dg0
%	&=a'_0\eta=0\;,\\
%		\Land
%	\(A'\,\Pi\,\eta\)\dg1
%	&=a'_0\,(\Pi\,\eta)\dg1+(\nabla^V+a'_1)\,\eta\;,
%\endsplit$$
%with~$a'_0\,(\Pi\,\eta)\dg1\in\Omega^1\(B;\im(a'_0)\)$
%and~$(\nabla^V+a'_1)\,\eta\in\Omega^1\(B;\ker(a'_0)\)$.

We write the superconnection~$A^{\prime H}$ on~$H$ of~\UniAxHDef\ as
	$$A^{\prime H}=\nabla^H+\sum_{i\ge 0}a^{\prime H}_i$$
with~$a^{\prime H}_i\in\Omega^i(B;\End H)$.
Let~$\eta\in\Omega^0\(B;\ker(a'_0+a''_0)\)$
represent a section of~$H$,
then clearly
	$$a^{\prime H}_0\eta
	=\(\Pi\circ\iota\circ A^{\prime H}\)\dg0\,\eta
	=\(A'\circ\iota\circ\Pi\)\dg0\,\eta
	=a'_0\eta=0\;.$$
To calculate~$a^{\prime H}_1$,
note that since~$a^{\prime H}_0=0$,
we have
$$\align
	\iota\,\(\nabla^H+a^{\prime H}_1\)\,\eta
	&=\(\Pi\circ\iota\circ A^{\prime H}\)\dg1\,\eta
	=\(A'\circ\Pi\circ\iota\)\dg1\,\eta\\
	&=\(\nabla^V+a'_1\)\,\eta+a'_0\,\Pi\dg1\,\eta
	\quad\in\quad\Omega^1\(B;\ker(a'_0+a''_0)\)\;.
\endalign$$
Since the result is in~$\Omega^1(B;\iota H)$
whereas~$\im(a'_0)\perp\iota H$,
we also get
	$$\iota\,\(\nabla^H+a^{\prime H}_1\)\,\eta
	=\Pi\dg0\,\(\nabla^V+a'_1\)\,\eta\;,$$
but~$\Pi\dg0\,\(\nabla^V+a'_1\)$ just represents the Gau\ss-Manin
connection~$\nabla^H$ on~$H$,
so~$a^{\prime H}_1=0$ as well.
%This finishes the proof of the Lemma.
\qed\enddemo

As a consequence,
we can now define a flat superconnection on~$\widehat V=V\oplus H\dg{-1}$
of the form
	$$\widehat A'
	=\pmatrix A'&\Pi\circ\iota\\0&A^{\prime H}\endpmatrix\;,
	\Formel\ConeAxFormel$$
where~$H\dg{-1}$ denotes the $\Z$-graded bundle~$H$
with degree shifted down by one.
The superconnection~$\widehat A'$ is apparently flat
and of total degree~$1$.
By assumption, $A'-\nabla^V$ takes values in a nipotent subalgebra of~$\End V$.
Similarly,
$A^{\prime H}-\nabla^H$ takes values in the nilpotent subalgebra of~$\End H$
that increases the vertical degree.
We conclude that~$\widehat A'-\nabla^{\widehat V}$ also
takes values in a nilpotent subalgebra.
Moreover,
the cohomology~$H$ of~$(V,a_0)$ is killed by~$H\dg{-1}$,
so the fibre-wise operator~$\hat a'_0=a'_0+\Pi\dg0\circ\iota$ is acyclic.

\Definition\ConeDef
Let~$(V,A',\nabla^V,g^V)$ be a family Thom-Smale complex
with an adapted metric,
and let~$g^H$ be a metric on the vector bundle~$H=H^*(V,a'_0)\to B$.
Then we call~$\bigl(\widehat V,\widehat A',\nabla^{\hat V},g^{\hat V}\bigr)$
the {\em acyclic cone\/} of~$\(V,A',\nabla^V\)$.
\enddefinition

\Remark\ConeRem
\roster
\item
The acyclic cone construction as a fibre-wise acyclic family Thom-Smale-complex
is up to homotopy independent of the choice
of metrics~$g^V$ and~$g^H$.
This follows from a standard argument involving an extension of metrics
from~$B\times\{0,1\}$ to~$B\times[0,1]$ on the pullbacks of~$V$ and~$H$
via the projection~$B\times[0,1]\to B$.
\item
If~$g^V$ and~$g^H$ are unitarily flat,
then so is~$g^{\hat V}=g^V\oplus g^H$.
%But now the homotopy type of the acyclic cone
%as a fibre-wise acyclic family Thom-Smale-complex with a parallel metric
%depends on on the choice of~$g^V$ and~$g^H$.
\item
We would like to turn the acyclic cone construction into a functor
from the universal unitary Whitehead category~$\cWh^u\(\Cal M(\C),U\)$
to a suitable acyclic Whitehead category.
Although the whole construction above is natural,
we encounter a technical problem.
We start in~$\cWh^u\(\Cal M_r(\C),U(r)\)$ for some fixed~$r$.
The dimension of the fibre-wise
cohomology~$\Cal H\to\Wh^u\(\Cal M_r(\C),U(r)\)$
depends on the connected component of~$\Wh^u\(\Cal M_r(\C),U(r)\)$
and is in general not equal to~$r$.
This means that~$\cWh^h\(\Cal M_r(\C),U(r)\)$ is not a good receptacle
for a universal cone construction.
Taking the limit~$\lim_{r\to\infty}\cWh^h\(\Cal M_r(\C),U(r)\)$ is difficult
because our stabilisation procedure in \WhUniDimStabDef\
destroys acyclicity.
Similarly,
if we pass to~$\lim_{r\to\infty}\Wh^u\(\Cal M(\C),U\)$,
then the dimension of the bundle~$\widehat{\Cal V}$ still depends on~$r$.
To solve this problem,
we would need a generalisation of the acyclic Whitehead space
that allows to take the limit~$r\to\infty$ in a natural way.
\endroster\endremark


\Abschnitt\UniSpecSeqSubsection Unitary and acyclic higher torsion

We show that
the analytic torsion of a family Thom-Smale complex~$\(V,\nabla^V,A'\)$
is related to the torsion of its acyclic
cone~$\bigl(\widehat V,\nabla^{\hat V},\widehat A',g^{\hat V}\bigr)$.
If both~$V$ and~$H$ carry parallel metrics,
this allows us to reduce the calculation of the unitary torsion
to the acyclic case.

Let~$(V,\nabla^V,A')$ be a family Thom-Smale complex
with an adapted metric~$g^V$,
and let~$\bigl(\widehat V,\nabla^{\widehat V},\widehat A'\bigr)$
be the acyclic cone of \ConeDef.
We have a natural filtration
	$$\(\widehat V,\widehat A'\)\supset (V,A')\supset0\;,
	\Formel\UniFiltFormel$$
to which~$g^{\hat V}=g^V\oplus g^H$ is adapted
in the sense of \FiltSplitDef.
The metric~$g^{\hat V}$ is parallel iff~$g^V$ and~$g^H$ are.
%Since~$\hat a'_0$ is acyclic,
%we do not need any condition on~$g^{\widehat H}$ here.


\Theorem\UniSpecSeqThm.
Let~$\(V,\nabla^V,A'\)$ be a family Thom-Smale complex,
let~$\bigl(\widehat V,\nabla^{\hat V},\widehat A'\bigr)$
be its acyclic cone with respect to the metric~$g^V$,
and let~$g^{\hat V}=g^V\oplus g^H$.
Then modulo exact forms,
we have
	$$T\(\nabla^V,A',g^V\)+\chslo\(\nabla^H,g^H,g^H_V\)
	=T\bigl(\nabla^{\hat V},\widehat A',g^{\hat V}\bigr)\;.$$

\Proof
The bundle~$\widehat V$ has a two-step filtration~\UniFiltFormel\
and carries an adapted metric~$g^{\hat V}=g^V\oplus g^H$.
Moreover, $\bigl(\widehat V,\hat a'_0\bigr)$ is acyclic by construction.
In other words,
the spectral sequence associated to~\UniFiltFormel\
degenerates at~$E_2=0$.

The $E_0$-term of the spectral sequence is the direct sum
	$$\(E_0,\nabla^{E_0},D'_0,g^{E_0}\)
	=\(V,\nabla^V,A',g^V\)
		\oplus\(H\dg{-1},\nabla^H,A^{\prime H},g^H\)\;,$$
and its torsion is given by
	$$T\(\nabla^{E_0},D'_0,g^{E_0}\)
	=T\(\nabla^V,A',g^V\)-T\(\nabla^H,A^{\prime H},g^H\)\;.$$
We extend~$A^{\prime H}$ to a flat superconnection
on~$\overline H=H\times(0,1]$ by
	$$\overline A^{\prime H}
	=s^{N^H}\,\biggl(A^{\prime H}+{\del\over\del s}\,ds\biggr)\,s^{-N^H}$$
and set
	$$\nabla^{\overline H}
	=\(\overline A^{\prime H}\)\dg1
	=\nabla^H+\biggl({\del\over\del s}-{N^H\over s}\biggr)\,ds\;.$$
Then we still have
	$$\overline A^{\prime H}
	=\nabla^{\overline H}+\sum_{i\ge2}\bar a^{\prime H}_i$$
with~$\bar a^{\prime H}_i\in\Omega^i\bigl(B\times(0,1],\End\overline H\bigr)$.

We note that~$\overline H$ is its own fibre-wise cohomology,
and if~$g^{\overline H}$ is a metric on~$\overline H$,
then the induced metric on the fibre-wise cohomology
is again~$g^{\overline H}$,
so
	$$dT\(\nabla^{\overline H},\overline A^{\prime H},g^{\overline H}\)
	=\cho\(\nabla^{\overline H},g^{\overline H}\)
		-\cho\(\nabla^{\overline H},g^{\overline H}\)
	=0\;.$$
We may thus take~$g^{\overline H}$ to be the pullback of~$g^H$.
It is now easy to see that
	$$\lim_{s\to 0}
	T\(\nabla^{\overline H},\overline A^{\prime H},g^{\overline H}\)
		\bigr|_{B\times\{s\}}
%	=T\(\nabla^H,\nabla^H,g^H\)
	=T^{\roman{BL}}\(\nabla^H,g^H\)
	=0\;,$$
and this is cohomologous to~$T\(\nabla^H,A^{\prime H},g^H\)$.
We conclude that
	$$T\(\nabla^{E_0},D'_0,g^{E_0}\)
	=T\(\nabla^V,A',g^V\)
	\quad\in\quad\Omega^\even(B)/d\Omega^\odd(B)\;.
	\Formel\UniEnullFormel$$

The~$E_1$ term of our spectral sequence is given by
	$$\(E_1,\nabla^{E_1},D'_1,g^{E_1}\)
	=\(H\oplus H\dg{-1},\nabla^{H\oplus H},D'_1,g^H_V\oplus g^H\)\;,$$
where the superconnection~$D'_1$ on~$H\oplus H\dg{-1}$
in matrix notation equals
	$$D'_1=\pmatrix\nabla^H&\id\\&\nabla^H\endpmatrix\;.$$
By the appendix of~\BL,
we conclude that
$$\split
	T^{\roman{BL}}\(D'_1,g^{E_1}\)
	&=T^{\roman{BL}}\(D'_1,g^H_V\oplus g^H\)\\
%	&=T^{\roman{BL}}\(D'_1,g^H\oplus g^H\)+\chslo\(\nabla^H,g^H,g^H_V\)\\
	&=\chslo\(\nabla^H,g^H,g^H_V\)\;.
\endsplit\Formel\UniEeinsFormel$$

By \SpecSeqThm,
we now have
$$\split
	T\bigl(\nabla^{\hat V},\widehat A',g^{\hat V}\bigr)
	&=T\(\nabla^{E_0},D'_0,g^{E_0}\)
		+T^{\roman{BL}}\(\nabla^{E_1},D'_1,g^{E_1}\)\\
	&=T\(\nabla^V,A',g^V\)+\chslo\(\nabla^H,g^H,g^H_V\)\;.\quad\qed
\endsplit$$
\enddemo

\Remark\UnitorConeRem
If we assume that both~$g^V$ and~$g^H$ are parallel,
then \UniSpecSeqThm\ gives us an identity of cohomology classes on~$B$.
It shows that the unitary torsion can be completely reduced
to the torsion in the acyclic case.
This is another justification for our
definition of~$\tau$ on~$\Wh^u\(\Cal M(\C),U\)$.

We recall that the torsion
on the acyclic Whitehead space~$\Wh^h\(\Cal M_r(\C),U(r)\)$
is completely determined by its restriction to the two-index
Whitehead space~$\Wh^{h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$,
which is a deformation retract of~$\Wh^h\(\Cal M_r(\C),U(r)\)$
by Igusa's two-index theorem in~\IBuch, Theorem~5.7.1.
It would be nice to know
that~$\tau\in H^\even\bigl(\Wh^u\(\Cal M(\C),U\)\bigr)$ is also
determined by its restriction to~$\Wh^{h,\{0,1\}}\(\Cal M_r(\C),U(r)\)$.
Unfortunately,
for the reasons explained in \ConeRem~(3),
we do not obtain this conclusion immediately.
\endremark


\enddocument









For the next construction,
we have to construct an acyclic Whitehead space~$\Wh^h\(\Cal M(\C),U\)$.
Note that we cannot simply take
the limit~$\lim_{\to}\Wh^h\(\Cal M_r(\C),U(r)\)$,
because extending~$a'_0$ by zeros destroys acyclicity.
Instead,
we will associate a rank~$r_p$ to each element of the graded poset~$P$.

\?Definition?

Let now~$(P,a',e)$ be an object of~$\cWh^{\diff,u}\(\Cal M_r(\C),U(r)\)$,
and assume that~$H^j=H^j\((\C^r)^P,a'_0\)$ is trivial unless~$a\le j\le b$.
We construct a new graded poset
	$$\widehat P=P\cup\{a,a+1,\dots,b\}$$
such that~$P$ inherits its original partial ordering and grading,
the degree of~$j\in\{a,a+1,\dots,b\}$ is~$j-1$,
and
	$$b\prec\dots\prec a\prec P\;.$$
We identify~$H$ with~$\C^{\rk H}$ using the basis~$e$.
Because the dimension of the~$H^j$ could be arbitrarily large,
we have to pass to~$\Wh\(\Cal M(\C),U\)$ at this point.
Let~$\widehat A'$ be defined by~\ConeAxFormel\
and put~$\hat a'=\widehat A'-d$,
where~$d$ denotes the trivial connection on~$\widehat V=(\C^r)^P\oplus H$.
Then~$\hat a'$ is triangular with respect to~$\widehat P$.

\Proposition\ConeFunctorProp.
The construction above gives a functor
	$$\Cal C\colon\cWh^{\diff,u}\(\Cal M_r(\C),U(r)\)
	\to\cWh^{\diff,h}\(\Cal M(\C),U\)\;.$$

\Proof
By \ConeLemma\ and the arguments above,
$\Cal C$ maps objects of the unitary differential
Whitehead category~$\cWh^{\diff,u}\(\Cal M_r(\C),U(r)\)$
to objects of the acyclic category~$\cWh^{\diff,h}\(\Cal M(\C),U\)$.
It thus remains to show that morphisms are mapped to morphisms.
However,
this guaranteed since by \WhUniDef~(2),
$\cWh^{\diff,u}\(\Cal M(\C),U\)$-morphisms induce unitary
maps on the fibre-wise cohomology.
\qed\enddemo

\Remark\ConeRemark
\roster
\item
To obtain a well-defined functor~$\Cal C$,
we had to fix local parallel bases~$e$ of~$\Cal H$
and not just parallel metrics.
\item
Stabilisation with respect to~$r$ in the range of~$\Cal C$
was necessary because there is no bound on~$\rk\Cal H$.
\?No longer acyclic?
\item
Stabilisation with respect to~$r$ in the domain of~$\Cal C$
is not possible however
since our choice of superconnection would introduce additional
additional ``elementary expansions'',
which change the elements of~$\cWh^{\diff,h}\(\Cal M(\C),U\)$.
However,
since elementary exchanges are represented by morphisms,
there is still a way of extending~$\abs{\Cal C}$
to a map from~$\Wh^u\(\Cal M(\C),U\)\to\Wh^h\(\Cal M(\C),U\)$.
\endroster\endremark





\Abschnitt\WhConeSubsection The universal cone construction

We want to turn the construction of \ConeSubsection\ into
a functor from the unitary Whitehead category to the acyclic
Whitehead category.
Unfortunately,
this implies that we have to specify a framing
for each bundle~$\Cal H\to\Wh\(\Cal M(\C),U\)$,
and we have to enlargen both~$R$ and~$G$
since the individual bundles~$\Cal H^i\to\Wh\(\Cal M(\C),U\)$
can have arbitrary rank.

The first problem is captured in the following definition.

\WhUniRem\ remains valid for~$\Wh^{\simp,uf}\(\Cal M(\C),U\)$ with suitable modifications.
Note that we could have worked with~$\Wh^{\simp,uf}\(\Cal M(\C),U\)$ throughout
this section.
Note also that there might be applications where it is wise
to restrict the $\cWh^{\prime\simp,uf}$-morphisms to pairs~$(f,g)$
such that the induced map on cohomology preserves an additional structure.
For example, if~$G=\GL(r,\Z)\cap U(r)$,
it is meaningful to demand that the induced maps
	$$(f,g)_*\colon H^*\(V^P,a(i)\)\to H^*\(V^Q,b(i)\)$$
in \WhUniDef\ are given by integral unitary matrices
with respect to the bases~$e$, $e'$.
Since we are only dealing with higher torsion here,
it is enough for us to work with arbitrary unitary matrices.

Note that higher analytic torsion is defined without reference
to a particular framing.

\Proposition\UniFrameProp.
There exists a forgetful functor~$\cWh^{uf}\(\Cal M(\C),U\)\to\cWh^u\(\Cal M(\C),U\)$.
If~$G$ is a subgroup of~$U(r)$,
then the unitary higher analytic torsion is preserved by this functor.
\qed

On the other hand,
the cone construction of \ConeSubsection\ provides us with
a functor from the unitary to the acyclic Whitehead category.
It follows from \UniSpecSeqThm\ that this functor is compatible
with the higher analytic torsion.

\Theorem\UniConeThm.
The cone construction is a functor
	$$\Cal C\colon\cWh^{uf}\(\Cal M(\C),U\)\to\cWh^h\(\Cal M_r(\C),\GL(\C)\)\;.$$
In particular,
the unitary framed Whitehead space~$\Wh^{uf}\(\Cal M_r(\C),\GL(\C)\)$
contains the acyclic Whitehead space~$\Wh^h\(\Cal M_r(\C),\GL(\C)\)$
as a retract.
\parr
Assume that~$G$ is a subgroup of~$U(r)$,
then the cone construction defines a functor
	$$\Cal C\colon\cWh^{uf}\(\Cal M(\C),U\)\to\cWh^h\(\Cal M(\C),U\)\;,$$
and the unitary higher torsion class on~$\Wh^{uf}\(\Cal M(\C),U\)$
is given as the pullback of the higher torsion class
on the acyclic unitary Whitehead space~$\Wh^h(\Cal M(\C),U)$.

\Proof
This is an easy consequence of \UniSpecSeqThm.
\qed\enddemo

Let~$\cWh^{h,\{0,1\}}\(\Cal M(\C),U\)$ denote the full subcategory of~$\cWh^h\(\Cal M(\C),U\)$
such that the graded poset~$P$ is concentrated in degrees~$0$ and~$1$,
and let~$\Wh^{h,\{0,1\}}\(\Cal M(\C),U\)$ denote its geometric realisation.
It is proved in~\IBuch, Chapter~5,
that~$\Wh^{h,\{0,1\}}\(\Cal M(\C),U\)$ is contained in~$\Wh^h\(\Cal M(\C),U\)$
as a deformation retract.
Compatibility of~$\tau$ with the cone construction
has the following easy consequence.

\Corollary\UniTwoIndexCor.
The unitary higher torsion class on~$\Wh^{uf}\(\Cal M(\C),U\)$ is completely determined
by its restriction to~$\Wh^{h,\{0,1\}}\(\Cal M(\C),U\)$.
\qed

In other words,
the universal torsion class~$\tau\in H^\even\(\Wh^{uf}\(\Cal M(\C),U\)\)$
is a natural extension of the class~$\tau\in H^\even\(\Wh^h\(\Cal M(\C),U\)\)$
considered in~\IBuch.


